Integrated Resource Allocation and Strategy Synthesis in Safety Games on Graphs with Deception

Deception plays a crucial role in strategic interactions with incomplete information. Motivated by security applications, we study a class of two-player turn-based deterministic games with one-sided incomplete information, in which player 1 (P1) aims to prevent player 2 (P2) from reaching a set of target states. In addition to actions, P1 can place two kinds of deception resources: "traps" and "fake targets" to disinform P2 about the transition dynamics and payoff of the game. Traps "hide the real" by making trap states appear normal, while fake targets "reveal the fiction" by advertising non-target states as targets. We are interested in jointly synthesizing optimal decoy placement and deceptive defense strategies for P1 that exploits P2's misinformation. We introduce a novel hypergame on graph model and two solution concepts: stealthy deceptive sure winning and stealthy deceptive almost-sure winning. These identify states from which P1 can prevent P2 from reaching the target in a finite number of steps or with probability one without allowing P2 to become aware that it is being deceived. Consequently, determining the optimal decoy placement corresponds to maximizing the size of P1's deceptive winning region. Considering the combinatorial complexity of exploring all decoy allocations, we utilize compositional synthesis concepts to show that the objective function for decoy placement is monotone, non-decreasing, and, in certain cases, sub- or super-modular. This leads to a greedy algorithm for decoy placement, achieving a $(1 - 1/e)$-approximation when the objective function is sub- or super-modular. The proposed hypergame model and solution concepts contribute to understanding the optimal deception resource allocation and deception strategies in various security applications.

==> sections/1_intro_automatica.tex <==
In security and defense applications, deception plays a key role to mitigate the information and strategic disadvantages of the defender against adversaries. In this paper, we investigate the design of active defense with deception for a class of reachability games \cite{de_alfaro_concurrent_2007} that represent a sequential interaction between an attacker and a defender. In this game, the attacker's objective is to reach a set of target states \cite{manna_temporal_1992}, while that of the defender is to thwart the attacker by selecting counter-actions and allocating decoys to disinform the attacker. We consider two classes of deception resources that serve the functions of \emph{hiding the real} and \emph{reveal the fiction} \cite{heckman_bridging_2015}. Hiding the real refers to defender simulating a trap to function like a real state, while revealing the fiction corresponds to camouflaging a state to look like a target state for attacker. Given this setup, we are interested in the following problem: \emph{How to optimally allocate the decoys so that the defender can influence the attacker into taking (or not taking) certain actions that maximize the defender's winning region?} The winning region is defined as the set of game states from which the defender has a strategy to prevent the attacker from successfully completing its attack mission.


As a motivating problem, consider a variant of the decoy placement problem over an attack-defend game graph, as studied in the field of cybersecurity \cite{}. In this problem, the objective of the attacker (P2) is to attain control over one of the target machines present in the network, while the defender (P1) strives to prevent such an outcome. To accomplish this, the attacker exploits vulnerabilities and enacts multi-stage lateral movements to escalate its privileges, while the defender dynamically adjusts the network configuration in response. The problem asks us to identify the optimal placement of honeypots, which hide the real by acting as traps and disrupting the attacker movement, and honeynets, which reveal the fiction by imitating a genuine data server and diverting attacker's attention to safeguard the real server from compromise.

%I.1. Effect of decoy insights. structure and objective. 
%I.2. control of P2's perception and its strategy. 
%I.3. Concept of stealthy deception under sure and almost-sure conditions. 
\ak{Explain key challenges posed by this problem. How to model P1's ability to reason about P2's perception? Coupling of strategy and placement.}

\paragraph*{Contributions.} To address this problem, we introduce a class of \emph{hypergames on graph} that allow us to model the consequence of P1 allocating a subset of states in the reachability game as either ``traps'' or ``fake targets'' on P2's perception. In principle, the traps alter the structure of the game but do not affect P2's perception, whereas the fake targets manipulate P2's perception the goal states in the game. Thus, by deciding the location of decoys P1 can control P2's perception and, therefore, its behavior. 


We introduce two solution concepts to study the equilibrium strategies of player in the hypergame on graph called \emph{stealthy deceptive sure winning} and \emph{stealthy deceptive sure winning}, and present a procedure to synthesize them. Intuitively, a deceptive strategy leverages P2's misperception to prevent the game from reaching a target state. While the stealthiness of the strategy prevents P2 from becoming aware of its misperception until a decoy state is reached. 


When analyzing the interaction under the sure winning condition, the players are assumed to follow deterministic strategies. In this case we show that \emph{fake targets could be more advantageous than traps.} Whereas, when the interaction is analyzed under the almost-sure winning condition and the players are assumed to follow randomized strategies, we find that \emph{neither the fake targets nor the traps provide a greater benefit over the other}. These insights enable us to design an algorithm to synthesize a stealthy deceptive sure/almost-sure winning strategy given a fixed placement decoys. 


%II.1. Cyclic dependence + Combinatorial problem. Solution by compositionality. 
%II.2. Decoupling of placement problem. Insights of fakes powerful than traps and otherwise. 
%II.3. Conditions for sub and super modularity. Algorithm. 
%However, determining a placement of decoys that yields the maximum size of stealthy deceptive sure/almost-sure winning region is a combinatorial problem. To derive a tractable placement algorithm, we show three properties: (1) We can decouple the placement of traps and fake targets because fake targets are at least as advantageous as traps; (2) Drawing inspiration from ideas in compositional synthesis \cite{filiot_antichains_2011,kulkarni_compositional_2018}, we derive the sufficient conditions when the objective function (\ie, the size of stealthy deceptive sure/almost-sure winning region) is submodular or supermodular; (3) Based on this, we can construct an under-approximation of the deceptive sure-winning regions incrementally (in polynomial time), instead of having to solve a combinatorially large number of hypergames for all possible decoy configurations.

However, the task of determining an optimal placement of decoys that maximizes the size of the stealthy deceptive sure/almost-sure winning region poses a challenging combinatorial problem. To address this challenge and develop an algorithm with practical feasibility, we establish three key properties. Firstly, we demonstrate that the placement of traps and fake targets can be treated independently, as fake targets offer at least the same advantages as traps. Secondly, drawing insights from concepts in compositional synthesis \cite{filiot_antichains_2011,kulkarni_compositional_2018}, we establish sufficient conditions under which the objective function (i.e., the size of the stealthy deceptive sure/almost-sure winning region) exhibits submodularity or supermodularity property. Lastly, leveraging these findings, we propose an incremental construction of an under-approximation of the deceptive sure-winning regions, accomplished in polynomial time. This approach alleviates the need to exhaustively solve a large number of hypergames for all possible configurations of decoys.


\paragraph*{Related Work}
The problem of optimal allocation of deception resources has received considerable attention in the domain of cyber- and cyber-physical system security. We refer the readers to \cite{Pawlick2019, Zhu2021} for a comprehensive survey on game-theoretic approaches to cyber deception. In \cite{pibil_game_2012,kiekintveld_game-theoretic_2015}, the authors propose a game-theoretic method to place honeypots in a network so as to maximize the probability that the attacker attacks a honeypot and not a real system. In their game formulation, the defender decides where to insert honeypots in a network,  and the attacker chooses one server to attack and receives different payoffs when attacking a real system (positive reward) or a honeypot (zero reward).  The game is imperfect information as the real systems and honeypots are indistinguishable for the attacker. By the solution of imperfect information games, the defender's honeypot placement strategy is solved to minimize the attacker's rewards. 


Security games \cite{sinha_stackelberg_2018,kiekintveld_computing_2009} are another class of important models for resource allocation in adversarial environments.  In  \cite{thakoor_cyber_2019}, the authors formulate a security game (Stackelberg game) to allocate limited deception resources in a cybernetwork to mask network configurations from the attacker. This class of deception manipulates the adversary's perception of the payoffs and thus causes the adversary to take (or not  to take) certain actions that aid the objective of the defender. In \cite{durkota_optimal_2015}, the authors formulate an Markov decision process to assess the effectiveness of a fixed honeypot allocation in an attack graph, which  captures multi-stage lateral movement attacks in a cybernetwork and dependencies between vulnerabilities \cite{jha_two_2002,ouScalableApproachAttack2006}. In \cite{anwar_honeypot_2020}, the authors analyze the honeypot allocation problem for attack graphs using normal-form games, where the defender allocates honeypots that changes the payoffs matrix of players. The optimal allocation strategy is determined using the minimax theorem. The attack graph is closely related to our game on graph model, which   generalizes the attack graph to \emph{attack-defend game graphs} \cite{jiang_optimal_2009,aslanyan_quantitative_2016} by incorporating the defender counter-actions in active defense.


There are several key distinctions between our work and the prior work. First, our work focuses on a qualitative approach to decoy placement instead of a quantitative one, which often requires solving an optimization problem over a well-defined reward/cost function. In the qualitative approach, we represent the P2's goal as Boolean behavioral objectives such as reachability, safety or a combination of these. Second, we show how to incorporate the P2's misinformation about decoy locations into a hypergame model. Hypergames \cite{bennett_hypergame_1986,sasaki_hierarchical_2016,wang_solution_1989} are a class of games with one-sided incomplete information in which different players might play according to different perceptual games that capture the information and higher-order information known to that player. While the underlying idea behind our game model is similar to ``indistinguishable honeypots'' discussed in \cite{pibil_game_2012}, we are able to leverage the solution approaches for hypergames to address decoy allocation problem. Third, we solve for a stealthy strategy for the defender, which ensures that defender's actions will not inform the attacker that deceptive tactics are being used. Lastly, we borrow the idea of compositional reasoning from formal methods to find approximately optimal solutions for the decoy allocation problem for this class of hypergames.

The paper is structured as follows. In Section~\ref{sec:prelim}, we discuss the preliminaries of reachability game on graph model to capture the interaction between P1 and P2 in which P2 does not know the locations of decoy resources. Section~\ref{sec:problem} formalizes our problem statement. In Section~\ref{sec:main}, we present the main results of this paper. Section~\ref{subsec:hypergames} introduces the hypergame on graph model and the notion of stealthy deceptive strategies, Section~\ref{subsec:p2-best-response} provides insight into the effect of deception resources on P2's perceptual game and its strategy, Sections~\ref{subsec:dswin} presents a procedure to synthesize stealthy deceptive winning strategy for P1 under sure winning criterion. In Section~\ref{subsec:placement}, we discuss the key properties of the objective function of the optimal decoy placement problem and develop a polynomial-time greedy algorithm to place the decoys. Section~\ref{subsec:daswin} extends the results obtained in previous two sub-sections to stealthy deceptive strategies under almost-sure winning criterion. We conclude the paper with a case study in Section~\ref{sec:experiment} and a conclusion. 




==> sections/allocation.tex <==
\paragraph*{} Based on the insights from Section~\ref{sec:deception}, in this section, we present a near-optimal approach to decoy placement. First, we introduce a metric to characterize the value of deception.   
%
%
\begin{align}
	\vod(X, Y) = \frac{|\dswin_1(X, Y) \cap \win_2(\game, F)|}{|\win_2(\game, F) \setminus F|}
\end{align}
%
%
\paragraph*{} The value of deception measures the proportion of P2's sure winning states in $\win_2(\game, F)$ that become  sure winning for P1 in $\widehat{\hgame}_1(X, Y)$. $\vod(X, Y)$ is a rational number between $0$ and $1$ where the value of $0$ denotes that P1 gains no advantage and the value of $1$ denotes that P1 gains maximum advantage by given decoy allocation. $\vod(X, Y) = 0$ occurs when $|\dswin_1(X, Y)| = |\win_1(\game, F)|$ and $\vod(X, Y) = 1$ occurs when P1 has a sure winning strategy to visit a decoy from every P2's non-final winning state in $\game$. 


\paragraph*{} Given the metric $\vod(X, Y)$, the optimal decoy placement is the solution of the following optimization problem:
%
%
\begin{equation} \label{eq:optimization-problem}
\begin{aligned}
	&\max_{X, Y \subseteq S} \vod(X, Y) \\
	&\mbox{subject to: } |X| \leq k ~\mbox{and}~ |Y| \leq m		
\end{aligned}
\end{equation}


\paragraph*{} Every choice defines a different hypergame, $\widehat\hgame_1(X, Y)$. Thus, solving Eq.~\ref{eq:optimization-problem} entails identifying a hypergame that has the largest deceptive sure-winning region of P1. A na\"ive approach is to compute $\dswin_1(X, Y)$ for each $X, Y \subseteq S \setminus F$ and then select a pair $X, Y$ for which $\abs{\dswin_1(X, Y)}$ is the largest. However, this approach is not scalable as the number of hypergames that must be solved is ${|\win_2(\game, F) \setminus F|} \choose {k + m}$, which increases rapidly with the size of game and the number of decoys that are to be placed. Hence, we propose a greedy approach to approximate the solution to Eq.~\ref{eq:optimization-problem}.


%\paragraph*{} Since every choice of $X, Y \subseteq S \setminus F$ defines a different hypergame, $\widehat\hgame_1(X, Y)$, solving Eq.~\ref{eq:optimization-problem} reduces to identifying a hypergame that has the largest deceptive sure-winning region, $\abs{\dswin_1(X, Y)}$. For this, a na\"ive approach would be to compute $\dswin_1(X, Y)$ for each $X, Y \subseteq S \setminus F$ and then select a pair $X, Y$ for which $\abs{\dswin_1(X, Y)}$ is the largest. Clearly, this approach is not scalable because the number of subsets, which is equal to \ak{${|S \setminus F|} \choose {k + m}$?}, increases rapidly with the size of game. To this end, we propose a greedy approach to approximate the solution to Eq.~\ref{eq:optimization-problem}.


\paragraph*{} In our previous work \cite{kulkarni2020decoy}, we have proposed a greedy-max algorithm to maximize $\vod(X, Y)$ when only traps are placed, \ie, $Y = \emptyset$. For this, we first define a function $f(X) = \abs{\dswin_1(X, \emptyset) \cap \win_2(\game, F)}$ and observe its key property: $f$ is monotone, non-decreasing and superadditive function that, under certain conditions on the topology of $\widehat{\hgame}_1(X, Y)$, $f$ becomes supermodular. When $f$ is supermodular, Eq.~\ref{eq:optimization-problem} is a supermodular maximization problem, for which there exists well-known greedy algorithm \cite{} that, in polynomial-time, computes a $(1-\frac{1}{e})$-approximate solution to Eq.~\ref{eq:optimization-problem}.


%For this, we first define a function $f(X) = \abs{\dswin_1(X, \emptyset) \cap \win_2(\game, F)}$ that counts the number of P2's winning states in $\game$ that become deceptively sure winning for P1 in $\widehat{\hgame}_1(X, Y)$. We, then, design the greedy-max algorithm based on the following three key ideas: (a) $\dswin_1$ operator enjoys compositional property, (b) $f$ is a superadditive function\footnote{A function $f$ is superadditive whenever $f(Z_1 \cup Z_2) \geq f(Z_1) + f(Z_2)$. A function $f$ is supermodular whenever $f(Z_1 \cup Z_2) + f(Z_1 \cap Z_2) \geq f(Z_1) + f(Z_2)$.}, and (c) under certain conditions on the topology of $\widehat{\hgame}_1(X, Y)$, $f$ becomes supermodular. When $f$ is supermodular, we designed a polynomial-time, bounded approximation to Eq.~\ref{eq:optimization-problem} based on the well-known greedy algorithm for supermodular function maximization \cite{}. 


%\paragraph*{} There are three key ideas behind the greedy-max algorithm described in \cite{kulkarni2020decoy}: (a) $\dswin_1$ operator has compositional property, (b) $\dswin_1(X, \emptyset)$ is a superadditive function, and (c) under certain conditions on the topology of $\widehat{\hgame}_1(X, Y)$, $\dswin_1(X, \emptyset)$ becomes supermodular\footnote{A function $f$ is superadditive whenever $f(Z_1 \cup Z_2) \geq f(Z_1) + f(Z_2)$. A function $f$ is supermodular whenever $f(Z_1 \cup Z_2) + f(Z_1 \cap Z_2) \geq f(Z_1) + f(Z_2)$.}. Thus, under these conditions, we adopted the well-known greedy algorithm for supermodular function maximization from \cite{} to design a polynomial-time, bounded approximation to Eq.~\ref{eq:optimization-problem}.  


\paragraph*{} Next, we show that the same procedure can be extended to place traps and fake targets to maximize $\dswin_1(X, Y)$. Algorithm~\ref{alg:greedymax} shows the procedure to place traps and fake targets. 


\begin{algorithm}[tb]
	\begin{algorithmic}[1]
		\item[\textbf{Inputs:}] $\langle S, A, T, F \rangle$: Base game, $k$: Number of traps to placed, $Y$: Number of fake targets to be placed.
		\item[\textbf{Outputs:}] $X, Y$: Placement of traps and fake targets for near-optimal $\vod(X, Y)$. 
		\State Initialize $X, Y$ to be empty sets. 
		\While {$m - |Y| > 0$}
			\State $D \gets \{v \in \win_2(\game, F) \mid v \notin (F \cup Y)\}$
			\If{$D$ is empty}
				\State Exit While
			\EndIf 
			\State Initialize $Z$ as a map from state to vod.
%		\State   For node in PotentialDecoys:
%		\State     vod, pi1, pi2 = solve(G, traps, fakes U {node}) 
%		\State     solutions[node] <- (vod, pi1, pi2) 
%		\State   next_fake <- node with maximum vod. 
%		\State   Add next_fake to fakes
		\State \EndWhile
%		#11. While ntraps - |traps| > 0:
%		#12.   PotentialDecoys = {v in Win2 | v is not final, not marked fake, not marked traps}
%		#13.   If |PotentialDecoys| == 0: Terminate 
%		#14.   solutions = {}
%		#15.   For node in PotentialDecoys:
%		#16.     vod, pi1, pi2 = solve(G, traps U {node}, fakes) 
%		#17.     solutions[node] <- (vod, pi1, pi2) 
%		#18.   next_trap <- node with maximum vod. 
%		#19.   Add next_trap to traps
%		\State \Return 
	\end{algorithmic}
	\caption{P1's Deceptively Sure Winning Region}
	\label{alg:greedymax}
\end{algorithm}



%For this to be true, the function $f(X, Y) \coloneqq \abs{\dswin_1(X, Y) \cap \win_2(\game, F)}$ should exhibit supermodularity under some conditions. 


\paragraph*{} Observe that any greedy optimal decoy placement algorithm must place fake targets first and then traps. This is because, by Theorem~\ref{thm:traps-fakes-subset-relation}, the number of states that jump from $\win_2(\game, F)$ to $\widehat{\hgame}_1(X, Y)$ when a fake target is placed at a state is greater than or equal to the case when a trap is placed the same state. Hence, we can write $f(X, Y) = g(Y) + h_Y(X)$, where $g(Y)$ counts the number of deceptive sure winning states when only fake targets are placed and $h_Y(X)$ counts the number of deceptive sure winning states when traps are allocated after allocating fake targets $Y$. We know from \cite[Corollary~2]{kulkarni2020decoy} that $h_Y$ is superadditive for any $Y \subseteq \win_2(\game, F)$ and supermodular when the conditions in \cite[Theorem~1]{kulkarni2020decoy} are satisfied. Next, we describe the conditions for $g(Y)$ to be supermodular. 


%\paragraph*{} We know from \cite[Corollary~2]{kulkarni2020decoy} that placing traps in any subset $\calD \subseteq \win_2(\game, F) \setminus F$ is superadditive. We now prove that placing fake targets in $\win_2(\game, F) \setminus F$ is also superadditive. Let $f(X, Y) \coloneqq \abs{\dswin_1(X, Y) \cap \win_2(\game, F)}$ count the number of P2's winning states in $\game$ that become sure winning for P1 in $\widehat{\hgame}_1(X, Y)$. Given we first place fake targets and then traps, we can write $f(X, Y) = g(Y) + h_Y(X)$, where $h(Y)$ counts the number of deceptive sure winning states when only fake targets are placed and $h_Y(X)$ counts the number of deceptive sure winning states when traps are allocated after allocating fake targets $Y$. We know from \cite[Corollary~2]{kulkarni2020decoy} that $h_Y$ is superadditive for any $Y \subseteq \win_2(\game, F)$. 


\begin{theorem} 
	The following statements are true. 
	\begin{enumerate}[(a)]
		\item $g$ is a monotone, non-decreasing, and superadditive function. 
		
		\item $g$ is modular if, for all  $Y \subseteq S \setminus F$ and any $s \in S \setminus F$, we have $\dswin_1(\emptyset, Y) \cup \dswin_1(\emptyset, \{s\}) = \dswin_1(\emptyset, Y \cup \{s\})$. 
		
		\item $g$ is supermodular if, for all  $Y \subseteq S \setminus F$ and any $s_1, s_2 \in S \setminus F$ and $s_1 \neq s_2$, we have $\dswin_1(X, Y \cup \{s_1\}) \cap \dswin_1(X, Y \cup \{s_2\}) = \dswin_1(X, Y) $ 
	\end{enumerate}
\end{theorem}
%\begin{proof}[Proof (Internal Use.)]
%	Prove it for sanity check. 
%\end{proof}


\paragraph*{} The proof of above theorem is similar to that of \cite[Theorem~1]{kulkarni2020decoy}. This is because $\dswin_1(X, Y)$ is computed analogous to $\dswin_1(X, \emptyset)$ is computed in \cite{kulkarni2020decoy} and it shares similar properties as $\dswin_2(X, \emptyset)$.


\paragraph*{} Based on Proposition~\ref{} and Theorem~\ref{}, the placement of traps and fake targets amounts to invoking the greedy-max algorithm \cite[Algorithm~1]{kulkarni2020decoy} twice; first to allocate fake targets and then to place traps. This procedure is listed in Algorithm~\ref{}. The algorithm starts with an empty set of states $\mathtt{Decoys}$ and incrementally adds new decoys to these set.  At each step, given the deceptive winning region of the chosen decoys, a new decoy is selected such that by adding the new decoy into the chosen decoys, P1's deceptive sure-winning region covers the largest number of states not included in $\dswin_1(X_k)$. 








==> sections/allocation2.tex <==
Given a placement of traps and fake targets, Theorem~\ref{thm:hgame-swin-is-dswin} provides a way to compute P1's deceptive sure winning region. In this section, we propose a polynomial-time algorithm to find a near-optimal placement of decoys that solve Problem~\ref{prob:decoy-placement}, which can be rewritten equivalently as following optimization problem: %maximize the size of P1's deceptive sure winning region. 


\begin{equation}
	\label{eq:problem}
	% 
	\begin{aligned}
	&X^\ast, Y^\ast = \argmax_{\begin{subarray}{c}X, Y \subseteq \win_2(\game, F) \setminus F,\\
			X \cap Y = \emptyset\end{subarray}} \left| \dswin_1(X, Y) \right|  \\
	&\quad \mbox{subject to: } \card{X} \leq M, \card{Y} \leq N.
	\end{aligned}
\end{equation}


In Eq.~\ref{eq:problem}, every distinct choice of  $X, Y$ defines a hypergame, $\widehat\hgame_1(X, Y)$, which must be solved to determine the size of $\dswin_1(X, Y)$. A na\"ive approach to solving Eq.~\ref{eq:problem} is to compute $\dswin_1(X, Y)$ for each possible placement of $X, Y$ and then select a set $X \cup Y$ for which $\abs{\dswin_1(X, Y)}$ is the largest. However, this approach is not scalable because number of hypergames to solve is ${|\win_2(\game, F) \setminus F|}\choose{M+N}$, which grows rapidly with the size of game and number of decoys to place. To address this issue, we introduce a compositional approach to decoy placement in which we show that, when certain conditions hold, the decoy allocation problem can be formulated as a constrained supermodular maximization problem, for which a $(1 - \frac{1}{e})$-approximation can be computed in polynomial time using a greedy algorithm \cite{}. 


A key insight behind our algorithm is that \emph{fake targets can be more advantageous than traps}. This enables us to separate the placement of traps and fake targets. %, allowing us to leverage the findings from our previous work \cite{kulkarni2020decoy}. In that work, we studied Problem~\ref{prob:decoy-placement} when traps alone are placed (i.e., $Y = \emptyset$).


\begin{theorem}
	\label{thm:traps-fakes-subset-relation}
	% 
	For any $Z \subseteq \win_2(\game, F) \setminus F$, we have $\dswin_1(Z, \emptyset) \subseteq \dswin_1(\emptyset, Z)$.
\end{theorem}
\begin{proof}
	To establish the theorem, it is crucial to examine the impact of placing fake targets on P2's subjectively rationalizable strategy, which is computed using P2's perceptual game $\game_{\emptyset, Z}^2$. Let $\pi_1$ be any P1's deceptively sure winning strategy in $\widehat{\hgame}_1(Z, \emptyset)$. We will show that $\pi_1$ is P1's deceptively sure winning strategy in $\widehat{\hgame}_1(\emptyset, Z)$.
	
	Consider any P1 state $s \in \dswin_1(Z, \emptyset)$ such that the state $s' = \widehat{T}_{Z, \emptyset}(s, \pi_1(s))$ is a P2 state. Then, by definition, every subjectively rationalizable action in $\srAct(s')$ is rank-reducing in $\widehat{\hgame}_1(Z, \emptyset)$. This is because a subjectively rationalizable strategy in $\widehat{\hgame}_1(Z, \emptyset)$ is a sure winning strategy in P2's perceptual game, $\game_{Z, \emptyset}^2$.
	
	Now, consider the transition $s \xrightarrow{\pi_1(s)} s'$ in P2's perceptual game, $\game_{\emptyset, Z}^2$, with fake targets. As demonstrated in Example~\ref{ex:}, the allocation of fake targets results in changes to the ranks of states within $\win_2(\game, F) \setminus F$. By extension, it affects P2's subjectively rationalizable strategy. However, Proposition~\ref{prop:effect-on-p2} provides assurance that every state in $\win_2(\game, F) \setminus F$ remains a sure winning state for P2 in its perceptual game $\game_{\emptyset, Z}^2$. This gives rise to two cases:
	
	(a) The set of subjectively rationalizable actions at $s'$ in $\game_{Z, \emptyset}^2$ and $\game_{\emptyset, Z}^2$ is equal. Then, the transition $s \xrightarrow{\pi_1(s)} s'$ remains winning for P1.
	
	(b) The set of subjectively rationalizable actions at $s'$ in $\game_{Z, \emptyset}^2$ and $\game_{\emptyset, Z}^2$ is not equal. Then, there exists a state $s'' = \widehat{T}(s', \pi_2(s'))$ such that $s''$ is unreachable from $s'$ under any subjectively rationalizable strategy in $\widehat{\hgame}_1(Z, \emptyset)$. This can happen only if $\rank(s'')$ is smaller than $\rank(s')$ in $\widehat{\hgame}_1(\emptyset, Z)$, which means that P2 has a strategy to visit $F \cup Z$ in at-most steps $\rank(s_{i+1}')$-many steps in $\game_{\emptyset, Z}^2$. Since addition of fake targets does not add any new path from $s''$ to $F$, the reduction of rank of $s''$ must be because P2 has a strategy to visit $Z$ within $\rank(s_{i+1}')$-many steps in $\game_{\emptyset, Z}^2$. Therefore, the transition $s \xrightarrow{\pi_1(s)} s'$ remains winning for P1.		
\end{proof}


It follows from Theorem~\ref{thm:traps-fakes-subset-relation} that any greedy algorithm to place traps and fake targets to solve Problem~\ref{prob:decoy-placement} must place fake targets before placing the traps. In our previous work \cite{kulkarni2020decoy}, we have studied the Problem~\ref{prob:decoy-placement} when only traps are placed, \ie, $Y = \emptyset$. Thus, in the sequel, we first study how to optimally place the fake targets and then propose an algorithm to jointly place the fake targets and traps. 


The concept of compositionality is important in the development of a greedy algorithm for Problem~\ref{prob:decoy-placement}. It enables us to incrementally place fake targets one by one, thereby, constructing $\dswin_1(\emptyset, Y)$ in an incremental manner. Indeed, $\dswin_1(\emptyset, Y)$ is compositional. 


\begin{proposition}
	\label{prop:or-composition}
	% 
	Let $\dswin_1(\emptyset, \{s_1\})$ and $\dswin_1(\emptyset, \{s_2\})$ be P1's deceptive sure-winning regions in the hypergames $\widehat\hgame_1(\emptyset, \{s_1\})$ and $\widehat\hgame_1(\emptyset, \{s_2\})$, respectively. Then, P1's deceptive sure-winning region $\dswin_1(\emptyset, \{s_1, s_2\})$ in the reachability game $\widehat\hgame_1(\emptyset, \{s_1, s_2\})$ is equal to the sure-winning region for P1 in the following game:
	\begin{align*}
		\widehat\hgame_1(\{s_1, s_2\}) = \langle &\win_2(\game_{X, Y}^2, F), A, \widehat T,  \\ 
			&\dswin_1(\emptyset, \{s_1\}) \cup \dswin_1(\emptyset, \{s_2\}) \rangle,
	\end{align*} 
	where P1's goal is to reach the target set $\dswin_1(\emptyset, \{s_1\}) \cup \dswin_1(\emptyset, \{s_2\})$
	and P2's goal is to prevent P1 from reaching the target set.
\end{proposition}
\begin{proof}
	We observe that the underlying graphs of the three deceptive reachability games, namely $\widehat\hgame_1(\emptyset, \{s_1\})$, $\widehat\hgame_1(\emptyset, \{s_2\})$, and $\widehat\hgame_1(\emptyset, \{s_1, s_2\})$, are identical. However, they differ in terms of the reachability objectives for P1. By definition of sure-winning regions, from every state $s \in \dswin_1(\emptyset, {\{s_i\}})$ for $i = 1, 2$, there exists a deceptive sure-winning strategy $\pi_1^{\{s_i\}}$ for P1 to ensure  $\{s_i\}$ is reached in finitely many steps, for any subjectively rationalizable strategy of P2. Clearly, every state in $\dswin_1(\emptyset, {\{s_i\}})$ is also winning in $\widehat\hgame_1(\emptyset, \{s_1, s_2\})$. Moreover, for any state $s \notin \dswin_1(\emptyset, {\{s_1\}}) \cup \dswin_1(\emptyset, {\{s_2\}})$ to be winning in $\widehat\hgame_1(\emptyset, \{s_1, s_2\})$, it must visit a state in the set $\dswin_1(\emptyset, {\{s_1\}}) \cup \dswin_1(\emptyset, {\{s_2\}})$. This is because the final states of $\widehat\hgame_1(\emptyset, \{s_1, s_2\})$ are contained in it.  
\end{proof}

%\begin{proof}[From GameSec (partially adopted)]
%	We observe that the underlying graphs of the three deceptive reachability games, namely $\widehat\hgame_1(\emptyset, \{s_1\})$, $\widehat\hgame_1(\emptyset, \{s_2\})$, and $\widehat\hgame_1(\emptyset, \{s_1, s_2\})$, are identical. However, they differ in terms of the reachability objectives for P1, denoted as $\{s_1\}$, $\{s_2\}$, and $\{s_1,s_2\}$, respectively. By definition of sure-winning regions, from every state $s \in \dswin_{\{s_i\}}$ for $i = 1, 2$, there exists a deceptive sure-winning strategy $\pi_1^{\{s_i\}}$ for P1 to ensure  $F\{s_i\}$ is reached in finitely many steps, for any subjectively rationalizable strategy of P2.
%	
%	Let $W^\ast$ be the sure-winning region for P1 in $\widehat \hgame_1(\emptyset, {\{s_1, s_2\}})$ and $\pi_1^\ast$ be a sure-winning strategy of P1. From a state $s \in W^\ast$, P1 can ensure to reach a state, say $s' \in \dswin_{\{s_1\}} \cup \dswin_{\{s_2\}}$ by following $\pi^\ast$. Upon reaching a state $s'$, P1 can ensure to reach a state in either $\{s_1\}$ or $\{s_2\}$---that is, P1 can ensure to reach a state in $\{s_1,s_2\}$. Hence, a sure-winning  state $s$ in the above reachability game is deceptive sure-winning in $\widehat\hgame_1(\emptyset, {\{s_1,s_2\}})$ in which $\{s_1,s_2\}$ is P1's reachability objective. 
%	
%	The deceptive sure-winning strategy
%	is sequentially composed of strategies $\pi^\ast$, $\pi_{\{s_1\}}^\ast$, and $\pi_{\{s_1\}}^\ast$ as follows: From a state $(s,q)\in W^\ast$, P1 uses $\pi^\ast$ until a state in $\dswin_{\{s_1\}}\cup \dswin_{\{s_2\}}$ is reached. If $\dswin_{\{s_1\}} \setminus \dswin_{\{s_2\}}$ is reached, P1 uses the  sure-winning strategy $\pi^\ast_{\{s_1\}}$; If $\dswin_{\{s_2\}}\setminus \dswin_{\{s_1\}}$ is reached, P1 uses the sure-winning stratgy $\pi^\ast_{\{s_2\}}$; if $\dswin_{\{s_1\}} \cap \dswin_{\{s_2\}}$, P1 selects one of $\pi^\ast_{\{s_1\}}$ and $\pi^\ast_{\{s_2\}}$ arbitrarily.
%\end{proof}


\begin{corollary}
	\label{cor:subset}
	% 
	Given a set of fake targets, $Y \subseteq \win_2(\game, F) \setminus F$ and a state $s \in \win_2(\game, F) \setminus F$, we have 
	\[
		\dswin_1(\emptyset, {Y}) \cup \dswin_1(\emptyset, {\{s\}}) \subseteq \dswin_1(\emptyset, {Y \cup \{s\}})
	\]
\end{corollary}
\begin{proof}[Proof (Sketch)]
	Follows immediately from Proposition~\ref{prop:or-composition} and  Alg.~\ref{alg:zielonka}. To see this, consider a P1 state $t \in \win_2(\game, F) \setminus F$ which is neither in $\dswin_1(\emptyset, {Y})$ nor in $\dswin_1(\emptyset, {\{s\}})$ but has exactly two transitions: one leading to $s$ and another leading to a state in $\dswin_1(\emptyset, {Y})$. Clearly, the new state will be added to $\dswin_{D \cup \{s\}}$. 
\end{proof}


Thus, if we consider the size of $\dswin_1(\emptyset, {Y})$ to be a measure of effectiveness of allocating the states in $D \subseteq \calD$ as decoys, then Corollary~\ref{cor:subset} states that the effectiveness of adding a new state to a set of decoys is greater than or equal to the sum of their individual effectiveness. In other words, $\dswin_1$ operator is \emph{superadditive} \cite{}. 


Let $\uplus$ represent the operation of composing two deceptive sure winning regions of P1. That is, given any subset $Y \subseteq \win_2(\game, F) \setminus F$ and a state $s \in \win_2(\game, F) \setminus F$,  
\[
\dswin_1(\emptyset, Y \cup \{s\}) =	\dswin_1(\emptyset, Y) \uplus \dswin_1(\emptyset, \{s\}).
\] 


With this notation, the problem of optimally placing the fake targets becomes equivalent to identifying a set $Y^\ast \subseteq \win_2(\game, F) \setminus F$ such that 
%
%
\begin{align}
	\label{eq:composition_opt}
	% 
	&Y^\ast = \argmax_{Y \subseteq \win_2(\game, F) \setminus F} \left| \biguplus\limits_{s \in Y} \dswin_1(\emptyset, \{s\}) \right|  \\
	&\quad \mbox{subject to: } \card{Y} \leq N \nonumber.
\end{align}
%
%
% ============================================================================================
% MOVE TO END OF SECTION.
% ============================================================================================
%\begin{remark}
%	Note that if we replace the composition operator $\uplus$ with the union operator $\cup$ in \eqref{eq:composition_opt}, then the problem becomes a maximum set-cover problem. 
%	\begin{align}
%		\label{eq:set-cover}
%		% 
%		&Y^\ast = \arg\max_{Y \subseteq \win_2(\game, F) \setminus F} \left| \bigcup\limits_{s \in D} \dswin_1(\emptyset, \{s\}) \right|  \\
%		&\quad \mbox{subject to: } \card{D}\le k \nonumber,
%	\end{align}
%	The maximum set-cover problem is well-studied submodular optimization problem, for which a $(1-1/e)$-approximate solution can be computed in polynomial time using a greedy algorithm \cite{vazirani_approximation_2003}. The solution to Eq.~\eqref{eq:set-cover} under-approximates the solution to Eq.~\eqref{eq:composition_opt}. However, it is not always possible to quantify or derive a bound on how close the under-approximation is. \ak{Nonetheless, this could be useful in practice as several optimization toolboxes include algorithms for maximum set-cover.}
%\end{remark}
% ============================================================================================


Let $g(Y) = \left| \biguplus\limits_{s \in Y} \dswin_1(\emptyset, \{s\}) \right|$ be a function that counts the number of P1's deceptive sure winning states when the set $Y \subseteq \win_2(\game, F)$ is allocated as fake targets. 


\begin{theorem} 
	\label{thm:dswinY-is-superadditive}
	The following statements are true. 
	\begin{enumerate}[(a)]
		\item $g$ is a monotone, non-decreasing, and superadditive function. 
		
		\item $g$ is submodular if, for all  $Y \subseteq S \setminus F$ and any $s \in S \setminus F$, we have $\dswin_1(\emptyset, Y) \cup \dswin_1(\emptyset, \{s\}) = \dswin_1(\emptyset, Y \cup \{s\})$. 
		
		\item $g$ is supermodular if, for all  $Y \subseteq S \setminus F$ and any $s_1, s_2 \in S \setminus F$ and $s_1 \neq s_2$, we have $\dswin_1(X, Y \cup \{s_1\}) \cap \dswin_1(X, Y \cup \{s_2\}) = \dswin_1(X, Y)$ 
	\end{enumerate}
\end{theorem}
\begin{proof}
	(\textbf{a}). Since for any set $Y \subseteq \win_2(\game, F) \setminus F$ and any state $s \in \win_2(\game, F) \setminus (F \cup Y)$, we have $\dswin_1(\emptyset, {Y}) \cup \dswin_1(\emptyset, \{s\}) \subseteq \dswin_1(\emptyset, Y \cup \{s\})$, $\dswin_1$ is a non-decreasing, monotone function. Consequently, $g$ is also a non-decreasing, monotone. The function $g$ is superadditive because, by Corollary~\ref{cor:subset}, $\dswin_1(\emptyset, {Y}) \cup \dswin_1(\emptyset, \{s\}) \subseteq \dswin_1(\emptyset, Y \cup \{s\})$.. Therefore, $g(Y) + g(\{s\}) \leq g(Y \cup \{s\})$.

	(\textbf{b}). When $\dswin_1(\emptyset, {Y \cup \{s\}}) = \dswin_1(\emptyset, {Y}) \cup \dswin_1(\emptyset, \{s\})$, we have $g(Y) = \left| \biguplus \limits_{s \in D} \dswin_{\{s\}} \right| = \left| \bigcup \limits_{s \in D} \dswin_{\{s\}} \right|$, which is submodular. 
	
	(\textbf{c}). The function $g$ is supermodular if and only if
	\begin{align*}
		g(Y \cup \{s_1\}) + g(Y \cup \{s_2\}) - g(Y) \leq g(Y \cup \{s_1, s_2\}).
	\end{align*}
	Given that $\dswin_1(\emptyset, Y \cup \{s_1\}) \cap \dswin_1(\emptyset, Y \cup \{s_2\}) = \dswin_1(\emptyset, Y)$ holds for any holds for any $Y \subseteq \win_2(\game, F)$ and any $s_1, s_2 \in \win_2(\game, F)$, the LHS counts every state in $\dswin_1(\emptyset, Y \cup \{s_1\}) \cup \dswin_1(\emptyset, Y \cup \{s_2\})$ exactly once. On the other hand, RHS counts the number of states in $\dswin_1(\emptyset, Y \cup \{s_1, s_2\})$. By Proposition~\ref{prop:or-composition}, we know that RHS may contain states that are neither in $\dswin_1(\emptyset, Y \cup \{s_1\})$ nor $\dswin_1(\emptyset, Y \cup \{s_2\})$. 
\end{proof}


%Theorem~\ref{thm:dswinY-is-superadditive} states that $g$ is a superadditive function when only fake targets are placed, and provides conditions under which $g$ is supermodular. In fact, the sum of two superadditive function is superadditive \cite{}. Therefore, we have the following corollary. 
%
%
%\begin{corollary}
%	Let $h(X, Y) = \left| \biguplus \dswin_1(X, Y) \right|$ be a function that counts the number of deceptive sure winning states when the subsets $X, Y$ of $\win_2(\game, F)$ are allocated as traps and fake targets respectively. Then, assuming fake targets are placed before traps, we can write $h(X, Y) = g(Y) + f_Y(X)$, where $f_Y(X)$ measures the size of $\dswin_1(X, Y)$ when a fixed set $Y$ is allocated as fake targets. 
%\end{corollary}


As of the time of writing this paper, the authors have not encountered any bounded approximation methods for maximizing a superadditive function that are applicable to Eq.~\ref{eq:composition_opt}. Therefore, we present Algorithm~\ref{alg:greedymax} that returns an $(1 - 1/e)$-approximate solution to Problem~\ref{prob:decoy-placement} when either condition (b) or (c) in Theorem~\ref{thm:dswinY-is-superadditive} is satisfied. This greedy algorithm is based on the GreedyMax algorithm for maximizing monotone submodular-supermodular functions in \cite{bai_greed_2018} and extends the algorithm discussed in \cite[Algorithm~1]{kulkarni2020decoy}. 


Algorithm~\ref{alg:greedymax} starts with empty sets of states $X$ and $Y$. It starts by iteratively constructing the set $Y$ through the incremental addition of a new fake target in each iteration. In every step, a new fake target $s$ is selected from the set of potential decoys $D$ such that its inclusion, along with the previously chosen fake targets, maximizes the coverage of P1's deceptive sure-winning region over the states in $\win_2(\game, F)$. The process continues until either a total of $N$ fake targets have been selected or the set of potential decoys is empty. Subsequently, the algorithm proceeds to the construction of $X$ using a similar procedure, where the set of fake targets $Y$ remains fixed, and a new trap is added to $X$ in each iteration.


\begin{algorithm}[tb]
	\begin{algorithmic}[1]
		\item[\textbf{Inputs:}] $\langle S, A, T, F \rangle$: Base game, $M$: Number of traps to placed, $N$: Number of fake targets to be placed.
		\item[\textbf{Outputs:}] $X, Y$: Near-optimal placement of traps and fake targets. 
		\State Initialize $X, Y$ to be empty sets. 
		\While {$N - |Y| > 0$}
			\State $D \gets \{v \in \win_2(\game, F) \mid v \notin (F \cup Y)\}$
			\If{$D$ is empty}
				\State Exit While
			\EndIf 
			\State Build a map $Z$ from state $s \in D$ to size of $\dswin_1(\emptyset, Y \cup \{s\})$.
			\State $d \gets \arg\max_{s \in D}{Z(s)}$ 
			\State Add $d$ to $Y$
		\EndWhile
		\While {$M - |X| > 0$}
			\State $D \gets \{v \in \win_2(\game, F) \mid v \notin (F \cup X \cup Y)\}$
			\If{$D$ is empty}
				\State Exit While
			\EndIf 
			\State Build a map $Z$ from state $s \in D$ to size of $\dswin_1(X \cup \{s\}, Y)$.
			\State $d \gets \arg\max_{s \in D}{Z(s)}$ 
			\State Add $d$ to $X$
		\EndWhile
		\State \Return $X, Y$
	\end{algorithmic}
	\caption{Greedy Algorithm for Decoy Placement}
	\label{alg:greedymax}
\end{algorithm}

==> sections/characterization.tex <==
\paragraph*{} The placement of traps and fake targets in $\game$ alters the winning region of each player as seen from their subjective views. Thus, we investigate the relation between winning regions of P1 and P2 in $\game$ and the respective winning regions in $\game_{X,Y}^1$ and $\game_{X,Y}^2$. 


\paragraph*{Notation.} We are concerned with three games: the base game, $\game$, P1's perceptual game (or true game) $\game_{X, Y}^1$, and P2's perceptual game, $\game_{X, Y}^2$. The symbols $X, Y$ are reserved to represent a set of traps and fake targets, respectively. We denote by $\win_i(\game_{X, Y}^j, F)$ to denote the winning region of player-$i$ in the perceptual game of player $j$, for $i, j \in  \{1, 2\}$. For simplicity, we write $\game_X^j, \game_Y^j$ to represent games in which only traps or only fake targets are placed. \deleted{The superscript $j$ is dropped when representing the winning regions in the base game. }\jf{there is no superscript for the base game.}

\jf{this notation $\win_i(\game_{X, Y}^j, F)$ 
 is not good. what does $F$ mean here? if it is the same for three games, can omit $F$. }
\paragraph*{Games with Only Traps.} We start by analyzing the case when only traps are allocated, \ie, $X \neq \emptyset$ and $Y = \emptyset$. The effect of traps on P2's perceptual game is captured by the following statement.


\begin{theorem}
	\label{thm:traps-p2-perceptual-win-regions}
	%
	In P2's perceptual game $\game_X^2$, we have $\win_1(\game_X^2, F) = \win_1(\game, F)$, and $\win_2(\game_X^2, F) = \win_2(\game, F)$. 
\end{theorem}
\begin{proof}
	From Definition~\ref{def:p2-perceptual-game}, it follows that, for any base game $\game$, we have $\game_{X}^2 = \game$. Hence, P1 and P2's winning regions are equal.
\end{proof}


\paragraph*{} In words, P2's perception of P1's and P2's winning regions is identical to the respective winning regions in the base game. This is because P2's perceptual game is identical to the base game without any decoys, as P2 is \replaced{unaware}{incapable of detecting} of traps \added{before the interaction}. In contrast, P1's perceptual game is the true game containing the decoys. In this game, P1 and P2's winning regions depend on whether the traps are placed within $\win_1(\game, F)$ or $\win_2(\game, F)$. 

\jf{replace the decoys in the above to ``traps'' because only traps are considered.}

\begin{theorem}
	\label{thm:traps-p1-perceptual-win-regions}
	%	
	The following statements hold true in any P1's perceptual game $\game^1_X$.
	\begin{enumerate}[(a)]
		\item If $X \subseteq \win_1(\game, F)$ then $\win_1(\game^1_X, F) = \win_1(\game, F)$ and $\win_2(\game^1_X, F) = \win_2(\game, F)$.
		
		\item If $X \subseteq \win_2(\game, F) \setminus F$ then $\win_1(\game^1_X, F) \supseteq \win_1(\game, F)$ and $\win_2(\game^1_X, F) \subseteq \win_2(\game, F)$.
	\end{enumerate}
\end{theorem}
\begin{proof}
	(a). Since $\win_1(\game_X^1, F) = \win_1(\game, F)$ is true whenever $\win_2(\game_X^1, F) = \win_2(\game, F)$ due to Fact~\ref{fact:determinacy}, we prove that latter statement. \jf{I don't get the sentence.  please clarify.}
	
	($\impliedby$). Consider any state $s \in \win_2(\game, F)$. Then, there exists a P2's sure winning strategy $\pi_2$ such that, for any P1 strategy $\pi_1$, the path $\rho = \mathsf{Outcome}(s, \pi_1, \pi_2)$ in $\game$ visits $F$. Notice that $\pi_2$ is also sure winning for P2 in $\game_X^1$ since $\rho$ is a valid path in $\game_X^1$. This is because, every state $s$ appearing in $\rho$ belongs to $\win_2(\game, F)$. Given that traps are allocated in $\win_1(\game, F)$, it follows that, for any state $t$ appearing in $\rho$, we have $T_X(t, \pi_2(t)) = T(t, \pi_2(t))$, by Definition~\ref{def:game-traps-faketargets}. Thus, $\rho$ must visit $F$ in $\game_X^1$. 
	
	($\implies$). By Fact~\ref{fact:determinacy}, $\win_2(\game_X^1) \subseteq \win_2(\game)$ is true if and only if $\win_1(\game_X^1, F) \supseteq \win_1(\game, F)$. We will prove the latter statement. Consider any state $s \in \win_1(\game, F)$. Then, P1 has a sure winning strategy $\pi_1$ such that, for any P2 strategy $\pi_2$, the path $\rho = \outcomes_{\game}(s, \pi_1, \pi_2)$ remains indefinitely within $\win_1(\game, F)$. Notice that $\pi_1$ is sure winning for P1 in $\game_X^1$. To see this, consider the path $\rho' = \outcomes_{\game_{X}^1}(s, \pi_1, \pi_2)$. We have two cases: (a) $\rho$ does not visit a state such that $t \in X$. Then, by Definition~\ref{def:game-traps-faketargets}, $\rho' = \rho$ because $T_X(t, \pi_1(t)) = T(t, \pi_1(t))$. (b) $\rho$ visits a state $t \in X$. Without loss of generality, let $t$ be the first trap visited by $\rho$. Clearly, $\rho'$ visits $t$. Then, $\rho'$ cannot visit $F$ because, by Definition~\ref{def:game-traps-faketargets}, $T_X(t, \pi_1(t)) = t$. 
	
	(b). Follows by similar reasoning as (a). 
\end{proof}

\jf{(b) is the interesting case right? maybe focus on the proof of (b). and give some intuition about your proof. right now it reads unclear, especially it is unclear what the $\leftarrow$, $\rightarrow$ try to show.}

\paragraph*{} In words, allocating traps in P1's winning region in $\game$ has no effect on either player's winning regions in P1's perspective (\ie, the true game). However, allocating them in P2's winning region expands the set of states from which P1 can surely satisfy its safety objective. Intuitively, this is because allocating a state $s \in S$ as a trap converts it to a sink state, thereby, \emph{cutting} any path $\rho$ that first visits $s$ and then $F$. 


\paragraph*{Games with Only Fake Targets.} Next, we consider allocation of fake targets and no traps. Because P2 misperceives the fake targets to contain valuable information but is unable to recognize them as decoys, the underlying graph of P2's perceptual game $\langle S, A, T\rangle$ is the same as the base game with no decoys. However, P2 perceives $F \cup Y$ to be final states instead of $F$. We analyze the effect of allocating fake targets in $\win_1(\game, F)$ and $\win_2(\game, F)$ separately. 


\begin{theorem}
	\label{thm:fakes-p1-perceptual-win-regions}
	%	
	Let $Y \subseteq \win_1(\game, F)$. The following statements hold in P1's perceptual game $\game^1_Y$ and P2's perceptual game $\game^2_Y$.
	\begin{enumerate}[(a)]
		\item $\win_1(\game^1_Y, F) = \win_1(\game, F)$ and $\win_2(\game^1_Y, F) = \win_2(\game, F)$.
		\item $\win_1(\game^2_Y, F \cup Y) \subseteq \win_1(\game, F)$ and $\win_2(\game^2_Y, F \cup Y) \supseteq \win_2(\game, F)$. 
	\end{enumerate}
\end{theorem}
\begin{proof}
	(a). Similar to Proposition~\ref{thm:traps-p1-perceptual-win-regions}(a).
	
	(b). Recall the property of sure winning regions that if $Z \subseteq Z'$ then $\win_2(\game, Z) \subseteq \win_2(\game, Z')$ where $Z, Z'$ represent P2's reachability objective \cite{}. The statement follows by observing that the games $\game$ and $\game_Y^1$ share the same underlying graph. 
\end{proof}


\paragraph*{} In words, the winning regions of both players in true game $\game_Y^1$ are the same as that in the base game $\game$. Note that statement (a) considers the winning region with final states $F$ since P1 is concerned with P2's ability to satisfy its true objective. The fake targets are viewed as additional final states in P2's perceptual game. Their addition does not eliminate any P2's winning strategy to visit $F$. However, in P2's perceptual game $\game_Y^2$, P2 may perceive its winning region to be larger than that in the base game due to presence of fake targets. The new states in P2's perceptual winning region are the ones from which P2 has sure winning strategy to visit $Y$ but not $F$. 

\jf{the last sentence needs a rigorous proof.}
%\paragraph*{} It is important to note that existence of a P2's sure winning strategy does not necessarily imply that P2 will always follow it. For example, consider a P2 state that has a transition leading into $F$ and a transition leading into $Y$. Clearly, the state is sure winning for P2, but since P2 cannot distinguish between $F$ and $Y$, P2 may choose either of the transitions. 

%In words, the winning regions of both players in true game $\game_Y^1$ are the same as that in the base game $\game$. However, P2 may perceive its winning region to be larger than that in the base game due to presence of fake targets. \deleted{As a result, P1 may get an advantage if it can enforce a visit to $\win_2(\game_Y^2, F \cup Y) \cap \win_1(\game, F)$, which is perceptually winning for P2 but truly winning for P1. In fact, from any state in $\win_2(\game_Y^2, F \cup Y) \cap \win_1(\game, F)$, P1 can not only guarantee satisfying its safety objective but also ensure a visit to $Y$. Such a strategy is valuable in applications such as cybersecurity where an attacker visiting a honeypot could help the defender learn about the attacker's identity, intention, etc. \cite{}.}


\paragraph*{} Now, consider the placement of fake targets in $\win_2(\game, F)$. 


\begin{theorem}
	\label{thm:fakes-p2-perceptual-win-regions}
	%	
	Let $Y \subseteq \win_2(\game, F) \setminus F$. The following statements hold in P1's perceptual game $\game^1_Y$ and P2's perceptual game $\game^2_Y$.
	
	\begin{enumerate}[(a)]
		\item $\win_1(\game^1_Y, F) \supsetneq \win_1(\game, F)$ and $\win_2(\game^1_Y, F) \subsetneq \win_2(\game, F)$.
		\item $\win_1(\game^2_Y, F \cup Y) = \win_1(\game, F)$ and $\win_2(\game^2_Y, F \cup Y) = \win_2(\game, F)$.
	\end{enumerate}
\end{theorem} 
\begin{proof}
	(a) Consider the statement $\win_1(\game^1_Y, F) \supsetneq \win_1(\game, F)$. Since fake targets are allocated in $\win_2(\game, F)$, for every state $s \in \win_1(\game, F)$ and any $a \in A$, we have $T_Y(s, a) = T(s, a)$. By an argument similar to Theorem~\ref{thm:traps-p1-perceptual-win-regions}, it follows that any sure winning strategy $\pi_1$ of P1 in $\game$ is also sure winning for P1 in $\game_Y^1$. Thus, $\win_1(\game^1_Y, F) \supseteq \win_1(\game, F)$. The strictness of relation is due to the fact that any fake target is sure winning for P1 in $\game_Y^1$. Using Fact~\ref{fact:determinacy}, we have $\win_2(\game^1_Y, F) \subsetneq \win_2(\game, F)$.
	
	(b) We will prove $\win_2(\game^2_Y, F \cup Y) = \win_2(\game, F)$. Using Fact~\ref{fact:determinacy}, it follows that $\win_1(\game^2_Y, F \cup Y) = \win_1(\game, F)$.
	
	($\impliedby$). Recall that $\game_Y^1$ and $\game$ share the same underlying graph $\langle S, A, T\rangle$. Since $F \cup Y \supseteq F$, it follows that $\win_2(\game^2_Y, F \cup Y) \supseteq \win_2(\game, F)$.
	
	($\implies$). By contradiction. Consider a state $s \in \win_2(\game^2_Y, F \cup Y)$ and suppose that $s \notin \win_2(\game, F)$. That is, $s \in \win_1(\game, F)$. By definition, there exists a sure winning strategy $\pi_1$ for P1 in $\game$ such that, for any P2 strategy $\pi_2$, the path $\rho = \outcomes_{\game}(s, \pi_1, \pi_2)$ remains indefinitely in $\win_1(\game, F)$. Since fake targets are allocated in $\win_2(\game, F)$, for every state $s \in \win_1(\game, F)$, we have $T_Y(s, a) = T(s, a)$ for any $a \in A$. Hence, by using $\pi_1$ in $\game_Y^1$, P1 can ensure that the game never visits $F \cup Y$---a contradiction. 	
\end{proof}


\paragraph*{} In words, placing traps in P2's sure winning region in $\game$ reduces the number of states from which P2 can achieve its true objective. However, in P2's perception, the presence of fake targets has no effect on the states that P2 perceives to be sure winning for itself. Thus, comparing the subset relations when $X \subseteq \win_2(\game, F)$ and $Y \subseteq \win_2(\game, F)$, the traps and fake targets appear to have a similar effect. This is not true. In fact, placing fake targets alters the winning strategy of P2. This observation allows us to prove a stronger result that \emph{fake targets are more powerful than traps}. 


\paragraph*{} To understand the effect of fake targets on P2's strategy, observe the rank of states that become winning for P2 when a subset $Z \subseteq \win_2(\game, F) \setminus F$ is allocated either as traps or as fake targets. First, we introduce a lemma.  


\begin{lemma} \label{lma:advantage-of-traps}
	Let $X \subseteq \win_2(\game) \setminus F$ be a set of traps. A strategy $\pi_1$ is sure winning for P1 in its safety objective in $\game^1_{X}$, \ie, to prevent the game from visiting $F$, if and only if $\pi_1$ is a sure winning strategy to visit $X$. 
\end{lemma}
\begin{proof}
	($\impliedby$). If $\pi_1$ is sure winning for P1 to visit $X$ from a state $s$, then for any strategy $\pi_2$, the path $\rho = \outcomes(s, \pi_1, \pi_2)$ visits $X$. But all states in $X$ are sink states in $\game_X^1$. Therefore, the path cannot visit $F$. Equivalently, $\pi_1$ is sure winning for P1 in its safety objective. 
	
	($\implies$). Since every state $s \in X$ is a sink state, there is no path from $s$ to $F$ in $\game_X^1$. Therefore, all states in $X$ are winning for P1 in $\game_X^1$. Thus, any sure winning strategy $\pi_1$ that visits $X$ from a state $s \in \win_2(\game)$ produces a path $\rho = \outcomes(s, \pi_1, \pi_2)$ that does not visit $F$, regardless of the sure winning strategy $\pi_2$ used by P2. In other words, $\pi_1$ is sure winning for P1 in its safety objective. 
\end{proof}


\paragraph*{} It is easy to see that the result from above lemma extends to fake targets as well. However, because of the difference in P2's perception of traps and fake targets, the set of states from which P1 has a sure winning strategy to visit a trap or a fake target is different. This intuition is illustrated in the following example. 


\begin{example}
	\label{ex:to-be-named}
	TODO. 
\end{example}

\begin{example}
	Consider the toy problem shown in Figure~\ref{fig:fake-betterthan-traps}. Suppose that we are given a single decoy placed at $s_0$. We are to decide whether it should be configured as a trap or a fake target. 
	
	\begin{figure}[tb!]
		\begin{center}
			\subfigure[Game with no fake targets.]{
				\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.5cm, scale = 0.4,transform shape]
					
					\node[state]              (0) [] {\Large $s_0$};
					\node[state, rectangle]   (1) [below left of=0] {\Large $s_1$};
					\node[state, rectangle]   (2) [below right of=0] {\Large $s_2$};
					\node[state, rectangle]   (3) [below left of=1] {\Large $s_3$};
					\node[state]              (4) [below right of=1] {\Large $s_4$};
					\node[state]              (5) [below right of=2] {\Large $s_5$};
					\node[state, rectangle, accepting] (6) [below right of=3] {\Large $s_6$};
					\node[state, accepting]   (7) [below left of=5] {\Large $s_7$};
					
					\path 
					(0) edge [bend left] node[above left=-5pt] 			{\Large $a_1$}  (1)
					(0) edge             node[above=2pt] 			 	{\Large $a_2$}  (2)
					(1) edge [bend left] node[above left=-5pt] 			{\Large $b_1$}  (0)
					(1) edge [bend left] node[above left=-5pt] 			{\Large $b_2$}  (3)        
					(1) edge             node[above right=-5pt] 		{\Large $b_3$}  (4)    
					(2) edge             node[above left=-5pt] 			{\Large $b_1$}  (4)        
					(2) edge             node[above right=-5pt] 		{\Large $b_2$}  (5) 
					(3) edge [bend left] node[above left=-5pt] 	  		{\Large $b_1$}  (1) 
					(3) edge             node[above right=-5pt] 		{\Large $b_2$}  (6) 
					(4) edge             node[above left=-5pt]  		{\Large $b_1$}  (6) 
					(4) edge             node[above right=-5pt] 		{\Large $b_2$}  (7) 
					(5) edge             node[above left=-5pt]  		{\Large $a_2$}  (7) 
					;
				\end{tikzpicture}
			}
			\hfill
			\subfigure[Game with fake target at $s_0$.]{
				\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3.5cm, scale = 0.35,transform shape]
					\node[state]              (0) [] {\Large $s_0$};
					\node[state, rectangle]   (1) [above left of=0] {\Large $s_1$};
					\node[state, rectangle, accepting] (6) [right of=0] {\Large $s_6$};
					\node[state, accepting]   (7) [right of=6] {\Large $s_7$};
					\node[state, rectangle]   (3) [right of=1] {\Large $s_3$};
					\node[state]              (4) [right of=3] {\Large $s_4$};
					\node[state]              (5) [right of=4] {\Large $s_5$};
					\node[state, rectangle]   (2) [above right of=3] {\Large $s_2$};
					
					\path 
					(0) edge [bend left] node[left] 			{\Large $a_1$}  (1)
					(0) edge [bend right, out=-10]            node[above=2pt, pos=0.1] 			 	{\Large $a_2$}  (2)
					(1) edge             node[above right=-5pt] 			{\Large $b_1$}  (0)
					(1) edge [bend left] node[above left=-5pt] 			{\Large $b_2$}  (3)        
					(1) edge [bend left, out=60] node[above right=-5pt] 		{\Large $b_3$}  (4)    
					(2) edge             node[above right=-5pt] 			{\Large $b_1$}  (4)        
					(2) edge             node[above right=-5pt] 		{\Large $b_2$}  (5) 
					(3) edge             node[above left=-5pt] 	  		{\Large $b_1$}  (1) 
					(3) edge             node[right] 		{\Large $b_2$}  (6) 
					(4) edge             node[above left=-5pt]  		{\Large $b_1$}  (6) 
					(4) edge             node[above right=-5pt] 		{\Large $b_2$}  (7) 
					(5) edge             node[above left=-5pt]  		{\Large $a_2$}  (7) 
					;
				\end{tikzpicture}
			}
		\end{center}
		\caption{A toy problem demonstrating how fake targets could be more effective than traps.}
		\label{fig:fake-betterthan-traps}
	\end{figure}
	
	First, note that all states in Figure~\ref{fig:fake-betterthan-traps} are winning for P2 in its objective to reach $F = \{s_6, s_7\}$. Using Algorithm~\ref{alg:zielonka}, the level sets are determined to be $[\{s_6, s_7\}, \{s_3, s_4, s_5\}, \{s_1, s_2\}, \{s_0\}]$ where the final states are assigned the lowest rank $0$ and $s_0$ is assigned the highest rank $3$. 
	
	When $s_0$ is configured as a trap, the only P2 state that becomes winning for P1 is $s_0$. However, when it is configured as a fake target, the states $s_0$ and $s_1$ become winning for P1. This is because when $s_0$ is a fake target, it is considered a final state in $\game_Y^2$. Hence, it's rank becomes $0$. The rank of P2 state $s_1$ becomes $1$ because P2 can reach from $s_1$ to $s_0$ in one-step using action $b_1$. As a result, in P2's perception, the action $b_1$ is subjectively rationalizable but action $b_2$ (which is truly a rational action) is not, since, by using $b_2$, it would take two-steps to visit $F$. 
	
	It is noted that the state $s_3$ from which P2 has a strategy to surely visit $s_0$ is not subjectively rationalizable for P2 in its perceptual game. Again, this is because it can visit the final state $s_6$ in one-step using $b_2$, whereas it would take two-steps to visit $s_0$. \qed
	\aknote{To be restructured.}
\end{example} 
\jf{this example is problematic. It assumes action $b_1$ is subjective rationalizable but $b_2$ is not because it takes two steps. However, both actions should be subjective rationalizable. there is no optimality considered for the number of steps required to reach the goal.}

\jf{all theorems are stated first and the intuition/implication explained later. Reverse the order. Otherwise the reader is not motivated to read your proofs. }

\jf{I don't know why the following proposition is interesting or how to interpret the meaning?}
\begin{proposition}
	\label{prop:traps-rank-of-p1-winner} 
	%	
	Given a set of traps $X \subseteq \win_2(\game, F)$, let $s \in \win_2(\game, F)$ be a state from which P1 has a sure winning strategy to  visit $X$. Then, $\rank(s) > \min \{\rank(t) \mid t \in Y\}$. 
\end{proposition}
\begin{proof}[Proof (Sketch)]
	By contradiction. Suppose there exists a state $s \in \win_2(\game, F)$ such that P1 has sure winning strategy $\pi_1$ to visit a trap in $X$ whose rank is at least equal to $\rank(s)$. Thus, for any P2's sure winning strategy $\pi_2$, there must exist a rank-increasing transition in the path $\rho = \outcomes(s, \pi_1, \pi_2)$. By definition of attractor \cite{}, if $s$ is a P1 state, then every action from $s$ is rank reducing. If $s$ is a P2 state, then a rational P2 will follow a sure winning strategy to visit $F$, which, at any state, chooses a rank reducing action. Hence, a rank-increasing transition cannot occur---a contradiction. 
\end{proof}


\paragraph*{} It is easy to see that if the states in $X$ in Proposition~\ref{prop:traps-rank-of-p1-winner} were to be allocated as fake targets instead, P1 could use the same sure winning strategy at $s$ to visit a fake target. But, as Example~\ref{ex:to-be-named} demonstrates, it is also possible that P1 may guarantee a visit to a fake target from a state with a lower rank than the fake target. This is because setting a state as fake target makes it a rank $0$ state in $\game_Y^2$. Hence, we have the following result.

\jf{this raises the same problem to the previous comments and I am not convinced that the statement holds. i will stop here for now.}
\begin{theorem}
	\label{thm:traps-fakes-subset-relation}
	For any $Z \subseteq \win_2(\game, F) \setminus F$, we have $\win_1(\game) \subseteq \win_1(\game_{Z, \emptyset}^1, F) \subseteq \win_1(\game_{\emptyset, Z}^1, F \cup Z)$.
\end{theorem}


==> sections/deception.tex <==
\paragraph*{} In this subsection, we show how to synthesize a stealthy deceptive strategy for P1 given a fixed set of decoys based on results from Section~\ref{sec:characterization}. Using this strategy, P1 can enforce a visit to a decoy while preventing P2 to become aware of its misperception.


\paragraph*{} Consider the case when a set of decoys $X \cup Y$ containing traps $X$ and fake targets $Y$ is placed in $\win_2(\game, F) \setminus F$. By Lemma~\ref{lma:advantage-of-traps}, P1 can enforce a visit to $X \cup Y$ from a state $s \in \win_2(\game, F) \setminus (F)$ if and only if P1 has a strategy to surely visit $X \cup Y$ from $s$. However, we cannot compute such a strategy by simply solving the following reachability game: $$\langle S, A, T_{X \cup Y}, X \cup Y \rangle,$$ where $X \cup Y$ is P1's reachability objective and $T_{X \cup Y}(s, a) = T(s, a)$ if and only if $T(s, a) \in \win_2(\game, F)$. Otherwise, ${T}_{X \cup Y}(s, a)$ is undefined. The following example demonstrates why this intuition is incorrect. 


\begin{example}
	Consider the game shown in Fig.~\ref{fig:inverted-jobstmann-example}, in which P1 and P2 states are represented by circle and square states, respectively. P2's goal is to reach $F = \{3, 4\}$ shown as accepting states. Using Alg.~\ref{alg:zielonka}, we obtain $\win_1 = \{1, 2\} $ and $\win_2 = \{0, 3, 4, 5, 6, 7\}$. Particularly, the attractor level set obtained is $[\{3, 4\}, \{0\}, \{7\}, \{6\}, \{5\}]$, where the level-$0$ of attractor contains the final states, level-$1$ contains state $0$ and so on. The sure winning strategy at any P2 state in $\win_2$ is the action that reduces the level of attractor. Therefore, $\pi_2(0) = (0, 3)$ and $\pi_2(6) = (6, 7)$.
	
	\begin{figure}
		\centering 
		\include{figures/inverted-jobstmann}
		\caption{TODO. }
		\label{fig:inverted-jobstmann-example}
	\end{figure}
	
	Suppose that P1 allocates a trap at state $0$ (colored red). Without the trap, from state $7$, P2 was guaranteed to visit $F$ because, if P1 chose $(7, 3)$ then a final state was visited immediately and if P1 chose $(7, 0)$ then P2 could choose $(0, 3)$ at state $0$ to visit $F$. However, when trap is allocated at $0$, P1 can choose $(7, 0)$ at state $7$ to enforce a visit to a trap, thereby achieving its safety objective. 
	
	Now, consider state $6$. Following Lemma~\ref{lma:advantage-of-traps}, if we were to use Alg.~\ref{alg:zielonka} to compute the sure winning region of P1 with $X = \{0\}$ as final states, then P1's winning region would be $\{0, 7\}$. This is because, at state $6$ in $\game_{X}^1$, there exists a self-loop action using which P2 can prevent the game from reaching $0$. But, since the self-looping action $(6, 6)$ is not a rank-reducing action for P2 in $\game$, P2 will never use $(6, 6)$ at state $6$. If $(6, 6)$ is eliminated from P2's available actions at state $6$, then $6$ becomes a sure winning state for P1 to visit the trap state $0$. 
	\qed
	\aknote{I will develop a running example to jointly illustrate allocation of fakes and traps. This example is just for traps.}
\end{example}


\paragraph*{} Formally, the action $(6, 7)$ at state $6$ in Fig.~\ref{fig:inverted-jobstmann-example} as a \emph{subjectively rationalizable} action for P2. This is because in P2's perceptual game, the action is rational. Whereas, the self-loop $(6, 6)$ is not subjectively rationalizable at $6$. Interested readers are referred to \cite{} for an elaborate discussion on subjective rationalizability for hypergames. 


\paragraph*{} Given any state $s \in S$, let $\rank_{X, Y}^i(s)$ denote the rank of state $s$ in the game $\game_{X, Y}^i$, $i = 1, 2$. 


\begin{definition}[Subjectively Rationalizable Actions]
	\label{def:sracts}
	% 
	Given P2's perceptual game $\game^2_{X, Y}$, an action $a \in A_2$ is said to be \emph{subjectively rationalizable} at a state $s \in S_2 \cap \win_2(\game_{X, Y}^2)$ if and only if the state $s' = \Delta(s, a)$ satisfies $\rank_{X, Y}^2(s') < \rank_{X, Y}^2(s)$. Every action at a P1 state $s \in S_1 \cap \win_2(\game_{X, Y}^2)$ is subjectively rationalizable for P2. The set of subjectively rationalizable actions at any state $s \in \win_2(\game_{X, Y}^2)$ is denoted by $\srAct(s)$. 
\end{definition}


\paragraph*{} A strategy is said to be \emph{subjectively rationalizable} if it maps any state to a subset of subjectively rationalizable actions at that state.


\paragraph*{} We now define a zero-sum game on graph representing $\hgame_1$ that P1 solves to compute its strategy in the L2-hypergame, $\hgame_2$.


\begin{definition}
	\label{def:hgame-labeling-misperception}
	% 
	Given the hypergame $\hgame_2$, the hypergame on graph $\hgame_1$ is the following game on graph in which P1 has a reachability objective.
	\[
	\widehat \hgame_1(X, Y)  = \langle S, A, \widehat T_{X, Y}, X \cup Y \rangle,
	\]
	where 
	\begin{itemize}
		\item $S$ is a set of game states, same as $\game$.
		
		\item $\widehat T_{X, Y}: S \times A  \rightarrow S$ is a \emph{deterministic} transition function such that, for any state $s \in \win_2(\game, F)$, $\widehat T_{X, Y}(s, a) = T(s, a)$ if and only if $a \in \srAct(s)$. Otherwise, $\widehat{T}_X(s, a)$ is undefined. 
		
		\item $X \cup Y \subseteq \win_2(\game, F) \setminus F$ is the set of states representing P1's reachability objective.  
	\end{itemize}	
\end{definition}
%\aknote{(Internal) We define the $\widehat{\hgame}_1(X, Y)$ over $S$ because P2 may be incentivized to visit $\win_1(\game, F)$ by allocating $Y \subseteq \win_1(\game, F)$.}


\paragraph*{} It is noted that the set $X$ in $\widehat{\hgame}_1(X, Y)$ defines P1's reachability objective, not P2's objective.

%\replaced{REPLACE THIS!}{Intuitively, $\widehat{\hgame_1}$ only considers P2's winning states $\win_2(\game)$ because, following Proposition~\ref{prop:traps-p1-perceptual-win-regions}, we know that only a subset of $\win_2(\game)$ can be turned into P1's winning states by allocating traps. The transition function eliminates P2's actions that are not subjectively rationalizable.  }


\begin{theorem}
	\label{thm:trap-effect}
	%		
	Given a state $s \in \win_2(\game, F) \setminus F$, let $\pi_2$ be any subjectively rationalizable, sure winning strategy of P2 to visit $F \cup Y$. Then, a P1 strategy $\pi_1$ ensures a visit to $X \cup Y$ if and only if $\pi_1$ is a sure winning strategy for P1 in $\widehat{\hgame}_1$.
\end{theorem}


\paragraph*{} Theorem~\ref{thm:trap-effect} is true by construction. To see this, first, recall that a sure winning strategy of P1 ensures satisfaction of P1's reachability objective against every possible strategy choice of strategy by P2. And, notice that the set of all P2 strategies in the hypergame $\widehat{\hgame}_1(X, Y)$ is equal to the set of all subjectively rationalizable strategies of P2 in $\game_{X, Y}^1$. 

%To see this, recall that a sure winning strategy of P1 ensures satisfaction of P1's reachability objective against every possible strategy choice of strategy by P2. In the hypergame $\widehat{\hgame}_1(X, Y)$, the set of all P2 strategies is equal to the set of all subjectively rationalizable strategies of P2 in $\game_{X, Y}^1$. And, the set of all P1 strategies is equal to the set of all subjectively rationalizable strategies of P1 in $\game_{X, Y}^1$.


\paragraph*{} Since P1's sure winning strategy in $\widehat \hgame_1(X, Y)$ enforces a visit to $X \cup Y$ by leveraging P2's misinformation, it is called P1's \emph{sure winning strategy under deception}, for short, \emph{deceptive sure winning strategy}. The strategy is \emph{stealthy} because it always selects an action that is subjectively rationalizable in P2's view. Thus, P2 cannot become aware of deception. The sure winning region of P1 in $\widehat \hgame_1(X, Y)$ is called the \emph{deceptive sure-winning region}, denoted $\dswin_1(X, Y)$. % It is easy to see that every state from which P1 can surely win without deception is also a state in P1's deceptive winning region, \ie, $\win_1(\game_{X, Y}^1, F) \subseteq \dswin_1(X, Y)$.


\paragraph*{} Next, we characterize the set of states from which P2 has a strategy to visit $F$ regardless of whether P1 uses deception. From these states, any subjectively rationalizable P2 strategy must avoid visit $X \cup Y$. We call such a P2 strategy as \emph{sure winning strategy of P2 under deception}, or abusing the notation slightly, P2's deceptively sure winning strategy.

%For this, we identify the states from which every subjectively rationalizable, sure winning strategy of P2 induces a visit to $F$ without visiting $X \cup Y$. Such a strategy is called a \emph{sure winning strategy of P2 under deception}, for short, P2's deceptively sure winning strategy. 


%Given P1's deceptive sure winning region, next, we want to characterize the set of states from which P2 can surely visit $F$ regardless of P1 using deception. Since $\widehat{\hgame}_1(X, Y)$ is an instance of Definition~\ref{def:game}, due to Fact~\ref{fact:determinacy}, P2 has a sure winning strategy from every state in $\win_2(\game) \setminus \dswin_1$. However, due to misperception, P2 might follow a strategy that is not sure winning. This is because P2 does not know $\widehat{\hgame}_1(X, Y)$. In this case, we say a state is deceptively sure winning for P2 if and only if every subjectively rationalizable strategy of P2 from that state is also a rational strategy in the true game.


\begin{proposition}
	\label{prop:traps-dswin2}
	%  
	Given any state $s \in \win_2(\game, F) \setminus F$, P2 has a deceptive sure winning strategy to visit $F$ from $s$ if and only if, for any pair of P1 and P2 strategies $\pi_1, \pi_2$, the path $\rho = \outcomes(s, \pi_1, \pi_2)$ in $\widehat{\hgame}_1(X, Y)$ does not visit $X \cup Y$. 
\end{proposition}
\begin{proof}[Proof (Sketch)]
	Let $\Pi^{SR}(\game^2)$ be the set of subjectively rationalizable strategies in $\game^2$. Given any pair of strategies $\pi_2, \pi_2' \in \Pi^{SR}(\game^2)$, P2 has no incentive to choose $\pi_2$ over $\pi_2'$, or vice versa, because, in P2's perspective, starting from state $s$, both of them visit $F$ in at most $\rank_{X, Y}^2(s)$ steps. As a result, there exists a possibility that P2 chooses $\pi_2$ even if the resulting path $\rho = \outcomes(s, \pi_1, \pi_2)$, when P1 follows $\pi_1$ and P2 follows $\pi_2$, visits a state in $X \cup Y$ before visiting $F$. Noting that the set of all P2 strategies in $\widehat{\hgame}_1(X, Y)$ is equal to $\Pi^{SR}(\game^2)$, the states from which P2 is ensured to visit $F$ without visiting $X \cup Y$ are the states that are disconnected from $X \cup Y$ in the underlying graph of $\widehat{\hgame}_1(X, Y)$. 
%		Given a set of subjectively rationalizable strategies at $s$, P2 has no incentive to choose any given strategy over the another because, in P2's perspective, all of them visit $F$. Therefore, if there exists a subjectively rationalizable strategy $\pi_2^*$ that induces a visit to $X \cup Y$, then there exists a possibility that P2 selects $\pi_2^*$. Thus, the states from which P2 is ensured to visit $F$ are those that are disconnected from $X \cup Y$ because every strategy at a state $s \in \win_2(\game, F) \setminus F$ in $\widehat{\hgame}_1(X, Y)$ is subjectively rationalizable, by construction. 
\end{proof}


\paragraph*{} It follows that $\widehat{\hgame}_1$ is \emph{not} determined. That is, from any state $s \in \win_2(\game, F) \setminus F$ which is connected to $X \cup Y$, the winner of the game can only be determined after players fix their strategies.


\paragraph*{} Finally, we consider the case where the decoys $X \cup Y$ are placed in $\win_1(\game, F)$. 
\begin{proposition}
	\label{prop:decoy-in-win1-benefit}
	If $X \cup Y \subseteq \win_1(\game, F)$, then $\dswin_1(X, Y) = \win_1(\game_{X, Y}^1, F) =  \win_1(\game, F)$. 
\end{proposition}
\begin{proof}
	By Theorem~\ref{thm:traps-p1-perceptual-win-regions}, \ref{thm:fakes-p1-perceptual-win-regions}. 
\end{proof}


\paragraph*{} Proposition~\ref{prop:decoy-in-win1-benefit} states that P1 gains no benefit by placing decoys in $\win_1(\game, F)$. However, for similar reason as Proposition~\ref{prop:decoy-in-win1-benefit}, such a placement reduces the size of P2's deceptive winning region. 

%Although P1 placing decoys in $\win_1(\game, F)$ does not affect sure winning region of P1, it shrinks the states from which P2's deceptive winning region. Again, this is a consequence of non-determinacy of $\widehat{\hgame}_1(X, Y)$.

\begin{proposition}
	If $X \cup Y \subseteq \win_1(\game, F)$, then $\dswin_2(X, Y) \subseteq \win_2(\game_{X, Y}^1, F)$. 
\end{proposition}


%\paragraph*{} Similar to Proposition~\ref{prop:traps-dswin2}, notice that any strategy that visits $Y$ is subjectively rationalizable for P2. Thus, there is a possibility that P2 may choose such a strategy.



%\paragraph*{} In conclusion, the partition of state space of a L2-hypergame in Definition~\ref{def:generalized-hypergame} can be represented as shown in Fig.~\ref{fig:hgame-partition}. 




==> sections/effectsOfDecoy.tex <==
Recall that by placing traps P1 can manipulate the structure of game as perceived by P2, whereas by placing fake targets P1 can manipulate the structure of game and the objective of P2 in its perceptual game. In this subsection, we investigate how the placement of traps and fake targets affects the winning regions and strategies of players in P1 and P2's perceptual games when compared to those in the base game. 

\jf{I am not sure about the word ``manipulate''--- maybe we shall change it to the following. ``By placing traps, P1 can change the game transition dynamics without P2 knowing the changes. By placing fake targets, P1 can change the objective perceived by P2. ...''} 


\paragraph*{Effect on P1's Perceptual Game.} The introduction of any type of decoy within P1's winning region in the base game, $\game$, does not alter the winning regions of the players in P1's perceptual game, $\game_{X, Y}^1$. This is due to the fact that every state within the winning region $\win_2(\game, F)$ remains a guaranteed winning state for P2 in $\game_{X, Y}^1$, as the placement of decoys within $\win_1(\game, F)$ does not eliminate any winning strategies available to P2 from states within $\win_2(\game, F)$.
\jf{The above paragraph is confusing. Do you mean that if a state is winning for P1 in the original game, placing a trap or fake target at that state will not help to increase P1's winning set? It is easy to see for the case of the trap. What about fake target? it is not easy to see so. }

On the contrary, when traps or fake targets are placed in P2's winning region, $\win_2(\game, F)$, some of P2's sure winning states in $\game$ become sure winning for P1 in $\game_{X, Y}^1$. This is because the states in $X \cup Y$ become sink states in $\game_{X, Y}^1$. Moreover, any state in $\win_2(\game, F) \setminus F$ from which P1 has a sure winning strategy to visit $X \cup Y$ also becomes sure winning for P1 in $\game_{X, Y}^1$. The following lemma describes the condition for a state in $\win_2(\game, F) \setminus F$ to become sure winning for P1 in $\game_{X, Y}^1$. 
% In addition, given a state $s \in \win_2(\game, F)$, if there exists a strategy $\pi_1$ of P1 such that, for any sure winning strategy $\pi_2$ of P2, the path $\rho = \outcomes(s, \pi_1, \pi_2)$ visits $X \cup Y$ before visiting $F$, then $s$ is sure winning state for P1 in $\game_{X, Y}^1$. These observations are formalized in the following lemma and proposition. 


\begin{lemma} 
	\label{lma:effect-on-p1-decoys-in-win2}
	Let the set $X \cup Y \subseteq \win_2(\game, F) \setminus F$ be allocated as traps and fake targets. Given a state $s \in \win_2(\game, F) \setminus F$, a strategy $\pi_1$ is sure winning for P1 at state $s$ in the game $\game^1_{X, Y}$ if and only if $\pi_1$ is a sure winning strategy for P1 at $s$ to visit $X \cup Y$. 
\end{lemma}
\begin{proof}
	($\implies$). Given that $\pi_1$ is sure winning in $\game_{X, Y}^1$ to prevent a visit to $F$, we want to establish that $\pi_1$ is sure winning in $\game_{X, Y}^1$ to visit $X \cup Y$. Since $s$ is P2's sure winning state in $\game$, consider any sure winning strategy $\pi_2$ at $s$. Then, the path $\rho = \outcomes_\game(s, \pi_1, \pi_2)$ must visit $F$ in $\game$. Consider the path $\rho' = \outcomes_{\game_{X, Y}^1}(s, \pi_1, \pi_2)$. If $\rho$ does not visit any state in $X \cup Y$, then, by Definition~\ref{def:p1-perceptual-game}, we have $\rho' = \rho$, which violates the given information. The only other case is that $\rho$ visit some state in $X \cup Y$, in which case, $\rho'$ visits a sink state in $X \cup Y$ and therefore does not visit $F$. 

	($\impliedby$). Given that $\pi_1$ is sure winning in $\game_{X, Y}^1$ to visit $X \cup Y$, we want to establish that $\pi_1$ is sure winning in $\game_{X, Y}^1$ to prevent a visit to $F$. Since every state $t \in X \cup Y$ is a sink state, there is no path from $t$ to $F$ in $\game_X^1$. Therefore, all states in $X \cup Y$ are winning for P1 in $\game_X^1$. By definition, every path $\rho = \outcomes(s, \pi_1, \pi_2)$ visits $X \cup Y$ for any P2 strategy $\pi_2$. Therefore, the game cannot visit $F$. 
\end{proof}


A key insight from Lemma~\ref{lma:effect-on-p1-decoys-in-win2} is that decoys \emph{cut the winning paths} passing through them when placed in $\win_2(\game, F)$. The following proposition describes the effect of decoys on P1's perceptual game. 


\begin{proposition}[Effect of Decoys on P1's Perceptual Game]
	\label{prop:effect-on-p1}
	Given the base game $\game$, the following statements are true about P1's perceptual game, $\game_{X, Y}^1$. 
	\begin{enumerate}[(a)] 
		\item If $X \cup Y \subseteq \win_1(\game, F)$ then $\win_1(\game_{X, Y}^1, F) = \win_1(\game, F)$. 
		\item If $X \cup Y \subseteq \win_2(\game, F) \setminus F$ then $\win_1(\game_{X, Y}^1, F) \supsetneq \win_1(\game, F)$. 
	\end{enumerate}
\end{proposition}
\begin{proof}
	In Appendix~\ref{}. 
\end{proof}


Next, we study the effect of placing decoys on P2's perceptual game, $\game_{X, Y}^2$. It is easy to see from Remark~\ref{rmk:p2-game-is-base-game} that placing traps anywhere in $\game$ does not affect P2's perception of players' winning regions or strategies. However, placing the fake targets within P1's winning region in $\game$, some of P1's sure winning states in $\game$ are perceived to be sure winning for P2 in $\game_{X, Y}^2$. This is obvious because P2 misperceives the subset $Y$ of P1's winning region in $\game$ to be `goal' states in $\game_{X, Y}^2$. As a result, any state $s \in \win_1(\game, F)$ from which P2 has a sure winning strategy to visit $F \cup Y$ is also perceived to be sure winning for itself by P2 in $\game_{X, Y}^2$. On the contrary, placing the fake targets within P2's winning region in $\game$ has no effect on perceived winning regions of players in $\game_{X, Y}^2$. This is because every state in $\win_2(\game, F)$ is also sure winning for P2 $\game_{X, Y}^2$ due to Remark~\ref{rmk:p2-game-is-base-game}. And, placing of fake targets in $\win_2(\game, F)$ does not affect P1's sure winning strategy at any state in $\win_1(\game, F)$. Altogether, the effect of decoys on P2's perceptual game is captured by following proposition.


\begin{proposition}[Effect of Decoys on P2's Perceptual Game]
	\label{prop:effect-on-p2}
	Given the base game $\game$, the following statements are true about P2's perceptual game, $\game_{X, Y}^2$. 
	\begin{enumerate}[(a)] 
		\item If $X \subseteq S \setminus F$ and $Y \subseteq \win_1(\game, F)$, then $\win_2(\game_{X, Y}^2, F \cup Y) \supsetneq \win_2(\game, F)$.
		\item If $X \subseteq S \setminus F$ and $Y \subseteq \win_2(\game, F)$, then $\win_2(\game_{X, Y}^2, F \cup Y) = \win_2(\game, F)$
	\end{enumerate}
\end{proposition}
\begin{proof}
	In Appendix~\ref{}. 
\end{proof}


Propositions~\ref{prop:effect-on-p1} and \ref{prop:effect-on-p2} provide important insights to solve Problem~\ref{prob:decoy-placement}. They suggest that traps could be beneficial to P1 when they are placed within $\win_2(\game, F)$, whereas fake targets could be beneficial when they are placed anywhere in $S \setminus F$. Specifically, when fake targets are placed in $\win_2(\game, F)$, they behave like traps and \emph{cut the winning paths}. However, when placed in $\win_1(\game, F)$, fake targets might induce P2 to visit a state in $\win_1(\game, F)$, from which, by Proposition~\ref{prop:effect-on-p1}, P1 has a sure winning strategy to prevent a visit to $F$. % Interestingly, in the next subsection, we show that placing fake targets in $\win_1(\game, F)$ does not help P1 to convert any of P2's sure winning states in $\game$ to its sure winning states (see Proposition~???) 


\paragraph*{Effect on P2's Strategy.} Since the presence of traps does not affect P2's perception, they have no effect on P2's strategy. Whereas, inclusion of fake targets may introduce spurious strategies into the set of strategies perceived by P2 as sure winning for itself in $\game_{X, Y}^2$. These strategies might actually induce a visit to a sure winning state of P1 in the true game, $\game_{X, Y}^1$. An interesting effect on P2's strategy is observed when fake targets are placed in $\win_2(\game, F)$.


\begin{example}
	\ak{Need an example that illustrates the effect of fake in P1's winning region as well.}
	\qed
\end{example}


\ak{placeholder: An important lesson from the above example is that, even though placing traps and fake targets in $\win_2(\game, F)$ do not affect the size of winning region in $\game_{X, Y}^2$, the rank of a state in $\win_2(\game, F)$ may be different from its rank in $\win_2(\game_{X, Y}^2, F \cup Y)$. Therefore, P2's sure winning strategy at the same state in $\game$ and $\game_{X, Y}^2$ could be different.} This observation will help us establish an important result in Section~\ref{subsec:allocation} that \emph{fake targets can be more advantageous than traps}.  


%\begin{theorem}
%	\label{thm:traps-fakes-subset-relation}
%	For any $Z \subseteq \win_2(\game, F) \setminus F$, we have $\win_1(\game) \subseteq \win_1(\game_{Z, \emptyset}^1, F) \subseteq \win_1(\game_{\emptyset, Z}^1, F \cup Z)$.
%\end{theorem}
%\begin{proof}
%	The relation $\win_1(\game) \subseteq \win_1(\game_{Z, \emptyset}^1, F)$ is true by Proposition~\ref{prop:effect-on-p1}. To see why $\win_1(\game_{Z, \emptyset}^1, F) \subseteq \win_1(\game_{\emptyset, Z}^1, F \cup Z)$ is true, consider a state $s \in \win_2(\game, F)$ from which P1 can surely visit $Z$ in $\game_{Z, \emptyset}^1$. We will show that $s$ is sure winning for P1 to visit $Z$ in $\game_{\emptyset, Z}^1$. 
%	
%	Since $s$ is sure winning for P1 to visit $Z$ in $\game_{Z, \emptyset}^1$, there exists a P1 strategy $\pi_1$ such that, for any sure winning strategy $\pi_2$ of P2 to reach $F$, every path $\rho = s_0 s_1 s_2 \ldots = \outcomes(s, \pi_1, \pi_2)$ with $s_0 = s$ visits $Z$ before visiting $F$. Furthermore, for every $i \geq 0$, it holds that $\rank(s_{i+1}) < \rank(s_i)$. 
%	
%	Now, consider the game $\game_{\emptyset, Z}^1$. The rank of all states in $Z$ is $0$, by definition. As illustrated in Example~\ref{}, the ranks of other states in $\win_2(\game_{\emptyset, Z}^2, F \cup Z)$ may undergo changes. Nonetheless, from Proposition~\ref{prop:effect-on-p2}, we know that all P2's sure winning states within $\win_2(\game, F)$ remain winning for P2 within $\win_2(\game_{\emptyset, Z}^2, F \cup Z)$, although the winning strategies employed by P2 at those states may differ. This gives rise to two cases:
%	
%	(a) The set of P2's sure winning strategies in $\game_{Z, \emptyset}^1$ at any state $s_i \in S_2$ appearing in $\rho$ is equal to the set of P2's sure winning strategies at $s_i$ in $\game_{\emptyset, Z}^2$. Then, by definition, $\pi_1$ is also sure winning for P1 to visit $Z$ in $\game_{\emptyset, Z}^2$. 
%	
%	(b) There exists a P2 state $s_i$ appearing in $\rho$ for which there exists a sure winning strategy $\pi_2'$ in $\game_{\emptyset, Z}^2$ such that $\pi_2'(s_i) = s_{i+1}' \neq s_{i+1}$. That is, $\rank(s_{i+1}') < \rank(s_i)$ in $\game_{\emptyset, Z}^2$, which was not the case in $\game$. This means that P2 has a strategy to visit $F \cup Z$ in at-most steps $\rank(s_{i+1}')$-many steps. Since addition of fake targets does not add any new path from $s_{i+1}'$ to $F$, the reduction of rank of $s_{i+1}'$ must be because, in $\game_{\emptyset, Z}^2$, P2 has a strategy to visit $Z$ in $\rank(s_{i+1}')$-many steps. Therefore, the game is ensured to visit $Z$ in $\win_2(\game_{\emptyset, Z}^2, F \cup Z)$. This concludes the proof.
%\end{proof}



%
%\hrule 
%
%
%The overall effect of placing a mixture of traps and fake targets can be understood by studying the effects of placing only traps and only fake targets. We start by analyzing the effect of placing traps and fake targets on P1's perceptual game, $\game_{X, Y}$. 
%
%
%
%The overall effect of placing a mixture of traps and fake targets can be understood by studying the effects of placing only traps and only fake targets. We start by analyzing the case when only traps are allocated, \ie, $X \neq \emptyset$ and $Y = \emptyset$. For convenience, we will write the game $\game_{X, \emptyset}$ as $\game_X$ with an understanding that $Y = \emptyset$.
%
%
%Consider the case when the traps are placed in P2's winning region in the base game $\game$, \ie, $X \subseteq \win_2(\game, F)$. Such a placement increases the number of states from where P1 can surely prevent P2 from visiting $F$. To see this, first observe that P2 cannot win from any state in $X$. Moreover, since the states in $X$ become `sink' states, any winning path of P2 in $\game$ that visits a state in $X$ before visiting $F$, will become winning for P1 in the true game $\game_X^1$. Hence, if there exists a strategy $\pi_1$ for P1 such that all paths $\rho = \outcomes(s, \pi_1, \pi_2)$ starting from a state $s \in \win_2(\game, F)$ visit $X$ before visiting $F$ for any P2's sure winning strategy $\pi_2$ in $\game_X^2$, then the P2's sure winning state $s$ in $\game$ would become sure winning for P1 in $\game_X^1$. This intuition is formalized in the following statement. 
%
%
%\begin{lemma} \label{lma:advantage-of-traps}
%	Let $X \subseteq \win_2(\game, F) \setminus F$ be a set of traps. A strategy $\pi_1$ is sure winning for P1 in $\game^1_{X}$ to prevent the game from visiting $F$, if and only if $\pi_1$ is a sure winning strategy to visit $X$. 
%\end{lemma}
%\begin{proof}
%	($\impliedby$). If $\pi_1$ is sure winning for P1 to visit $X$ from a state $s$, then for any strategy $\pi_2$, the path $\rho = \outcomes(s, \pi_1, \pi_2)$ visits $X$. But all states in $X$ are sink states in $\game_X^1$. Therefore, the path cannot visit $F$. Equivalently, $\pi_1$ is sure winning for P1 in its safety objective. 
%	
%	($\implies$). Since every state $s \in X$ is a sink state, there is no path from $s$ to $F$ in $\game_X^1$. Therefore, all states in $X$ are winning for P1 in $\game_X^1$. Thus, any sure winning strategy $\pi_1$ that visits $X$ from a state $s \in \win_2(\game)$ produces a path $\rho = \outcomes(s, \pi_1, \pi_2)$ that does not visit $F$, regardless of the sure winning strategy $\pi_2$ used by P2. In other words, $\pi_1$ is sure winning for P1 in its safety objective. 
%\end{proof}
%
%
%Placing traps in P1's winning region in $\game$ does not increase the number of states from which P1 can prevent P2 from reaching $F$ in $\game_X^1$. This is because from every state in $\win_1(\game, F)$, P1 has a sure winning strategy to prevent the game from visiting $F$, and the placement of traps does not provide any incentive to P2 to deviate from its sure winning strategy to visit $F$ from any state in $\win_2(\game, F)$. The following proposition captures the effect of placing only traps in all possible configurations. 
%
%
%\begin{proposition}[Effect of Traps]
%	\label{prop:effect-of-traps}
%	Given the base game $\game$, and P1 and P2's perceptual games, $\game_{X}^1$ and $\game_{X}^2$, the following statements are true. 
%	\begin{enumerate}[(a)] 
%		\item $\win_1(\game_X^2, F) = \win_1(\game, F)$ and $\win_2(\game_X^2, F) = \win_2(\game, F)$.
%		\item If $X \subseteq \win_1(\game, F)$ then $\win_1(\game^1_X, F) = \win_1(\game, F)$ and $\win_2(\game^1_X, F) = \win_2(\game, F)$;
%		\item If $X \subseteq \win_2(\game, F) \setminus F$ then $\win_1(\game^1_X, F) \supsetneq \win_1(\game, F)$ and $\win_2(\game^1_X, F) \subsetneq \win_2(\game, F)$.
%	\end{enumerate}
%\end{proposition}
%\begin{proof}
%	In Appendix~\ref{}. 
%\end{proof}
%
%
%Proposition~\ref{prop:effect-of-traps}(a) formalizes the intuition that placement of traps does not alter P2's perception of P1 and P2's winning regions. This is because, by Remark~\ref{rmk:p2-game-is-base-game}, when $Y = \emptyset$, P2's perceptual game $\game_X^2$ is is identical to the base game $\game$. % Hence, the winning regions of P1 and P2 in $\game_X^2$ are same as those in $\game$. That is, $\win_1(\game_X^2, F) = \win_1(\game, F)$ and $\win_2(\game_X^2, F) = \win_2(\game, F)$. 
%
%
%%\paragraph*{Reword.} In words, allocating traps in P1's winning region in $\game$ has no effect on either player's winning regions in P1's perspective (\ie, the true game). However, allocating them in P2's winning region expands the set of states from which P1 can surely satisfy its safety objective. Intuitively, this is because allocating a state $s \in S$ as a trap converts it to a sink state, thereby, \emph{cutting} any path $\rho$ that first visits $s$ and then $F$. 
%
%
%Next, we analyze the case when only fake targets are allocated, \ie, $X = \emptyset$ and $Y \neq \emptyset$. For convenience, we will write the game $\game_{\emptyset, Y}$ as $\game_Y$ with an understanding that $X = \emptyset$. 
%
%
%Although the presence of fake targets affects P2's perception of the structure of the game and its payoff function, the following proposition shows that the size of P1's sure winning region in $\game_Y^1$ increases only when the fake targets are placed in P2's winning region in $\game$. 
%
%%we consider allocation of fake targets and no traps. Because P2 misperceives the fake targets to contain valuable information but is unable to recognize them as decoys, the underlying graph of P2's perceptual game $\langle S, A, T\rangle$ is the same as the base game with no decoys. However, P2 perceives $F \cup Y$ to be final states instead of $F$. We analyze the effect of allocating fake targets in $\win_1(\game, F)$ and $\win_2(\game, F)$ separately. 
%
%
%\begin{proposition}[Effect of Fake Targets]
%	\label{prop:effect-of-fakes}
%	Given the base game $\game$, and P1 and P2's perceptual games, $\game_{Y}^1$ and $\game_{Y}^2$, the following statements are true. 
%	\begin{enumerate}[(a)] 
%		\item If $Y \subseteq \win_1(\game, F)$, then $\win_1(\game^1_Y, F) = \win_1(\game, F)$ and $\win_2(\game^1_Y, F) = \win_2(\game, F)$. 
%		\item If $Y \subseteq \win_2(\game, F) \setminus F$, then $\win_1(\game^1_Y, F) \supsetneq \win_1(\game, F)$ and $\win_2(\game^1_Y, F) \subsetneq \win_2(\game, F)$.
%		\item If $Y \subseteq \win_1(\game, F)$, then $\win_1(\game^2_Y, F \cup Y) \subseteq \win_1(\game, F)$ and $\win_2(\game^2_Y, F \cup Y) \supseteq \win_2(\game, F)$. 
%		\item If $Y \subseteq \win_2(\game, F) \setminus F$, then $\win_1(\game^2_Y, F \cup Y) = \win_1(\game, F)$ and $\win_2(\game^2_Y, F \cup Y) = \win_2(\game, F)$.
%	\end{enumerate}
%\end{proposition}
%\begin{proof}
%	In Appendix~\ref{}. 
%\end{proof}
%
%
%In Proposition~\ref{prop:effect-of-fakes}, statements (a), (b) describe the effect of placing fake targets on P1's perceptual game $\game_Y^1$, while statements (c), (d) describe the effect on P2's perceptual game $\game_Y^2$. As expected, placing fake targets in P1's sure winning region in $\game$ expands P2's sure winning region in P2's perceptual game, whereas placing them in P2's sure winning region in $\game$ has no effect on the size of winning regions in P2's perceptual game. 
%
%
%An interesting case is expressed by Proposition~\ref{prop:effect-of-fakes}(a), which states that placing fake targets within P1's sure winning region in $\game$ does not benefit P1. This might appear to be contrary to common intuition. However, P1 does not gain any benefit because the fake targets are viewed as additional final states in P2's perceptual game. Their presence does not eliminate any of the P2's sure winning strategies to visit $F$. But instead, it augments the set of sure winning strategies with some spurious strategies, which if used by P2 would allow P1 to achieve its objective. 
%
%
%Similar to placing traps, P1 can ensure that the game never visits $F$ starting from a P2's sure winning state in $\game$ only if it has a sure winning strategy to visit $Y$. 
% 
%
%\begin{lemma}
%	\label{lma:advantage-of-fakes}
%	Let $Y \subseteq \win_2(\game, F) \setminus F$ be a set of traps. Given a state a state $s \in \win_2(\game, F) \setminus F$, a strategy $\pi_1$ is sure winning for P1 at $s$ in $\game^1_{Y}$ to prevent the game from visiting $F$ if and only if $\pi_1$ is a sure winning strategy to visit $Y$. 
%\end{lemma}
%\begin{proof}
%	The proof is similar to that of Lemma~\ref{lma:advantage-of-traps}. 
%\end{proof}
%
%
%We conclude this subsection by showing that \emph{fake targets can be more advantageous than traps}. This is observed by comparing the size of winning regions in $\game_{X}^1$ and $\game_{Y}^1$, as illustrated by the following example.  
%
%\begin{example}
%	Consider the toy problem shown in Figure~\ref{fig:fake-betterthan-traps}. Suppose that we are given a single decoy placed at $s_0$. We are to decide whether it should be configured as a trap or a fake target. 
%	
%	\begin{figure}[tb!]
%		\begin{center}
%			\subfigure[Game with no fake targets.]{
%				\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.5cm, scale = 0.4,transform shape]
%					
%					\node[state]              (0) [] {\Large $s_0$};
%					\node[state, rectangle]   (1) [below left of=0] {\Large $s_1$};
%					\node[state, rectangle]   (2) [below right of=0] {\Large $s_2$};
%					\node[state, rectangle]   (3) [below left of=1] {\Large $s_3$};
%					\node[state]              (4) [below right of=1] {\Large $s_4$};
%					\node[state]              (5) [below right of=2] {\Large $s_5$};
%					\node[state, rectangle, accepting] (6) [below right of=3] {\Large $s_6$};
%					\node[state, accepting]   (7) [below left of=5] {\Large $s_7$};
%					
%					\path 
%					(0) edge [bend left] node[above left=-5pt] 			{\Large $a_1$}  (1)
%					(0) edge             node[above=2pt] 			 	{\Large $a_2$}  (2)
%					(1) edge [bend left] node[above left=-5pt] 			{\Large $b_1$}  (0)
%					(1) edge [bend left] node[above left=-5pt] 			{\Large $b_2$}  (3)        
%					(1) edge             node[above right=-5pt] 		{\Large $b_3$}  (4)    
%					(2) edge             node[above left=-5pt] 			{\Large $b_1$}  (4)        
%					(2) edge             node[above right=-5pt] 		{\Large $b_2$}  (5) 
%					(3) edge [bend left] node[above left=-5pt] 	  		{\Large $b_1$}  (1) 
%					(3) edge             node[above right=-5pt] 		{\Large $b_2$}  (6) 
%					(4) edge             node[above left=-5pt]  		{\Large $b_1$}  (6) 
%					(4) edge             node[above right=-5pt] 		{\Large $b_2$}  (7) 
%					(5) edge             node[above left=-5pt]  		{\Large $a_2$}  (7) 
%					;
%				\end{tikzpicture}
%			}
%			\hfill
%			\subfigure[Game with fake target at $s_0$.]{
%				\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3.5cm, scale = 0.35,transform shape]
%					\node[state]              (0) [] {\Large $s_0$};
%					\node[state, rectangle]   (1) [above left of=0] {\Large $s_1$};
%					\node[state, rectangle, accepting] (6) [right of=0] {\Large $s_6$};
%					\node[state, accepting]   (7) [right of=6] {\Large $s_7$};
%					\node[state, rectangle]   (3) [right of=1] {\Large $s_3$};
%					\node[state]              (4) [right of=3] {\Large $s_4$};
%					\node[state]              (5) [right of=4] {\Large $s_5$};
%					\node[state, rectangle]   (2) [above right of=3] {\Large $s_2$};
%					
%					\path 
%					(0) edge [bend left] node[left] 			{\Large $a_1$}  (1)
%					(0) edge [bend right, out=-10]            node[above=2pt, pos=0.1] 			 	{\Large $a_2$}  (2)
%					(1) edge             node[above right=-5pt] 			{\Large $b_1$}  (0)
%					(1) edge [bend left] node[above left=-5pt] 			{\Large $b_2$}  (3)        
%					(1) edge [bend left, out=60] node[above right=-5pt] 		{\Large $b_3$}  (4)    
%					(2) edge             node[above right=-5pt] 			{\Large $b_1$}  (4)        
%					(2) edge             node[above right=-5pt] 		{\Large $b_2$}  (5) 
%					(3) edge             node[above left=-5pt] 	  		{\Large $b_1$}  (1) 
%					(3) edge             node[right] 		{\Large $b_2$}  (6) 
%					(4) edge             node[above left=-5pt]  		{\Large $b_1$}  (6) 
%					(4) edge             node[above right=-5pt] 		{\Large $b_2$}  (7) 
%					(5) edge             node[above left=-5pt]  		{\Large $a_2$}  (7) 
%					;
%				\end{tikzpicture}
%			}
%		\end{center}
%		\caption{A toy problem demonstrating how fake targets could be more effective than traps.}
%		\label{fig:fake-betterthan-traps}
%	\end{figure}
%	
%	First, note that all states in Figure~\ref{fig:fake-betterthan-traps} are winning for P2 in its objective to reach $F = \{s_6, s_7\}$. Using Algorithm~\ref{alg:zielonka}, the level sets are determined to be $Z_0 = \{s_6, s_7\}, Z_1 = \{s_3, s_4, s_5\}, Z_2 = \{s_1, s_2\}, Z_3 = \{s_0\}$ where the states in $Z_i$ have rank $i$, $i = 0 \ldots 3$. 
%	
%	When $s_0$ is configured as a trap, the only P2 state that becomes winning for P1 is $s_0$. However, when it is configured as a fake target, the states $s_0$ and $s_1$ become winning for P1. This is because when $s_0$ is a fake target, it is considered a final state in $\game_Y^2$. Hence, it's rank becomes $0$ and the rank of P2 state $s_1$ becomes $1$ because P2 can reach from $s_1$ to $s_0$ in one-step using action $b_1$. As a result, in P2's perception, the only subjectively rationalizable action at $s_1$ is $b_1$ since it is the only rank-reducing action. The action $b_2$ is not subjectively rationalizable because it is not rank-reducing.
%		
%	It is noted that the state $s_3$ from which P2 has a strategy to surely visit $s_0$ is not subjectively rationalizable for P2 in its perceptual game. Again, this is because the only rank-reducing action at $s_3$ is $b_2$, which induces a visit to $s_6$ in one-step. \qed
%\end{example}
%
%
%The above example illustrates that, even though placing fake targets in $\win_2(\game, F)$ does not affect the size of winning region in $\game_{Y}^2$, it may alter their ranks. Since any sure winning strategy of P2 selects a rank-reducing action, any change in ranks of the states might change P2's sure winning strategy. As a consequence, we have the following theorem which states that \emph{fake targets can be more advantageous than traps}. 
%
%%Since traps do not affect P2's payoff function, they do not induce such an effect in P2's perceptual game. The following proposition formalizes this idea. 
%
%
%%\begin{proposition}
%%	\label{prop:traps-rank-of-p1-winner} 
%%	%	
%%	Given a set of traps $X \subseteq \win_2(\game, F)$, let $s \in \win_2(\game, F)$ be a state from which P1 has a sure winning strategy to  visit $X$. Then, $\rank(s) > \min \{\rank(t) \mid t \in Y\}$. 
%%\end{proposition}
%%\begin{proof}[Proof (Sketch)]
%%	By contradiction. Suppose there exists a state $s \in \win_2(\game, F)$ such that P1 has sure winning strategy $\pi_1$ to visit a trap in $X$ whose rank is at least equal to $\rank(s)$. Thus, for any P2's sure winning strategy $\pi_2$, there must exist a rank-increasing transition in the path $\rho = \outcomes(s, \pi_1, \pi_2)$. By definition of attractor \cite{}, if $s$ is a P1 state, then every action from $s$ is rank reducing. If $s$ is a P2 state, then a rational P2 will follow a sure winning strategy to visit $F$, which, at any state, chooses a rank reducing action. Hence, a rank-increasing transition cannot occur---a contradiction. 
%%\end{proof}
%%
%%
%%It is easy to see that if the states in $X$ in Proposition~\ref{prop:traps-rank-of-p1-winner} were to be allocated as fake targets instead, P1 could use the same sure winning strategy at $s$ to visit a fake target. But, as Example~\ref{ex:to-be-named} demonstrates, it is also possible that P1 may guarantee a visit to a fake target from a state with a lower rank than the fake target. This is because setting a state as fake target makes it a rank $0$ state in $\game_Y^2$. Hence, we have the following result.
%
%
%\begin{theorem}
%	\label{thm:traps-fakes-subset-relation}
%	For any $Z \subseteq \win_2(\game, F) \setminus F$, we have $\win_1(\game) \subseteq \win_1(\game_{Z, \emptyset}^1, F) \subseteq \win_1(\game_{\emptyset, Z}^1, F \cup Z)$.
%\end{theorem}
%\begin{proof}
%	From Proposition~\ref{prop:effect-of-traps}, we know that $\win_1(\game) \subseteq \win_1(\game_{Z, \emptyset}^1, F)$ holds. To see why $\win_1(\game_{Z, \emptyset}^1, F) \subseteq \win_1(\game_{\emptyset, Z}^1, F \cup Z)$ is true, consider a state $s \in \win_2(\game, F)$ from which P1 has a sure winning strategy $\pi_1$ to visit $Z$ in $\game_{Z, \emptyset}^1$. We will show that $\pi_1$ is sure winning for P1 to visit $Z$ in $\game_{\emptyset, Z}^1$. 
%	
%	\ak{todo}. 
%\end{proof}
%
%
%
%
%
%
%
%
%


==> sections/effectsOfDecoy2.tex <==
\paragraph*{} Recall that by placing traps P1 can manipulate the structure of game as perceived by P2, whereas by placing fake targets P1 can manipulate the structure of game and the payoff function of P2 in its perceptual game. In this subsection, we investigate how the placement of traps and fake targets affect the winning regions and strategies of players in P1 and P2's perceptual games, $\game_{X,Y}^1$ and $\game_{X,Y}^2$. 


\paragraph*{} The overall effect of placing a mixture of traps and fake targets can be understood by studying the effects of placing only traps and only fake targets. We start by analyzing the case when only traps are allocated, \ie, $X \neq \emptyset$ and $Y = \emptyset$. For convenience, we will write the game $\game_{X, \emptyset}$ as $\game_X$ with an understanding that $Y = \emptyset$.


\paragraph*{} Consider the case when the traps are placed in P2's winning region in the base game $\game$, \ie, $X \subseteq \win_2(\game, F)$. Such a placement increases the number of states from where P1 can surely prevent P2 from visiting $F$. To see this, first observe that P2 cannot win from any state in $X$. Moreover, since the states in $X$ become `sink' states, any winning path of P2 in $\game$ that visits a state in $X$ before visiting $F$, will become winning for P1 in the true game $\game_X^1$. Hence, if there exists a strategy $\pi_1$ for P1 such that all paths $\rho = \outcomes(s, \pi_1, \pi_2)$ starting from a state $s \in \win_2(\game, F)$ visit $X$ before visiting $F$ for any P2's sure winning strategy $\pi_2$ in $\game_X^2$, then the P2's sure winning state $s$ in $\game$ would become sure winning for P1 in $\game_X^1$. This intuition is formalized in the following statement. 


\begin{lemma} \label{lma:advantage-of-traps}
	Let $X \subseteq \win_2(\game, F) \setminus F$ be a set of traps. A strategy $\pi_1$ is sure winning for P1 in $\game^1_{X}$ to prevent the game from visiting $F$, if and only if $\pi_1$ is a sure winning strategy to visit $X$. 
\end{lemma}
\begin{proof}
	($\impliedby$). If $\pi_1$ is sure winning for P1 to visit $X$ from a state $s$, then for any strategy $\pi_2$, the path $\rho = \outcomes(s, \pi_1, \pi_2)$ visits $X$. But all states in $X$ are sink states in $\game_X^1$. Therefore, the path cannot visit $F$. Equivalently, $\pi_1$ is sure winning for P1 in its safety objective. 
	
	($\implies$). Since every state $s \in X$ is a sink state, there is no path from $s$ to $F$ in $\game_X^1$. Therefore, all states in $X$ are winning for P1 in $\game_X^1$. Thus, any sure winning strategy $\pi_1$ that visits $X$ from a state $s \in \win_2(\game)$ produces a path $\rho = \outcomes(s, \pi_1, \pi_2)$ that does not visit $F$, regardless of the sure winning strategy $\pi_2$ used by P2. In other words, $\pi_1$ is sure winning for P1 in its safety objective. 
\end{proof}


\paragraph*{} Placing traps in P1's winning region in $\game$ does not increase the number of states from which P1 can prevent P2 from reaching $F$ in $\game_X^1$. This is because from every state in $\win_1(\game, F)$, P1 has a sure winning strategy to prevent the game from visiting $F$, and the placement of traps does not provide any incentive to P2 to deviate from its sure winning strategy to visit $F$ from any state in $\win_2(\game, F)$. The following proposition captures the effect of placing only traps in all possible configurations. 


\begin{proposition}[Effect of Traps]
	\label{prop:effect-of-traps}
	Given the base game $\game$, and P1 and P2's perceptual games, $\game_{X}^1$ and $\game_{X}^2$, the following statements are true. 
	\begin{enumerate}[(a)] 
		\item $\win_1(\game_X^2, F) = \win_1(\game, F)$ and $\win_2(\game_X^2, F) = \win_2(\game, F)$.
		\item If $X \subseteq \win_1(\game, F)$ then $\win_1(\game^1_X, F) = \win_1(\game, F)$ and $\win_2(\game^1_X, F) = \win_2(\game, F)$;
		\item If $X \subseteq \win_2(\game, F) \setminus F$ then $\win_1(\game^1_X, F) \supsetneq \win_1(\game, F)$ and $\win_2(\game^1_X, F) \subsetneq \win_2(\game, F)$.
	\end{enumerate}
\end{proposition}
\begin{proof}
	In Appendix~\ref{}. 
\end{proof}


\paragraph*{} Proposition~\ref{prop:effect-of-traps}(a) formalizes the intuition that placement of traps does not alter P2's perception of P1 and P2's winning regions. This is because, by Remark~\ref{rmk:p2-game-is-base-game}, when $Y = \emptyset$, P2's perceptual game $\game_X^2$ is is identical to the base game $\game$. % Hence, the winning regions of P1 and P2 in $\game_X^2$ are same as those in $\game$. That is, $\win_1(\game_X^2, F) = \win_1(\game, F)$ and $\win_2(\game_X^2, F) = \win_2(\game, F)$. 


%\paragraph*{Reword.} In words, allocating traps in P1's winning region in $\game$ has no effect on either player's winning regions in P1's perspective (\ie, the true game). However, allocating them in P2's winning region expands the set of states from which P1 can surely satisfy its safety objective. Intuitively, this is because allocating a state $s \in S$ as a trap converts it to a sink state, thereby, \emph{cutting} any path $\rho$ that first visits $s$ and then $F$. 


\paragraph*{} Next, we analyze the case when only fake targets are allocated, \ie, $X = \emptyset$ and $Y \neq \emptyset$. For convenience, we will write the game $\game_{\emptyset, Y}$ as $\game_Y$ with an understanding that $X = \emptyset$. 


\paragraph*{} Although the presence of fake targets affects P2's perception of the structure of the game and its payoff function, the following proposition shows that the size of P1's sure winning region in $\game_Y^1$ increases only when the fake targets are placed in P2's winning region in $\game$. 

%we consider allocation of fake targets and no traps. Because P2 misperceives the fake targets to contain valuable information but is unable to recognize them as decoys, the underlying graph of P2's perceptual game $\langle S, A, T\rangle$ is the same as the base game with no decoys. However, P2 perceives $F \cup Y$ to be final states instead of $F$. We analyze the effect of allocating fake targets in $\win_1(\game, F)$ and $\win_2(\game, F)$ separately. 


\begin{proposition}[Effect of Fake Targets]
	\label{prop:effect-of-fakes}
	Given the base game $\game$, and P1 and P2's perceptual games, $\game_{Y}^1$ and $\game_{Y}^2$, the following statements are true. 
	\begin{enumerate}[(a)] 
		\item If $Y \subseteq \win_1(\game, F)$, then $\win_1(\game^1_Y, F) = \win_1(\game, F)$ and $\win_2(\game^1_Y, F) = \win_2(\game, F)$. 
		\item If $Y \subseteq \win_2(\game, F) \setminus F$, then $\win_1(\game^1_Y, F) \supsetneq \win_1(\game, F)$ and $\win_2(\game^1_Y, F) \subsetneq \win_2(\game, F)$.
		\item If $Y \subseteq \win_1(\game, F)$, then $\win_1(\game^2_Y, F \cup Y) \subseteq \win_1(\game, F)$ and $\win_2(\game^2_Y, F \cup Y) \supseteq \win_2(\game, F)$. 
		\item If $Y \subseteq \win_2(\game, F) \setminus F$, then $\win_1(\game^2_Y, F \cup Y) = \win_1(\game, F)$ and $\win_2(\game^2_Y, F \cup Y) = \win_2(\game, F)$.
	\end{enumerate}
\end{proposition}
\begin{proof}
	In Appendix~\ref{}. 
\end{proof}


\paragraph*{} In Proposition~\ref{prop:effect-of-fakes}, statements (a), (b) describe the effect of placing fake targets on P1's perceptual game $\game_Y^1$, while statements (c), (d) describe the effect on P2's perceptual game $\game_Y^2$. As expected, placing fake targets in P1's sure winning region in $\game$ expands P2's sure winning region in P2's perceptual game, whereas placing them in P2's sure winning region in $\game$ has no effect on the size of winning regions in P2's perceptual game. 


\paragraph*{} An interesting case is expressed by Proposition~\ref{prop:effect-of-fakes}(a), which states that placing fake targets within P1's sure winning region in $\game$ does not benefit P1. This might appear to be contrary to common intuition. However, P1 does not gain any benefit because the fake targets are viewed as additional final states in P2's perceptual game. Their presence does not eliminate any of the P2's sure winning strategies to visit $F$. But instead, it augments the set of sure winning strategies with some spurious strategies, which if used by P2 would allow P1 to achieve its objective. 


\paragraph*{} Similar to placing traps, P1 can ensure that the game never visits $F$ starting from a P2's sure winning state in $\game$ only if it has a sure winning strategy to visit $Y$. 


\begin{lemma}
	\label{lma:advantage-of-fakes}
	Let $Y \subseteq \win_2(\game, F) \setminus F$ be a set of traps. Given a state a state $s \in \win_2(\game, F) \setminus F$, a strategy $\pi_1$ is sure winning for P1 at $s$ in $\game^1_{Y}$ to prevent the game from visiting $F$ if and only if $\pi_1$ is a sure winning strategy to visit $Y$. 
\end{lemma}
\begin{proof}
	The proof is similar to that of Lemma~\ref{lma:advantage-of-traps}. 
\end{proof}


\paragraph*{} We conclude this subsection by showing that \emph{fake targets can be more advantageous than traps}. This is observed by comparing the size of winning regions in $\game_{X}^1$ and $\game_{Y}^1$, as illustrated by the following example.  

\begin{example}
	Consider the toy problem shown in Figure~\ref{fig:fake-betterthan-traps}. Suppose that we are given a single decoy placed at $s_0$. We are to decide whether it should be configured as a trap or a fake target. 
	
	\begin{figure}[tb!]
		\begin{center}
			\subfigure[Game with no fake targets.]{
				\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.5cm, scale = 0.4,transform shape]
					
					\node[state]              (0) [] {\Large $s_0$};
					\node[state, rectangle]   (1) [below left of=0] {\Large $s_1$};
					\node[state, rectangle]   (2) [below right of=0] {\Large $s_2$};
					\node[state, rectangle]   (3) [below left of=1] {\Large $s_3$};
					\node[state]              (4) [below right of=1] {\Large $s_4$};
					\node[state]              (5) [below right of=2] {\Large $s_5$};
					\node[state, rectangle, accepting] (6) [below right of=3] {\Large $s_6$};
					\node[state, accepting]   (7) [below left of=5] {\Large $s_7$};
					
					\path 
					(0) edge [bend left] node[above left=-5pt] 			{\Large $a_1$}  (1)
					(0) edge             node[above=2pt] 			 	{\Large $a_2$}  (2)
					(1) edge [bend left] node[above left=-5pt] 			{\Large $b_1$}  (0)
					(1) edge [bend left] node[above left=-5pt] 			{\Large $b_2$}  (3)        
					(1) edge             node[above right=-5pt] 		{\Large $b_3$}  (4)    
					(2) edge             node[above left=-5pt] 			{\Large $b_1$}  (4)        
					(2) edge             node[above right=-5pt] 		{\Large $b_2$}  (5) 
					(3) edge [bend left] node[above left=-5pt] 	  		{\Large $b_1$}  (1) 
					(3) edge             node[above right=-5pt] 		{\Large $b_2$}  (6) 
					(4) edge             node[above left=-5pt]  		{\Large $b_1$}  (6) 
					(4) edge             node[above right=-5pt] 		{\Large $b_2$}  (7) 
					(5) edge             node[above left=-5pt]  		{\Large $a_2$}  (7) 
					;
				\end{tikzpicture}
			}
			\hfill
			\subfigure[Game with fake target at $s_0$.]{
				\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3.5cm, scale = 0.35,transform shape]
					\node[state]              (0) [] {\Large $s_0$};
					\node[state, rectangle]   (1) [above left of=0] {\Large $s_1$};
					\node[state, rectangle, accepting] (6) [right of=0] {\Large $s_6$};
					\node[state, accepting]   (7) [right of=6] {\Large $s_7$};
					\node[state, rectangle]   (3) [right of=1] {\Large $s_3$};
					\node[state]              (4) [right of=3] {\Large $s_4$};
					\node[state]              (5) [right of=4] {\Large $s_5$};
					\node[state, rectangle]   (2) [above right of=3] {\Large $s_2$};
					
					\path 
					(0) edge [bend left] node[left] 			{\Large $a_1$}  (1)
					(0) edge [bend right, out=-10]            node[above=2pt, pos=0.1] 			 	{\Large $a_2$}  (2)
					(1) edge             node[above right=-5pt] 			{\Large $b_1$}  (0)
					(1) edge [bend left] node[above left=-5pt] 			{\Large $b_2$}  (3)        
					(1) edge [bend left, out=60] node[above right=-5pt] 		{\Large $b_3$}  (4)    
					(2) edge             node[above right=-5pt] 			{\Large $b_1$}  (4)        
					(2) edge             node[above right=-5pt] 		{\Large $b_2$}  (5) 
					(3) edge             node[above left=-5pt] 	  		{\Large $b_1$}  (1) 
					(3) edge             node[right] 		{\Large $b_2$}  (6) 
					(4) edge             node[above left=-5pt]  		{\Large $b_1$}  (6) 
					(4) edge             node[above right=-5pt] 		{\Large $b_2$}  (7) 
					(5) edge             node[above left=-5pt]  		{\Large $a_2$}  (7) 
					;
				\end{tikzpicture}
			}
		\end{center}
		\caption{A toy problem demonstrating how fake targets could be more effective than traps.}
		\label{fig:fake-betterthan-traps}
	\end{figure}
	
	First, note that all states in Figure~\ref{fig:fake-betterthan-traps} are winning for P2 in its objective to reach $F = \{s_6, s_7\}$. Using Algorithm~\ref{alg:zielonka}, the level sets are determined to be $Z_0 = \{s_6, s_7\}, Z_1 = \{s_3, s_4, s_5\}, Z_2 = \{s_1, s_2\}, Z_3 = \{s_0\}$ where the states in $Z_i$ have rank $i$, $i = 0 \ldots 3$. 
	
	When $s_0$ is configured as a trap, the only P2 state that becomes winning for P1 is $s_0$. However, when it is configured as a fake target, the states $s_0$ and $s_1$ become winning for P1. This is because when $s_0$ is a fake target, it is considered a final state in $\game_Y^2$. Hence, it's rank becomes $0$ and the rank of P2 state $s_1$ becomes $1$ because P2 can reach from $s_1$ to $s_0$ in one-step using action $b_1$. As a result, in P2's perception, the only subjectively rationalizable action at $s_1$ is $b_1$ since it is the only rank-reducing action. The action $b_2$ is not subjectively rationalizable because it is not rank-reducing.
	
	It is noted that the state $s_3$ from which P2 has a strategy to surely visit $s_0$ is not subjectively rationalizable for P2 in its perceptual game. Again, this is because the only rank-reducing action at $s_3$ is $b_2$, which induces a visit to $s_6$ in one-step. \qed
\end{example}


\paragraph*{} The above example illustrates that, even though placing fake targets in $\win_2(\game, F)$ does not affect the size of winning region in $\game_{Y}^2$, it may alter their ranks. Since any sure winning strategy of P2 selects a rank-reducing action, any change in ranks of the states might change P2's sure winning strategy. As a consequence, we have the following theorem which states that \emph{fake targets can be more advantageous than traps}. 

%Since traps do not affect P2's payoff function, they do not induce such an effect in P2's perceptual game. The following proposition formalizes this idea. 


%\begin{proposition}
%	\label{prop:traps-rank-of-p1-winner} 
%	%	
%	Given a set of traps $X \subseteq \win_2(\game, F)$, let $s \in \win_2(\game, F)$ be a state from which P1 has a sure winning strategy to  visit $X$. Then, $\rank(s) > \min \{\rank(t) \mid t \in Y\}$. 
%\end{proposition}
%\begin{proof}[Proof (Sketch)]
%	By contradiction. Suppose there exists a state $s \in \win_2(\game, F)$ such that P1 has sure winning strategy $\pi_1$ to visit a trap in $X$ whose rank is at least equal to $\rank(s)$. Thus, for any P2's sure winning strategy $\pi_2$, there must exist a rank-increasing transition in the path $\rho = \outcomes(s, \pi_1, \pi_2)$. By definition of attractor \cite{}, if $s$ is a P1 state, then every action from $s$ is rank reducing. If $s$ is a P2 state, then a rational P2 will follow a sure winning strategy to visit $F$, which, at any state, chooses a rank reducing action. Hence, a rank-increasing transition cannot occur---a contradiction. 
%\end{proof}
%
%
%\paragraph*{} It is easy to see that if the states in $X$ in Proposition~\ref{prop:traps-rank-of-p1-winner} were to be allocated as fake targets instead, P1 could use the same sure winning strategy at $s$ to visit a fake target. But, as Example~\ref{ex:to-be-named} demonstrates, it is also possible that P1 may guarantee a visit to a fake target from a state with a lower rank than the fake target. This is because setting a state as fake target makes it a rank $0$ state in $\game_Y^2$. Hence, we have the following result.


\begin{theorem}
	\label{thm:traps-fakes-subset-relation}
	For any $Z \subseteq \win_2(\game, F) \setminus F$, we have $\win_1(\game) \subseteq \win_1(\game_{Z, \emptyset}^1, F) \subseteq \win_1(\game_{\emptyset, Z}^1, F \cup Z)$.
\end{theorem}
\begin{proof}
	From Proposition~\ref{prop:effect-of-traps}, we know that $\win_1(\game) \subseteq \win_1(\game_{Z, \emptyset}^1, F)$ holds. To see why $\win_1(\game_{Z, \emptyset}^1, F) \subseteq \win_1(\game_{\emptyset, Z}^1, F \cup Z)$ is true, consider a state $s \in \win_2(\game, F)$ from which P1 has a sure winning strategy $\pi_1$ to visit $Z$ in $\game_{Z, \emptyset}^1$. We will show that $\pi_1$ is sure winning for P1 to visit $Z$ in $\game_{\emptyset, Z}^1$. 
	
	\ak{todo}. 
\end{proof}











==> sections/effectsOfDecoy3.tex <==
Recall that the presence of traps affects the structure of game, whereas the presence of fake targets changes the structure of game and P2's perceived objective in its perceptual game. In this section, we study the effect of these changes on the winning regions and strategies in the modified game when compared to those in the base game. 

\begin{remark}
	The results derived in this section are general. They apply to any problem in which the structure and/or the objectives of players are modified during the game.
\end{remark}
 

Consider the base game $\game$ and the game $\game_{X, Y}^1$, in which the subsets $X, Y \subseteq S \setminus F$, $X \cap Y = \emptyset$, are allocated as traps and fake targets, and P1's objective is to prevent P2 from reaching $F$. In Problem~\ref{prob:decoy-placement}, this corresponds to P1's perceptual game or the true game. 

\jf{For simplicity in your notation, you can use $\game$ for the base game. $\game^1$ for the game where $X$ and $Y$ are traps. $\game^2$ is the game where $Y\cup F$ are targets. }

\jf{My other comment is that it is very difficulty to say it is the effect of decoys without talking about the misperceptions players have.}

\begin{proposition}
	\label{prop:effect-on-p1}
	The following statements are true about $\game_{X, Y}^1$. 
	\begin{enumerate}[(a)] 
		\item If $X \cup Y \subseteq \win_1(\game, F)$ then $\win_1(\game_{X, Y}^1, F) = \win_1(\game, F)$ and $\win_2(\game_{X, Y}^1, F) = \win_2(\game, F)$. 
		\item If $X \cup Y \subseteq \win_2(\game, F) \setminus F$ then $\win_1(\game_{X, Y}^1, F) \supsetneq \win_1(\game, F)$ and $\win_2(\game_{X, Y}^1, F) \subsetneq \win_2(\game, F)$. 
	\end{enumerate}
\end{proposition}

\jf{the first statement seems to be incorrect. if new target is added, then P2's winning region must be increased.}
\ak{P2's winning region increases in P2's perceptual game. $\game_{X, Y}^1$ is the true game, where P2's objective is to reach $F$ and P1's is prevent it.}

A rigorous proof is included in Appendix~\ref{app:proofs}. Here, we discuss the key insights behind the proof. 


When decoys are placed within P1's winning region in $\game$, the players' winning regions in $\game_{X, Y}^1$ remain identical to those in $\game$. This is because converting the states in $\win_1(\game, F)$ to sink states neither eliminates any P2's winning strategy from any state in $\win_2(\game, F)$ nor does it convert a P1's winning state in $\win_1(\game, F)$ to a P2's winning state. 


On the contrary, when traps or fake targets are placed in P2's winning region in $\game$, some of P2's sure winning states in $\game$ become sure winning for P1 in $\game_{X, Y}^1$. Clearly, every state in $X \cup Y$ is winning for P1 in $\game_{X, Y}^1$ because it is a sink state. Furthermore, any state in $\win_2(\game, F) \setminus F$ from which P1 has a sure winning strategy to visit $X \cup Y$ also becomes sure winning for P1 in $\game_{X, Y}^1$. The following lemma describes the condition for a state in $\win_2(\game, F) \setminus F$ to become sure winning for P1 in $\game_{X, Y}^1$. 


\begin{lemma} 
	\label{lma:effect-on-p1-decoys-in-win2}
	Let the set $X \cup Y \subseteq \win_2(\game, F) \setminus F$ be allocated as traps and fake targets. Given a state $s \in \win_2(\game, F) \setminus F$, a strategy $\pi_1$ is sure winning for P1 at state $s$ in the game $\game^1_{X, Y}$ if and only if $\pi_1$ is a sure winning strategy for P1 at $s$ to visit $X \cup Y$. 
\end{lemma}
\begin{proof}
	($\implies$). Given that $\pi_1$ is sure winning in $\game_{X, Y}^1$ to prevent a visit to $F$, we want to establish that $\pi_1$ is sure winning in $\game_{X, Y}^1$ to visit $X \cup Y$. Since $s$ is P2's sure winning state in $\game$, consider any sure winning strategy $\pi_2$ at $s$. Then, the path $\rho = \outcomes_\game(s, \pi_1, \pi_2)$ must visit $F$ in $\game$. Consider the path $\rho' = \outcomes_{\game_{X, Y}^1}(s, \pi_1, \pi_2)$. If $\rho$ does not visit any state in $X \cup Y$, then, by Definition~\ref{def:p1-perceptual-game}, we have $\rho' = \rho$, which violates the given information. The only other case is that $\rho$ visit some state in $X \cup Y$, in which case, $\rho'$ visits a sink state in $X \cup Y$ and therefore does not visit $F$. 

 \jf{the path $\rho = \outcomes_\game(s, \pi_1, \pi_2)$  should be $\rho \in \outcomes_\game(s, \pi_1, \pi_2)$. similarly for $\rho'$.
I don't see why $\rho$ must equal $\rho'$.
}
	($\impliedby$). Given that $\pi_1$ is sure winning in $\game_{X, Y}^1$ to visit $X \cup Y$, we want to establish that $\pi_1$ is sure winning in $\game_{X, Y}^1$ to prevent a visit to $F$. Since every state $t \in X \cup Y$ is a sink state, there is no path from $t$ to $F$ in $\game_X^1$. Therefore, all states in $X \cup Y$ are winning for P1 in $\game_X^1$. By definition, every path $\rho = \outcomes(s, \pi_1, \pi_2)$ visits $X \cup Y$ for any P2 strategy $\pi_2$. Therefore, the game cannot visit $F$. 
\end{proof}

\jf{there is another consideration. when p1 try to reach $X\cup Y$, what is the assumption for P2's strategy? trying to avoid $X\cup Y$? The sure winning for reaching $X\cup Y$ is played against P2 who tries to avoid $X\cup Y$. I think the result only holds in the hypergame.}

A key insight from Lemma~\ref{lma:effect-on-p1-decoys-in-win2} is that decoys \emph{cut the winning paths} passing through them when placed in $\win_2(\game, F)$. 


Next, we consider the base game $\game$ and the game $\game^2$, in which a subset $Y \subseteq S \setminus F$ is allocated as fake targets and P2's objective is to reach $F \cup Y$. In Problem~\ref{prob:decoy-placement}, this corresponds to P2's perceptual game $\game_{X, Y}^2$ since traps $X$ do not affect P2's perception. 


\begin{proposition}
	\label{prop:effect-on-p2}
	The following statements are true about $\game^2$. 
	\begin{enumerate}[(a)] 
		\item If $Y \subseteq \win_1(\game, F)$, then $\win_1(\game^2, F \cup Y) \subsetneq \win_1(\game, F)$ and $\win_2(\game^2, F \cup Y) \supsetneq \win_2(\game, F)$.
		\item If $Y \subseteq \win_2(\game, F)$, then $\win_1(\game^2, F \cup Y) = \win_1(\game, F)$ and $\win_2(\game^2, F \cup Y) = \win_2(\game, F)$.
	\end{enumerate}
\end{proposition}


Again, we provide a rigorous proof in Appendix~\ref{app:proofs} and discuss the key insights behind the proof. 


When fake targets are placed within P1's winning region in $\game$, some of P1's sure winning states in $\game$ become sure winning for P2 in $\game^2$. Clearly, P2 misperceives every state in $Y$ to be winning for itself in $\game^2$ because it is a goal state in $\game^2$. Thus, any state $s \in \win_1(\game, F)$ from which P2 can surely visit $F \cup Y$ is also perceived to be sure winning for itself by P2 in $\game^2$. 


When fake targets are placed within P2's winning region in $\game$, the players' winning regions in $\game^2$ remain identical to those in $\game$. To understand the insight behind the proof of this fact, we must understand how fake targets affect the winning strategies of P2. 


\begin{example}
	Consider a game shown in Figure~\ref{fig:toy-game}. We will denote it by $\game$. The game consists of $12$ states of which $F = \{s_0, s_1\}$ are final states. Using Algorithm~\ref{alg:zielonka}, the level sets are determined to be $Z_0 = \{s_0, s_1\}$, $Z_1 = \{s_2, s_3, s_4\}$, $Z_2 = \{s_4, s_5\}$, $Z_3 = \{s_7\}$, $Z_4 = \{s_8\}$, $Z_5 = \{s_9\}$ where the final states, which are in $Z_0$, have the lowest rank $0$, and $s_9$ has the highest rank $5$. The states $s_10, s_11$ are losing for P2. 
	
%	\begin{figure}[t]
%		\centering
%		\subfloat[Perceptual Game Arena of P2\label{fig:arena-p2}]{%
%			\input{figures/toy-example.tex}
%		}\hfill
%		\subfloat[\centering Perceptual Game Arena of P2 (Ground-Truth)\label{fig:arena-p1}]{%
%			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.5cm, scale = 0.5,transform shape]
%				
%				\node[state,rectangle] (a) []                         {\Large $a$};
%				\node[state] (b) [right of=a]                         {\Large $b$};
%				\node[state,rectangle] (c) [right of=b]               {\Large $c$};
%				\node[state,rectangle] (d) [right of=c]               {\Large $d$};
%				\node[state,rectangle] (e) [right of=d]               {\Large $e$};
%				\node[state] (f) [below of=b]                         {\Large $f$};
%				\node[state] (g) [below of=c]                         {\Large $g$};
%				\node[state,fill=red!40] (h) [below of=d]             {\Large $h$};
%				\node[state] (i) [below of=e]                         {\Large $i$};
%				\node[state,rectangle] (j) [below of=f]               {\Large $j$};
%				\node[state,rectangle,fill=red!40] (k) [below of=g]   {\Large $k$};
%				\node[state,rectangle] (l) [below of=h]               {\Large $l$};
%				\node[state,rectangle] (m) [below of=i]               {\Large $m$};
%				\node[state] (n) [below of=k]                         {\Large $n$};
%				\node[state] (o) [below of=l]                         {\Large $o$};
%				
%				\path (a) edge[bend left]   node {} (b)
%				(b) edge[bend left]   node {} (a)
%				(c) edge              node {} (b)
%				(c) edge              node {} (f)
%				(c) edge              node {} (g)
%				(c) edge              node {} (h)
%				(d) edge              node {} (g)
%				(d) edge              node {} (h)
%				(e) edge              node {} (i)
%				(f) edge              node {} (j)
%				(f) edge              node {} (k)
%				(g) edge              node {} (k)
%				(h) edge              node {} (l)
%				(i) edge              node {} (m)
%				(j) edge              node {} (n)
%				(k) edge              node {} (n)
%				(k) edge              node {} (o)
%				(l) edge              node {} (n)
%				(m) edge              node {} (o)
%				(n) edge [loop below]             node {} (n)
%				(o) edge [loop below]              node {} (o)
%				;
%				
%			\end{tikzpicture}
%		}
%		
%		\caption{Perceptual Game Arenas of P1 and P2 in Ex.~\ref{ex:running-example-1}.}
%		\label{fig:arena}
%	\end{figure}
	\aknote{Add figure.}

	
	Consider the case when $Y = \{s_7\}$. Figure~\ref{fig:toy-game-with-fake-7} shows the result of applying Algorithm~\ref{alg:zielonka} to game $\game^2$, in which $F \cup Y$ are final states. The level sets are determined to be $Z_0 = \{s_0, s_1, s_7\}$, $Z_1 = \{s_2, s_3, s_4, s_5, s_8\}$, $Z_2 = \{s_6\}$, $Z_3 = \{s_9\}$. Because of the changes in ranks of states, the (greedy) sure winning strategy of P2 at $s_5$ selects $b_1$ to visit $s_7$ since it is the only rank-reducing strategy. This is in contrast to the winning strategy  at $s_5$ in $\game$, which selects $b_2$ to visit $s_2$. 		
	\qed
\end{example}


Example~\ref{} highlights that fake targets affect the ranks of states because the rank of states in $Y$ is set to $0$. In fact, we observe that the rank of any state in $\game^2$ is smaller than the rank of that state in $\game$. 


\begin{lemma}
	Given a state $s \in \win_2(\game, F)$, the rank of $s$ in $\game^2$ is less than or equal to its rank in $\game$. 
\end{lemma}
\begin{proof}[Proof (Sketch)]
	Rank of a state in $\game$ is the smallest number of steps in which the player can ensure a visit to $F$. Fix P1 strategy $\pi_1$. We have two cases: (a) There exists a greedy sure winning strategy $\pi_2$ at $s$ which induces a path that first visits $Y$ then visits $F$, and (b) Every greedy sure winning strategy $\pi_2$ at $s$ induces a path that visits $F$ without visiting $Y$. In case (a), the rank of $s$ would reduce in $\game^2$ because by following $\pi_2$, P2 can visit $F \cup Y$ in smaller number of steps than in $\game$. In case (b), if any state appearing in the the path satisfies case (a), then the rank of $s$ in $\game^2$ would reduce. Otherwise, the rank would remain the same. 
\end{proof}


Since the rank of a state may only decrease, it must be the case that every P2's winning state in $\game$ remains winning for P2 in $\game^2$. 
	

==> sections/experiment.tex <==
\begin{figure}[tb]
	\centering
	\includegraphics[scale=0.25]{figures/gridworld.png}
	\caption{Gridworld example}
	\label{fig:tom-jerry-gridworld}
\end{figure}


In this section, we illustrate the key insights from our paper using a gridworld example featuring the characters Tom and Jerry. As shown in Figure~\ref{fig:tom-jerry-gridworld}, the $7 \times 7$ gridworld has two cheese blocks placed in two cells $(1, 6)$ and $(4, 6)$, where a cell is represented using row-column format. Tom is equipped with $M$ traps and $N$ fake cheese blocks to protect the real cheese from Jerry. Jerry's objective is to steal the cheese while that of Tom is to strategically place the decoys to safeguard the real cheese and potentially capture Jerry. Tom captures Jerry when they are simultaneously in the same cell. Jerry is assumed to be unaware about the presence of decoys. Both Tom and Jerry can occupy any cell in the gridworld that does not contain an obstacle. To avoid trivial cases, we assume that the game does not start with Jerry in a cell that contains the real cheese or a decoy.
%Both characters can occupy any cell devoid of an obstacle in the gridworld, with an assumption that the game does not start with Jerry in a cell containing the real cheese or a decoy.


%We examine three scenarios: (A) when $M=2$ and $N=0$, (B) when $M=1$ and $N=1$, and (B) when $M=0$ and $N=2$. In each case, we compare the positions and value of deception (formally defined below) between the placements generated by Algorithm~\ref{} and the true optimal placements, which we determine by exhaustively solving ${43}\choose{2}$ possible placement combinations. Also, we compare the value of deception when the players use deterministic strategies versus when they use randomized strategies. 

A state in the base game between Tom and Jerry is represented as \texttt{(tom.row, tom.col, jerry.row, jerry.col, turn)}. At any state, the player whose turn it is to play chooses an action from the set $\{N, E, S, W\}$. If the result of the action leads the player to a cell outside the bounds of gridworld or an obstacle, the player returns to the same cell it started from. This results in the graph of base game to have $4050$ states and $16200$ transitions. 


%We implemented the case study in Python 3.10\footnote{The code is available at \url{https://github.com/abhibp1993/ggsolver}}. All the experiments were performed on a Windows 10 machine with a core i$7$, 3.30GHz CPU and a 32GB memory. 


%We consider three scenarios: (A) when $M=2$ and $N=0$, (B) when $M=1$ and $N=1$, and (C) when $M=0$ and $N=2$. For each scenario, we determine the best decoy placement under sure and almost-sure winning criterion using the greedy approach, Algorithm~\ref{alg:greedymax}, and by exhaustive enumeration, \ie, by solving ${{43}\choose{2}} = 1176$ hypergames defined by all possible ways of allocating $2$ decoys among $43$ cells (\ie, the cells devoid of obstacles and real cheese).


We consider three scenarios: (A) with $M=2$ and $N=0$, (B) with $M=1$ and $N=1$, and (C) with $M=0$ and $N=2$. For each scenario, we determine the optimal decoy placement based on the sure and almost-sure winning criteria using two methods: the greedy approach implemented in Algorithm~\ref{alg:greedymax} and exhaustive enumeration. Exhaustive enumeration involves solving ${{43}\choose{2}} = 1176$ hypergames, which consider all possible ways of allocating $2$ decoys among the $43$ cells devoid of obstacles and real cheese. Additionally, we record the solutions to $43 + 42 = 85$ hypergames solved during the two iterations of the \texttt{While} loop in Algorithm~\ref{alg:greedymax}. Both algorithms are implemented in Python 3.10 and executed on a Windows 10 machine with a core i$7$, 3.30GHz CPU, and 32GB of memory.


%For each scenario, we determine the best decoy placement under sure and almost-sure winning criterion using Algorithm~\ref{alg:greedymax} and by exhaustively enumerating the solutions to ${{43}\choose{2}} = 1176$ hypergames defined by all possible ways of allocating $2$ decoys among $43$ cells (\ie, the cells devoid of obstacles and real cheese). We also record the solutions to $43 + 42 = 85$ hypergames solved during the two iterations of \texttt{While} loop of Algorithm~\ref{alg:greedymax}. Both the algorithms are implemented in Python 3.10 and run on a Windows 10 machine with a core i$7$, 3.30GHz CPU and a 32GB memory. %\footnote{The code is available at \url{https://github.com/abhibp1993/ggsolver}}.

%For each scenario, we determine the decoy placement using Algorithm~\ref{alg:greedymax} and compare it to the true optimal placement. The true optimal placements are determined enumeratively, \ie, by solving ${{43}\choose{2}} = 1176$ hypergames defined by all possible ways of allocating $2$ decoys among $43$ cells.
%evaluate the positions and the corresponding value of deception (defined below) of the placements generated by Algorithm~\ref{} and compare them to the true optimal placements. The true optimal placements are determined by exhaustively solving all ${43}\choose{2}$ possible ways of placing $2$ decoys among $43$ cells. Additionally, we compare the value of deception when players employ deterministic strategies versus randomized strategies.


To measure the effectiveness of a given placement of traps and fake targets during the iterations of Algorithm~\ref{alg:greedymax}, we introduce a real-valued metric called \emph{value of deception}. Intuitively, the value of deception measures the proportion of P2's winning states in $\game$ that become winning for P1 in the hypergame $\widehat{\hgame}(X, Y)$ or $\widetilde{\hgame}(X, Y)$. When the interaction is analyzed under the sure winning condition and $\win_2(\game, F) \neq F$, the value of deception is defined as follows:
\begin{align*}
	\vod(X, Y) = \frac{|\dswin_1(X, Y)|}{|\win_2(\game, F)| - |F|}
\end{align*}
If $\win_2(\game, F) = F$, \ie, when no states apart from the final states are winning for P2 in $\game$, we set $\vod(X, Y) = 0$. The value of deception is defined analogously when the interaction is analyzed under almost-sure winning criterion. 


%Recall that during each iteration of the \texttt{While} loop in Algorithm~\ref{alg:greedymax}, all valid cells, devoid of real cheese or obstacles or decoys, are evaluated to be the next decoy, and the one yielding the maximum value of deception is selected as the next fake target or a trap. Figure~\ref{fig:results} depicts the map $Z$ constructed during the two iterations on either line \texttt{} or \texttt{} of Algorithm~\ref{alg:greedymax} for the three mentioned scenarios (A)-(C). 


\paragraph*{Insights from Greedy Allocation.} Recall that during each iteration of the \texttt{While} loop in Algorithm~\ref{alg:greedymax}, either on line \texttt{6} or \texttt{13}, we evaluate all eligible cells, devoid of real cheese, obstacles, or decoys, to determine the best choice for the next decoy. The cell with the highest value of deception is selected for placing the next fake target or trap. 


%Figure~\ref{fig:results} depict the map $Z$ created during the each of the two iterations of Algorithm~\ref{alg:greedymax} for each of the three scenarios we consider as a heatmap. Specifically, Figures~\ref{fig:sub-a}-\ref{fig:sub-b} depict the map $Z$ observed during first and second iteration of Algorithm~\ref{alg:greedymax} for scenario (A). Simiarly,   Figures~\ref{fig:sub-c}-\ref{fig:sub-d} depict the map $Z$ for scenario (B), and Figures~\ref{fig:sub-e}-\ref{fig:sub-f} for scenario (C). In Figures~\ref{fig:sub-a}, \ref{fig:sub-c}, and \ref{fig:sub-e}, the value at any cell $(r, c)$ represents the value of deception achieved by placing the first decoy at that cell. For example, ... .
%Similarly, in Figures~\ref{fig:sub-b}, \ref{fig:sub-d}, and \ref{fig:sub-f}, the value at any cell $(r, c)$ represents the combined value of deception achieved by placing the first decoy at the cell determined in the first iteration and the second decoy at that cell.


Figure~\ref{fig:results} displays the map $Z$, depicted as heatmaps, constructed during each of the two iterations of Algorithm~\ref{alg:greedymax} for the three scenarios (A), (B), and (C), when the game is analyzed under sure winning condition. Specifically, Figures~\ref{fig:sub-a} and \ref{fig:sub-b} show the map $Z$ for scenario (A), while Figures~\ref{fig:sub-c} and \ref{fig:sub-d} show it for scenario (B), and Figures~\ref{fig:sub-e} and \ref{fig:sub-f} show it for scenario (C). 


In Figure~\ref{fig:sub-a}, the cell values indicate the value of deception achieved by placing the first trap at each respective cell. For instance, the value $0.28$ in cell $(1, 5)$ indicates the value of deception obtained by placing the first trap at that location. As it is the highest value, the first trap is positioned at $(1, 5)$.


In Figure~\ref{fig:sub-b}, the cell values indicate the combined value of deception achieved by placing the second trap at each cell, in addition to the trap selected in the first iteration. For instance, the value $0.5$ in cell $(5, 5)$ represents the deception value obtained by placing two traps: the first trap at location $(1, 5)$ (as determined in the first iteration) and the second trap at $(5, 5)$. Since the maximum deception value is observed at $(5, 5)$, the second trap is placed there.


The heatmaps in Figures~\ref{fig:sub-c}-\ref{fig:sub-f} can be understood in a similar manner.

%On the other hand, the values shown in Figure~\ref{fig:sub-b} represent the combined value of deception achieved by placing the second trap at each cell, in addition to the trap selected in the first iteration. For instance, in Figure~\ref{fig:sub-a}, the value $0.28$ in cell $(1, 5)$ indicates the value of deception obtained by placing the first trap at that location. As it is the highest value, the first trap is positioned at $(1, 5)$. In Figure~\ref{fig:sub-b}, the value $0.5$ in cell $(5, 5)$ indicates the value of deception obtained by placing two traps; first at location $(1, 5)$, as determined in first iteration, and second at $(5, 5)$. Since the maximum value of deception is observed at $(5, 5)$, the second trap is placed at that cell. The heatmaps in Figures~\ref{fig:sub-c}-\ref{fig:sub-f} are understood similarly. 


%\hrule 

%The cell values shown in Figures~\ref{fig:sub-a}, \ref{fig:sub-c}, and \ref{fig:sub-e}, represent the value of deception achieved by placing the first decoy at that cell.

%In Figures~\ref{fig:sub-a}, \ref{fig:sub-c}, and \ref{fig:sub-e}, the cell values represent the value of deception achieved by placing the first decoy at that cell. Similarly, in Figures~\ref{fig:sub-b}, \ref{fig:sub-d}, and \ref{fig:sub-f}, the cell values represent the combined deception achieved by placing the first decoy determined in the first iteration and the second decoy at that cell.

%\ak{explain how to read the heatmap here.}


%\begin{figure*}[t]
%	
%	\centering
%	
%	\begin{subfigure}{0.3\textwidth}
%		\centering
%		\includegraphics[width=\linewidth]{figures/f0t2_iter0.pdf}
%		\caption{Figure 1}
%		\label{fig:sub1}
%	\end{subfigure}%
%	\hfill
%	\begin{subfigure}{0.3\textwidth}
%		\centering
%		%		\includesvg[width=\linewidth]{figures/f0t2_iter0.svg}
%		\includegraphics[width=\linewidth]{figures/f1t1_iter0.pdf}
%		\caption{Figure 2}
%		\label{fig:sub2}
%	\end{subfigure}%
%	\hfill
%	\begin{subfigure}{0.3\textwidth}
%		\centering
%		%		\includesvg[width=\linewidth]{figures/f0t2_iter0.svg}
%		\includegraphics[width=\linewidth]{figures/f2t0_iter0.pdf}
%		\caption{Figure 3}
%		\label{fig:sub3}
%	\end{subfigure}
%	
%	\vspace{1cm}
%	
%	\begin{subfigure}{0.3\textwidth}
%		\centering
%		%		\includesvg[width=\linewidth]{figures/f0t2_iter0.svg}
%		\includegraphics[width=\linewidth]{figures/f0t2_iter1.pdf}
%		\caption{Figure 4}
%		\label{fig:sub4}
%	\end{subfigure}%
%	\hfill
%	\begin{subfigure}{0.3\textwidth}
%		\centering
%		%		\includesvg[width=\linewidth]{figures/f0t2_iter0.svg}
%		\includegraphics[width=\linewidth]{figures/f1t1_iter1.pdf}
%		\caption{Figure 5}
%		\label{fig:sub5}
%	\end{subfigure}%
%	\hfill
%	\begin{subfigure}{0.3\textwidth}
%		\centering
%		%		\includesvg[width=\linewidth]{figures/f0t2_iter0.svg}
%		\includegraphics[width=\linewidth]{figures/f2t0_iter1.pdf}
%		\caption{Figure 6}
%		\label{fig:sub6}
%	\end{subfigure}
%	
%	\caption{Arrangement of figures}
%	\label{fig:results}
%\end{figure*}


%\begin{figure*}
%	\centering
%	
%	\begin{subfigure}[b]{0.3\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/f0t2_iter0.pdf}
%		\caption{Subfigure A}
%		\label{fig:subfigure_a}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.3\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/f0t2_iter0.pdf}
%		\caption{Subfigure B}
%		\label{fig:subfigure_b}
%	\end{subfigure}
%	
%	\vspace{\baselineskip}
%	
%	\begin{subfigure}[b]{0.3\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/f0t2_iter0.pdf}
%		\caption{Subfigure C}
%		\label{fig:subfigure_c}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.3\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/f0t2_iter0.pdf}
%		\caption{Subfigure D}
%		\label{fig:subfigure_d}
%	\end{subfigure}
%	
%	\vspace{\baselineskip}
%	
%	\begin{subfigure}[b]{0.3\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/f0t2_iter0.pdf}
%		\caption{Subfigure E}
%		\label{fig:subfigure_e}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.3\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/f0t2_iter0.pdf}
%		\caption{Subfigure F}
%		\label{fig:subfigure_f}
%	\end{subfigure}
%	
%	\caption{Six subfigures arranged in two rows and three columns.}
%	\label{fig:subfigures}
%\end{figure*}


\begin{figure*}[!ht]
	\begin{multicols}{3}
		\centering
		\begin{subfigure}{\linewidth}
			\includegraphics[width=\linewidth]{figures/f0t2_iter0.pdf}
			\caption{}
			\label{fig:sub-a}
		\end{subfigure}
		\par
		\begin{subfigure}{\linewidth}
			\includegraphics[width=\linewidth]{figures/f0t2_iter1.pdf}
			\caption{}
			\label{fig:sub-b}
		\end{subfigure}
		\par
		\begin{subfigure}{\linewidth}
			\includegraphics[width=\linewidth]{figures/f1t1_iter0.pdf}
			\caption{} 
			\label{fig:sub-c}
		\end{subfigure}
		\par
		\begin{subfigure}{\linewidth}
			\includegraphics[width=\linewidth]{figures/f1t1_iter1.pdf}
			\caption{}
			\label{fig:sub-d}
		\end{subfigure}
		\par
		\begin{subfigure}{\linewidth}
			\includegraphics[width=\linewidth]{figures/f2t0_iter0.pdf}
			\caption{}
			\label{fig:sub-e}
		\end{subfigure}
		\par
		\begin{subfigure}{\linewidth}
			\includegraphics[width=\linewidth]{figures/f2t0_iter1.pdf}
			\caption{}
			\label{fig:sub-f}
		\end{subfigure}
	\end{multicols}
	\caption{All six.}
	\label{fig:results}
\end{figure*}

%Figure~\ref{fig:results} provides an overview of the results obtained by applying Algorithm~\ref{alg:greedymax} to the three mentioned scenarios (A)-(C). 


%Figure~\ref{fig:sub1} depicts the map $Z$, which is constructed during the first iteration of Algorithm~\ref{alg:greedymax} for scenario (A) where $M=2$ and $N=0$. 


%Figures~\ref{fig:sub1} and \ref{fig:sub4} depict the map $Z$ constructed during the two iterations of \texttt{While} loop on line \texttt{16} of  Algorithm~\ref{alg:greedymax} for scenario (A) where $M=2$ and $N=0$. The value shown within each cell of these figures is the value of deception achieved by placing the next trap within that cell. For instance, the value $0.28$ in the cell $(1, 5)$ is the value of deception achieved by placing the first trap at that cell. Since it is the maximum, the first trap is placed at $(1, 5)$. In Figure~\ref{fig:sub4}, the values in a cell $(r, c)$ represent the value of deception on placing the first trap at $(1, 5)$ and the second at $(r, c)$. Since maximum value of deception is observed at $(5, 5)$, the second trap is placed at that cell. 


%Figures~\ref{fig:sub1} and \ref{fig:sub4} display the map $Z$ created during the two iterations of the \texttt{While} loop, specifically on line \texttt{13} of Algorithm~\ref{alg:greedymax}, for scenario (A) with $M=2$ and $N=0$. The numerical value presented within each cell in these figures represents the value of deception achieved by locating the next trap within that particular cell. For instance, the value $0.28$ in cell $(1, 5)$ indicates the value of deception obtained by placing the first trap at that location. As it is the highest value, the first trap is positioned at $(1, 5)$. In Figure~\ref{fig:sub4}, the value within a cell $(r, c)$ indicate the deception value when placing the first trap at $(1, 5)$ and the second trap at $(r, c)$. Since the maximum deception value is observed at $(5, 5)$, the second trap is placed at that cell.


%Similarly, the Figures~\ref{fig:sub2} and \ref{fig:sub5} display the map $Z$ created on lines \texttt{6} and \texttt{13} of Algorithm~\ref{alg:greedymax}, respectively, for scenario (B) with $M=1$ and $N=1$. And, the Figures~\ref{fig:sub3} and \ref{fig:sub6} display the map $Z$ created on line \texttt{6} of Algorithm~\ref{alg:greedymax} for scenario (C) with $M=0$ and $N=2$. 


We now discuss key observations and insights obtained from Figure~\ref{fig:results}. Observe that when traps are placed, the value of deception increases from left to right. This is due to the fact that traps cut Jerry's winning paths to real cheese. To see this, consider the set of valid initial states determined by the initial locations of Tom and Jerry in the gridworld. This set can be divided into three partitions, each containing a subset of states with a different subjectively rationalizable sure winning strategy for Jerry\footnote{There could be a fourth partition containing states from which Jerry has a subjectively rationalizable sure winning strategy to steal either $(1, 6)$ or $(4, 6)$. However, this partition is empty in our example.}: (i) to steal the cheese at $(1, 6)$ only; (ii) to steal the cheese at $(4, 6)$ only; and (iii) no subjectively rationalizable sure winning strategy available. Among the states in partition (i), consider the states in which Tom starts at $(5, 1)$ and Jerry starts at any of the cells with row coordinate $1$ and column coordinate in $0, \ldots, 5$. Then, in every winning path from an initial state with Jerry at $(1, 0)$ passes, Jerry visits each of the cells in $(1, 1), \ldots, (1, 5)$. Similarly, in every winning path from an initial state with Jerry at $(1, 1)$, Jerry visits each of  cells in $(1, 2), \ldots, (1, 5)$ before visiting cheese, and so on. Thus, by placing a trap closer to $(1, 5)$ cuts a larger number of winning paths, thereby, converting a larger number of Jerry's winning states to Tom's deceptively winning states. Note that placing a trap at $(1, 5)$ does not prevent Jerry from stealing cheese if either Jerry has a winning path that visits a cell containing cheese without visiting $(1, 5)$ or the game starts in partition (ii). 



%To see this, consider the set of all valid initial locations of Tom and Jerry. For a subset of these configurations, Jerry's subjectively rationalizable sure winning strategy is to steal the cheese at $(1, 6)$, for another subset of these Jerry's subjectively rationalizable sure winning strategy is to steal the cheese at $(4, 6)$, and for the rest Jerry has no subjectively rationalizable sure winning strategy to steal any cheese. 


%Consider the first case, where Jerry has a subjectively rationalizable sure winning strategy to steal the cheese at $(1, 6)$. Let Tom start at $(5, 1)$ and Jerry start at any of the cells with row coordinate $1$ and column coordinate among $0\ldots 5$. Then, every winning path from a state with Jerry at $(1, 0)$ passes through each of $(1, 1), \ldots, (1, 5)$ before visiting cheese. Similarly, every winning path from a state with Jerry at $(1, 1)$ passes through each of $(1, 2), \ldots, (1, 5)$ before visiting cheese, and so on. Thus, by placing a trap at $(1, 5)$, Tom can convert a large number of states that are winning for P2 (without traps) to be deceptively winning for him. Of course, placing a trap at $(1, 5)$ does not prevent Jerry from stealing cheese when the game starts with an initial configuration from which Jerry can visit $(1, 6)$ without visiting $(1, 5)$, or from which Jerry has a subjectively rationalizable sure winning strategy to visit $(5, 6)$. 

%\hrule 



%For instance in Figure~\ref{fig:sub-a}, suppose that Jerry starts at any of the cells with row coordinate $1$ and column coordinate among $0, 1, 2$. Then, Jerry's subjectively rationalizable sure winning strategy is to steal the cheese at $(1, 6)$.



%For instance in Figure~\ref{fig:sub-a}, suppose that Tom starts at $(5, 1)$ and Jerry starts at any of the cells with row coordinate $1$ and column coordinate among $0, 1, 2$. Then, Jerry's subjectively rationalizable sure winning strategy is to steal the cheese at $(1, 6)$. In this case, every path that leads Jerry to its goal passes through the cell $(1, 5)$. Thus, by placing a trap at $(1, 5)$, Tom can ensure that Jerry gets trapped and does not steal the cheese. 


%But notice that not all winning paths from aforementioned Jerry's initial positions pass through $(1, 5)$. For example, if Tom starts at $(0, 6)$ and Jerry at $(2, 3)$, then Jerry's subjectively rationalizable sure winning strategy is to steal the cheese at $(4, 6)$ since Tom may catch Jerry if it tries to steal the cheese at $(1, 6)$. Since the number of such initial configurations for which placing the trap at $(1, 5)$ is effective is largest, the value of deception corresponding to $(1, 5)$ is highest. 


%Now, consider the Figure~\ref{fig:sub2} in which we place the first fake cheese in the gridworld. First, we note that the value in any cell is larger than that in the same cell in Figure~\ref{fig:sub1}. This validates our finding that \emph{fake targets are more valuable than traps when the game is analyzed under sure winning condition}. Second, we observe the distribution of value of deception among the eligible cells. Unlike Figure~\ref{fig:sub1}, we see that value in $(2, 3), (3, 3)$ is higher than the neighboring cells. This is because a fake cheese alters Jerry's perception of its goal. Specifically, Jerry thinks that there are three cheese blocks in the environment instead of two. Therefore, when Tom starts at $(5, 1)$ and Jerry starts at any any cell with row coordinate $0, 1, 2$ and column coordinate $0, 1, 2, 3$, Jerry's subjectively rationalizable sure winning strategy would visit the fake cheese at either $(2, 3)$ or $(3, 3)$ instead of visiting $(1, 6)$ or $(4, 6)$. Since Jerry's winning paths from a larger number of initial positions visit $(4, 6)$ than those visiting $(1, 6)$, placing a fake cheese at $(4, 5)$ incentivizes Jerry to visit the fake cheese instead of the real cheese at $(4, 6)$. 


Let's analyze Figure~\ref{fig:sub2}, where the first fake cheese is placed in the gridworld. Firstly, we observe that the values in each cell are greater than the corresponding cells in Figure~\ref{fig:sub1}. This confirms our conclusion that \emph{fake targets hold higher value than traps when considering a certain victory condition}. Secondly, we examine the distribution of deception values among eligible cells. Unlike Figure~\ref{fig:sub1}, we notice that the values in cells $(2, 3)$ and $(3, 3)$ are higher than their neighboring cells. This is due to the fake cheese altering Jerry's perception of the goal. Jerry believes there are three cheese blocks instead of two. Consequently, when Tom starts at $(5, 1)$ and Jerry starts at any cell with row coordinates of $0, 1, 2$ and column coordinates of $0, 1, 2, 3$, Jerry's subjectively rational winning strategy would lead him to visit either the fake cheese at $(2, 3)$ or $(3, 3)$ instead of the real cheese at $(1, 6)$ or $(4, 6)$. Since Jerry's winning paths from a larger set of initial positions include $(4, 6)$ rather than $(1, 6)$, placing a fake cheese at $(4, 5)$ encourages Jerry to visit the fake cheese rather than the real cheese at $(4, 6)$.


Next, we compare Figure~\ref{fig:sub-a} with Figure~\ref{fig:sub-c}, and Figure~\ref{fig:sub-d} with Figure~\ref{fig:sub-f}. In both cases, we observe that the second heatmap shows higher value of deception than the first heatmap for any given cell. This affirms our conclusion that \emph{fake targets hold higher value than traps when the game is analyzed under sure winning condition}. To understand this further, we examine the distribution of value of deception in the heatmaps when fake cheese is being placed. 
%For instance, in Figure~\ref{fig:sub-f}, we notice a pattern of increasing value of deception converging at $(1, 5)$. This is because, firstly, by placing a fake cheese at $(4, 5)$ during first iteration, Tom has incentivized Jerry to visit the fake cheese instead of the real one from a large number of states from which Jerry had a subjectively rationalizable sure winning strategy to visit $(4, 6)$. Therefore, from a majority of Jerry's sure winning states, Jerry's strategy is to visit $(1, 6)$. 
For instance, in Figure~\ref{fig:sub-c}, we notice that the values in cells $(2, 3)$ and $(3, 3)$ are higher than their neighboring cells. This is because the fake cheese alters Jerry's perception of the game. That is, when fake cheese is present at either of these cells, Jerry believes there are three cheese blocks in the game instead of two. Consequently, when Tom starts at $(5, 1)$ and Jerry starts at any cell with row coordinates of $0, 1, 2$ and column coordinates of $0, 1, 2$, Jerry's subjectively rationalizable sure winning strategy would lead him to visit either the fake cheese at $(2, 3)$ or $(3, 3)$ instead of the real cheese at $(1, 6)$ or $(4, 6)$. Since highest value of deception is observed at cell $(4, 5)$, Tom places the first fake cheese at that cell. 


%% =================================================================================
%% DO NOT DELETE. 
%% =================================================================================
%It is important to note that Tom's strategy plays an important role in influencing Jerry's decision. \ak{Get some interesting strategy.}
%\aknote{Number of ways to place M identical traps and N identical fakes in K nodes is ${K \choose {M + N}} {{M+N} \choose {M}}$.}
%% =================================================================================
	

%Since Jerry's winning paths from a larger number of states include $(4, 6)$ rather than $(1, 6)$, placing a fake cheese at $(4, 5)$ encourages Jerry to visit the fake cheese rather than the real cheese at $(4, 6)$.


%Each valid cell, devoid of real cheese or obstacles, is evaluated as a potential trap location, and the corresponding value of deception is displayed within the respective cell. Cells that are not considered for trap placement are assigned a deception value of $0.0$. The maximum value of deception is observed in cell $(1, 5)$, leading to the placement of the first trap in that cell. Subsequently, Figure~\ref{} depicts the updated map $Z$ during the second iteration, where the deception values in the cell $(x, y)$ reflect the combined effect of placing a trap at $(1, 5)$ and $(x, y)$. Therefore, these values are larger compared to those in Figure~\ref{}. Notably, in the second iteration, the cell $(1, 5)$ has a deception value of $0.0$ in Figure~\ref{} since it is not considered as a potential decoy during the second iteration. Figures~\ref{} and \ref{} illustrate the map $Z$ for the placement of the first fake cheese and then trap for the scenario where $M=1$ and $N=1$. Similarly, Figures~\ref{} and \ref{} depict the map $Z$ for the sequential placement of two fake targets for the scenario where $M=0$ and $N=2$. 


% Left to right trend. Path cutting.
%Figure~\ref{} highlights the key findings discussed in our paper. In Figures~\ref{} and \ref{}, we observe the value of deception increases as the cell get closer to the real cheese, for example, from left to right. This is because by placing a trap closer to the real cheese, more of Jerry's winning paths are cut and, therefore, Jerry can reach true cheese with surety from a fewer number of states. 

% Fakes cut paths + attract paths. E.g. placing fake at (4, 5) because it attracts paths from (3, 5). 
%In scenario (B), when Tom can place a fake target and a trap, first the fake target is placed. Notice how the value of deception at the cells near $(2, 3), (3, 3), (4, 5)$ decrease in concentric circles centered at these cells. This is because the fake targets incentivize Jerry, who is following a greedy sure winning strategy, to take the fake cheese instead of the real one. Once a fake target is placed, the trap placement exhibits a similar pattern as seen for scenario (A). 


% First fake is the same VoD. Second one VoD increases for same placement. 
%In scenario (C), when Tom is to place two fake targets, we observe a pattern similar to Figure~\ref{} where the value of deception decreases in circle-like fashion. Notice that the decoys identified in scenarios (B) and (C) are the same. However, the value of deception when $(1, 5), (4, 5)$ are placed as fake targets is more than when a trap is placed at $(1, 5)$. This is expected because of Theorem~\ref{}, which states that, fake targets are are more valuable than traps when the game is analyzed under sure winning criterion. 


% Compare to true optimal. 
\paragraph*{Greedy vs. True Optimal Placement.} Next, we compare the placement returned by Algorithm~\ref{alg:greedymax} with the true optimal placement. For scenario (A), the greedy algorithm selects the cells $(5, 5), (1, 5)$ for two traps; for scenario (B), it selects the cell $(4, 5)$ to place fake cheese and $(1, 5)$ for the trap; and for scenario (C), it selects the cells $(4, 5), (1, 5)$ for placing the two fake cheese blocks. The respective placements yield $0.5, 0.75,$ and $0.81$ as the value of deception. By solving the ${43 \choose 2}$ hypergames, we identify the true optimal placements to be: $(5, 5), (1, 5)$ scenario (A) with a value of deception $0.5$; $(4, 5), (1, 5)$ scenario (B) with a value of deception $0.75$; and $(4, 5), (1, 5)$ scenario (C) with a value of deception $0.81$. 


%Algorithm~\ref{} identifies placing two traps at $\{(5, 5), (1, 5)\}$ to be the near-optimal decoy placement for scenario (A), placing a fake cheese at $(4, 5)$ and a trap at $(1, 5)$ to be near-optimal placement for scenario (B), and placing two fake cheese at $\{(4, 5), (1, 5)\}$ to be near-optimal placement for scenario (C). When compared with the true-optimal allocation, which we compute by enumerating all ${{43}\choose{2}} = 1176$  possible placements of decoys, we find $\{(), ()\}$ to be optimal for scenario (A) with a value of deception $??$, $\{(), ()\}$ to be optimal for scenario (B) with a value of deception $??$, and $\{(), ()\}$ to be optimal for scenario (C) with a value of deception $??$. 


We observe that the value of deception for the greedy placement is within a $(1 - 1/e)$ factor of the true optimal value of deception even though the game does not satisfy the conditions for sub- or super-modularity. As is the advantage of greedy approaches, Algorithm~\ref{alg:greedymax} returns a solution much faster than the enumerative ones. For our problem instance, Algorithm~\ref{alg:greedymax} required $??$ seconds, on average, to return the solution whereas the enumerative approach required around $??$ seconds. Thus, we find that Algorithm~\ref{alg:greedymax} could still be a useful heuristic approach that recommends an effective decoy placement for problem instances not satisfying the conditions in Theorem~\ref{}.   


% ASWin. Same VoD as 2 trap allocation. 
\paragraph*{Analysis under Almost-sure Winning Criterion.} Lastly, when the game is analyzed under the almost-sure winning condition, the map $Z$ is identical to that shown in Figures~\ref{} and \ref{} for all three scenarios (A)-(C). This is expected because fake targets are no more advantageous than traps are under almost-sure winning condition. 



==> sections/fakes.tex <==
\paragraph*{} In this subsection, we analyze the effect of fake target allocation. Because P2 misperceives the fake targets to contain valuable information but is unable to recognize them as decoys, the underlying graph of P2's perceptual game is the same as the base game with no decoys. However, P2 perceives $F \cup Y$ to be final states instead of $F$.


\paragraph*{} As in Section~\ref{subsec:traps}, we consider three games while analyzing the L2-hypergame $\hgame_2$: (i) the base game $\game$ containing no decoys with P2's reachability objective $F$, (ii) P1's perceptual (true) game $\game_Y^1$ with fake targets at $Y \subseteq S$ and P2's reachability objective $F$, and (iii) P2's perceptual game $\game_Y^2$ with P2's reachability objective $F \cup Y$. For clarity, we include the final states when writing winning regions; for example, $\win_1(\game_Y^1; F)$ denotes P1's winning region in the true game when P2's objective is to visit $F$. 


\paragraph*{} We analyze the effect of allocating fake targets in $\win_1(\game, F)$ and $\win_2(\game, F)$ separately. 


\begin{proposition}
	\label{prop:fakes-p1-perceptual-win-regions}
	%	
	Let $Y \subseteq \win_1(\game, F)$. The following statements hold in P1's perceptual game $\game^1_Y$ and P2's perceptual game $\game^2_Y$.
	
	\begin{enumerate}
		\item $\win_1(\game^1_Y, F) = \win_1(\game, F)$.  
		\item $\win_2(\game^1_Y, F) = \win_2(\game, F)$.
		\item $\win_2(\game^2_Y, F \cup Y) \supseteq \win_2(\game, F)$.
		\item $\win_1(\game^2_Y, F \cup Y) \subseteq \win_1(\game, F)$.
	\end{enumerate}
\end{proposition}
\begin{proof}[Proof (Sketch)]
	Because the proof is similar to Proposition~\ref{prop:traps-p1-perceptual-win-regions}, we highlight key observations. The truth of statement (1) is based on the two observations: (a) Allocating a state as fake target converts it to a sink state in $\game_Y^1$. Apart from this, $\game_Y^1$ is identical to $\game$. (b) Marking a state $s \in \win_1(\game, F)$ as `sink' keeps it a P1's winning state in $\game_Y^1$ because, on visiting $s$, the game remains at $s$ indefinitely. Statement (2) follows from (1) using Fact~\ref{fact:determinacy}. Statement (3) is true because, for any two reachability objectives of P2 over the sets $Z_1, Z_2 \subseteq S$ such that $Z_1 \subseteq Z_2$, we have $\win_2(\game, Z_1) \subseteq \win_2(\game, Z_2)$.  Statement (4) follows from (3) using Fact~\ref{fact:determinacy}.
\end{proof}

%\paragraph*{} The truth of statement (1) is based on the two observations: (a) Allocating a state as fake target converts it to a sink state in $\game_Y^1$. Apart from this, $\game_Y^1$ is identical to $\game$. (b) Marking a state as `sink' keeps it a P1's winning state in the safety objective. The remaining proof is similar to that of Proposition~\ref{prop:traps-p1-perceptual-win-regions}. Statement (2) follows from (1) using Fact~\ref{fact:determinacy}. Statement (3) is true because, for any two reachability objectives of P2 over the sets $I, J \subseteq S$ such that $I \subseteq J$, we have $\win_2(\game, I) \subseteq \win_2(\game, J)$.  Statement (4) follows from (3) using Fact~\ref{fact:determinacy}.


\paragraph*{} In words, the winning regions of both players in true game $\game_Y^1$ are the same as that in the base game $\game$. However, P2 may perceive its winning region to be larger than that in the base game due to presence of fake targets. As a result, P1 may get an advantage if it can enforce a visit to $\win_2(\game_Y^2, F \cup Y) \cap \win_1(\game, F)$, which is perceptually winning for P2 but truly winning for P1. In fact, from any state in $\win_2(\game_Y^2, F \cup Y) \cap \win_1(\game, F)$, P1 can not only guarantee satisfying its safety objective but also ensure a visit to $Y$. Such a strategy is valuable in applications such as cybersecurity where an attacker visiting a honeypot could help the defender learn about the attacker's identity, intention, etc. \cite{}. 


%\paragraph*{} As a result of statement (3) in  Proposition~\ref{fakes-p1-perceptual-win-regions}, P2's perceived winning region includes some states from $\win_1(\game, F)$. Hence, there exists a possibility that by using a sure winning strategy in its perceptual game, P2 might visit a state in $\win_1(\game, F)$. Specifically, such a state would be a part of $\win_2(\game_Y^2, F \cup Y) \cap \win_1(\game, F)$. Once such a state is visited, P1 has a strategy to enforce its safety objective of preventing the game from reaching $F$. In fact, from any state in $\win_2(\game_Y^2, F \cup Y) \cap \win_1(\game, F)$, P1 can enforce a visit to $Y$. 


\begin{proposition}
	From every state in $\win_2(\game_Y^2, F \cup Y) \cap \win_1(\game, F)$, P1 has a sure winning strategy to visit $Y$.
\end{proposition}
\begin{proof}[Proof (Sketch)]
	Given that both players play subjectively rationalizable strategies, P2's strategy at a state in $\win_2(\game_Y^2, F \cup Y)$ ensures a visit to either $F$ or $Y$. But from any state in $\win_1(\game, F)$, P1's strategy prevents a visit to $F$. Therefore, the game must visit $Y$ \deleted{from any state in $\win_2(\game_Y^2, F \cup Y) \cap \win_1(\game, F)$}.
\end{proof}


\paragraph*{} Now, consider placement of fake targets in $\win_2(\game, F)$. We observe the subset relations are similar to that of placing traps in $\win_2(\game, F)$. 


\begin{proposition}
	\label{prop:fakes-p2-perceptual-win-regions}
	%	
	Let $Y \subseteq \win_2(\game, F) \setminus F$. The following statements hold in P1's perceptual game $\game^1_Y$ and P2's perceptual game $\game^2_Y$.
	
	\begin{enumerate}
		\item $\win_2(\game^1_Y, F) \subseteq \win_2(\game, F)$.
		\item $\win_1(\game^1_Y, F) \supseteq \win_1(\game, F)$.  
		\item $\win_2(\game^2_Y, F \cup Y) = \win_2(\game, F)$.
		\item $\win_1(\game^2_Y, F \cup Y) = \win_1(\game, F)$.
	\end{enumerate}
\end{proposition}
\begin{proof}[Proof (Sketch)]
	Since the proofs are similar in principle to those in Propositions~\ref{prop:traps-p2-perceptual-win-regions}-\ref{prop:traps-p1-perceptual-win-regions}, we discuss the insight behind the proof.
	
	(1). First, observe that P2 cannot visit $F$ from any state in $Y$ because they are sink states in $\game_Y^1$. Hence, the states from which P1 has a sure winning strategy to visit $Y$ in $\win_2(\game)$ become winning for P1 in $\game_Y^1$. To see why no state in $\win_1(\game)$ becomes winning for P2 in $\game_Y^1$, note that placing fake targets in $\win_2(\game)$ does not affect any sure winning strategy of P1 from any state in $\win_1(\game)$ to satisfy its safety objective. This is because, on allocating fake targets, neither P2 gains new actions that would allow it to enter $\win_2(\game)$, nor does P1 lose any actions that would prevent it to remain in $\win_1(\game)$ indefinitely.	
	
	
	(3) In $\game_Y^2$, P2 misperceives a subset of states in $\win_2(\game, F)$ to be final states. However, the underlying graphs of both the games are identical. As a result, every state $s \in \win_2(\game, F)$ is also winning for P2 in $\game_Y^2$. Also, there is no P2 state in $\win_1(\game)$ that would become winning for P2 in $\game_Y^2$ because, otherwise, it would have been winning for P2 in $\game$ itself. Similarly, no P1 state in $\win_1(\game)$ would be winning for P2 in $\game_Y^2$. Thus, $\win_2(\game^2_Y, F \cup Y) = \win_2(\game, F)$.
	
	(2), (4) follow from (1), (3) using Fact~\ref{fact:determinacy}. 
\end{proof}


\paragraph*{} Although traps and fake targets behave similarly when considering the subset relations, allocating fake targets could be advantageous for P1 over allocating traps. The following example illustrates why. 


\begin{example}
	Consider the toy problem shown in Figure~\ref{fig:fake-betterthan-traps}. Suppose that we are given a single decoy placed at $s_0$. We are to decide whether it should be configured as a trap or a fake target. 
	
%	\begin{figure}[tb!]
%		\begin{center}
%			\subfigure[Game with no fake targets.]{
%				\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.5cm, scale = 0.4,transform shape]
%					
%					\node[state]              (0) [] {\Large $s_0$};
%					\node[state, rectangle]   (1) [below left of=0] {\Large $s_1$};
%					\node[state, rectangle]   (2) [below right of=0] {\Large $s_2$};
%					\node[state, rectangle]   (3) [below left of=1] {\Large $s_3$};
%					\node[state]              (4) [below right of=1] {\Large $s_4$};
%					\node[state]              (5) [below right of=2] {\Large $s_5$};
%					\node[state, rectangle, accepting] (6) [below right of=3] {\Large $s_6$};
%					\node[state, accepting]   (7) [below left of=5] {\Large $s_7$};
%					
%					\path 
%					(0) edge [bend left] node[above left=-5pt] 			{\Large $a_1$}  (1)
%					(0) edge             node[above=2pt] 			 	{\Large $a_2$}  (2)
%					(1) edge [bend left] node[above left=-5pt] 			{\Large $b_1$}  (0)
%					(1) edge [bend left] node[above left=-5pt] 			{\Large $b_2$}  (3)        
%					(1) edge             node[above right=-5pt] 		{\Large $b_3$}  (4)    
%					(2) edge             node[above left=-5pt] 			{\Large $b_1$}  (4)        
%					(2) edge             node[above right=-5pt] 		{\Large $b_2$}  (5) 
%					(3) edge [bend left] node[above left=-5pt] 	  		{\Large $b_1$}  (1) 
%					(3) edge             node[above right=-5pt] 		{\Large $b_2$}  (6) 
%					(4) edge             node[above left=-5pt]  		{\Large $b_1$}  (6) 
%					(4) edge             node[above right=-5pt] 		{\Large $b_2$}  (7) 
%					(5) edge             node[above left=-5pt]  		{\Large $a_2$}  (7) 
%					;
%				\end{tikzpicture}
%			}
%			\hfill
%			\subfigure[Game with fake target at $s_0$.]{
%				\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3.5cm, scale = 0.35,transform shape]
%					\node[state]              (0) [] {\Large $s_0$};
%					\node[state, rectangle]   (1) [above left of=0] {\Large $s_1$};
%					\node[state, rectangle, accepting] (6) [right of=0] {\Large $s_6$};
%					\node[state, accepting]   (7) [right of=6] {\Large $s_7$};
%					\node[state, rectangle]   (3) [right of=1] {\Large $s_3$};
%					\node[state]              (4) [right of=3] {\Large $s_4$};
%					\node[state]              (5) [right of=4] {\Large $s_5$};
%					\node[state, rectangle]   (2) [above right of=3] {\Large $s_2$};
%					
%					\path 
%					(0) edge [bend left] node[left] 			{\Large $a_1$}  (1)
%					(0) edge [bend right, out=-10]            node[above=2pt, pos=0.1] 			 	{\Large $a_2$}  (2)
%					(1) edge             node[above right=-5pt] 			{\Large $b_1$}  (0)
%					(1) edge [bend left] node[above left=-5pt] 			{\Large $b_2$}  (3)        
%					(1) edge [bend left, out=60] node[above right=-5pt] 		{\Large $b_3$}  (4)    
%					(2) edge             node[above right=-5pt] 			{\Large $b_1$}  (4)        
%					(2) edge             node[above right=-5pt] 		{\Large $b_2$}  (5) 
%					(3) edge             node[above left=-5pt] 	  		{\Large $b_1$}  (1) 
%					(3) edge             node[right] 		{\Large $b_2$}  (6) 
%					(4) edge             node[above left=-5pt]  		{\Large $b_1$}  (6) 
%					(4) edge             node[above right=-5pt] 		{\Large $b_2$}  (7) 
%					(5) edge             node[above left=-5pt]  		{\Large $a_2$}  (7) 
%					;
%				\end{tikzpicture}
%			}
%		\end{center}
%		\caption{A toy problem demonstrating how fake targets could be more effective than traps.}
%		\label{fig:fake-betterthan-traps}
%	\end{figure}
	\aknote{Add back Image}
	
	First, note that all states in Figure~\ref{fig:fake-betterthan-traps} are winning for P2 in its objective to reach $F = \{s_6, s_7\}$. Using Algorithm~\ref{alg:zielonka}, the level sets are determined to be $[\{s_6, s_7\}, \{s_3, s_4, s_5\}, \{s_1, s_2\}, \{s_0\}]$ where the final states are assigned the lowest rank $0$ and $s_0$ is assigned the highest rank $3$. 
	
	When $s_0$ is configured as a trap, the only P2 state that becomes winning for P1 is $s_0$. However, when it is configured as a fake target, the states $s_0$ and $s_1$ become winning for P1. This is because when $s_0$ is a fake target, it is considered a final state in $\game_Y^2$. Hence, it's rank becomes $0$. The rank of P2 state $s_1$ becomes $1$ because P2 can reach from $s_1$ to $s_0$ in one-step using action $b_1$. As a result, in P2's perception, the action $b_1$ is subjectively rationalizable but action $b_2$ (which is truly a rational action) is not, since, by using $b_2$, it would take two-steps to visit $F$. 
	
	It is noted that the state $s_3$ from which P2 has a strategy to surely visit $s_0$ is not subjectively rationalizable for P2 in its perceptual game. Again, this is because it can visit the final state $s_6$ in one-step using $b_2$, whereas it would take two-steps to visit $s_0$. \qed
\end{example} 
\ak{Can use Fig. 2(b) to elaborate.}


\begin{proposition}
	Let $Z \subseteq \win_2(\game) \setminus F$. P1's winning regions in true games $\game_{Z, \emptyset}^1$ and $\game_{\emptyset, Z}^1$, where the set $Z$ is allocated as traps in the former game and as fake targets in the latter, satisfy the condition that $\win_1(\game) \subseteq \win_1(\game_{Z, \emptyset}) \subseteq \win_1(\game_{\emptyset, Z})$. 
\end{proposition}
\begin{proof}[Proof (Sketch)]
	Recall that a subjectively rationalizable strategy for P2 is a rank reducing strategy in the attractor whereas every P1 action at any P1 state in P2's winning region is rank reducing. Consider the game $\game_{Z, \emptyset}$ in which the states in $Z$ are allocated as traps. Then, every state in $\dswin_1$ must have a rank greater than or equal to the smallest rank of any state in $Z$. Since allocating the same set $Z$ as fake targets sets the rank of states in $Z$ to $0$, every subjectively rationalizable strategy at $s \in \dswin_1$ in $\game_{Z, \emptyset}$ remains subjectively rationalizable remains in $\game_{\emptyset, Z}$. 
%	
%	Consider a state $s \in \win_2(\game) \setminus F$ with rank $k$. If there exists a strategy $\pi_1$ to visit $Z$ in $\game_{Z, \emptyset}$, \ie, when states in $Z$ are configured as traps, then visited trap's rank $k'$ must be strictly smaller rank than $k$. On allocating $Z$ as fake targets, $k' \rightarrow 0$. Hence, $\pi_2$ used before must remain subjectively rationalizable. Above example shows a case where $\win_1(\game_{\emptyset, Z})$ contains a state not in $\win_1(\game_{Z, \emptyset})$. 
\end{proof}


\hrule
\ak{Add paragraph on DSWin1, DSWin2 and SRActs.}

\paragraph*{} While P1 does not have a sure winning strategy to satisfy its safety objective from any state in $\win_2(\game, F)$, P2 might follow a strategy to visit $Y$ instead of $F$ due to misperception. Thus, using a similar argument as Proposition~\ref{prop:traps-dswin2}, the states from which P2 is guaranteed to visit $F$, even when it misperceives $Y$ as final states, is the subset of states in $\win_2(\game, F)$ that are disconnected from $Y$ \replaced{in the underlying graph of $\game$.}{under every pair of subjectively rationalizable strategies of P1 and P2.} 
\ak{An example would help here. Add a few states to Ex. 2?}


%\hrule 
%
%Intuitively, in this case, fake targets behave like traps. By placing a fake target at a state $s$, the state is converted to `sink', thereby, cutting any winning path that visits $s$. \ak{use an example to explain.}
%
%
%\begin{lemma}
%	Let $Z \subseteq \win_2(\game, F)$. P1 and P2's perceptual winning regions when $Z$ is allocated as traps and when it is allocated as fake targets is identical.
%\end{lemma}
%
%
%\paragraph*{} In practice, P2 considers fake targets $Y = Z$ to be final states. Therefore, it could visit $Y$ by choice. On the contrary, P2 may visit a trap in $X = Z$ inadvertently. But since we assume that P2 has no preference between visiting $F$ and $Y$, marking a winning state as fake target has no effect on subjectively rationalizable actions/strategy of P2.  
%\ak{rewrite last sentence.}
%
%
%\begin{proposition}
%	\label{prop:fakes-p2-perceptual-win-regions}
%	%	
%	Let $Y \subseteq \win_2(\game, F)$. The following statements hold in P1's perceptual game $\game^1_Y$ and P2's perceptual game $\game^2_Y$.
%	
%	\begin{enumerate}
%		\item $\win_1(\game^1_Y, F) \supseteq \win_1(\game, F)$.  
%		\item $\win_2(\game^1_Y, F) \subseteq \win_2(\game, F)$.
%		\item $\win_1(\game^2_Y, F \cup Y) = \win_1(\game, F)$.
%		\item $\win_2(\game^2_Y, F \cup Y) = \win_2(\game, F)$.
%	\end{enumerate}
%\end{proposition}
%
%
%\paragraph*{} Since fake targets behave like traps when allocated in $\win_2(\game, F)$, P1's deceptive sure winning region can be determined by solving the game $\widehat \hgame_1$ from Definition~\ref{def:hgame-labeling-misperception} and replacing $X$ by $Y$. It is also easy to see that the result of Proposition~\ref{prop:traps-dswin1} applies to the case of fake targets. 
%


==> sections/general_effect.tex <==
Consider two games $G$ and $G^2$
\begin{itemize}
\item Case 1:  $G^2$ has the same dynamics as $G$ except the set $X$ of states are marked as sinks.
\item  Case 2:  $G^2$ has the same dynamics as $G$ except the set $F\cup Y$ of states are marked as P2's reachability objectives.
\item Case 3:  $G^2$ has the same dynamics as $G$ except the set $F\cup Y$ of states are marked as P2's reachability objectives and the set $X$ of states are marked as sinks. 
\end{itemize}

Let $\win_i$ and $\win_i^2$ be winning region for player $i$ in game $G$ and $G^2$ respectively.

\begin{proposition}
In case 1, 
\begin{itemize}
    \item if $X\subseteq \win_1 $, then $\win_1 = \win_1^2$ and $\win_2=\win_2^2$.
    \item if $X\cap \win_2\ne \emptyset$, then $\win_1 \subseteq \win_1^2$ and $\win_2\supseteq \win_2^2$.
\end{itemize}
\end{proposition}



\begin{proposition}
In case 2, ...
\end{proposition}




\begin{proposition}
In case 3, ...
\end{proposition}

\jf{are these three propositions capturing what you intend to express? actually I am not sure if case 3 is   needed. }

==> sections/hypergame.tex <==
%\jf{preliminaries?}

\paragraph*{} When decoys are allocated in $\game$, P1 and P2 interact with different subjective views of their interaction. P1 has complete information about the location and type of the decoys whereas P2 does not. The two types of decoys influence P2's decision-making in different manner. In this section, we define a hypergame model to represent the interaction between P1 and P2 under incomplete information. 

\jf{should define what is the effect of trap and fake target first.}
 
\paragraph*{} We start by formalizing the notion of \textit{perceptual games} of P1 and P2. First, we define a game model containing traps and fake targets.

\jf{in the definition, $F$ is defined after the first usage of the set.}

\begin{definition}[True Game]
	\label{def:game-traps-faketargets}
	Given a game $\game$, let $X$ and $Y$ be two subsets of $S \setminus F$ such that $X \cap Y = \emptyset$. The deterministic two-player turn-based complete information game representing the interaction between P1 and P2 when the states in $X$ are allocated as traps and those in $Y$ are allocated as fake targets is the tuple,
	\[
		\game_{X,Y} = \langle S, A, T_{X,Y}, s_0, F \rangle,
	\]
	where 
	\begin{itemize}
		\item $S$ and $A$ are defined as in Definition~\ref{def:game};
		
		\item $T_{X, Y}$ is a deterministic transition function. Given any state $s \in S$ and any action $a \in A$,
		\begin{align*}
			T_{X, Y}(s, a) = 
			\begin{cases*}
				T(s, a)	& \text{if } $s \notin X \cup Y$  \\
				s & \text{otherwise} 
			\end{cases*}
		\end{align*}
		\item $F$ is a set of states describing P2's reachability objective. 
	\end{itemize}
\end{definition}


\paragraph*{} The states in $\game$ that are allocated as decoys (either traps or fake targets) become `sink' states in $\game_{X, Y}$. A state is called a ``sink state'' if, for any action taken at that state, the game remains at the same state. In cybersecurity, this models the situation that P2 cannot visit any other state once it visits a decoy \cite{}. 


\paragraph*{} Since P1 has complete information about the interaction, P1 knows the true game, $\game_{X, Y}$. On the other hand, we assume that \replaced{P2 is unaware of the presence of decoys}{P2 is unable to recognize a state in $X \cup Y$ to be a decoy}. As a result, P2 does not mark the states in $X \cup Y$ as sink states but instead considers the states in $Y$ to be goal states. 
\aknote{Reviewers may ask to justify unawareness. Isn't it common for an attacker to anticipate existence of a traps or fake target?}

\jf{describe the two effects of decoys first. before talking about true game and P2's perceptual game.}


\begin{definition}[P2's Perceptual Game]
	\label{def:p2-perceptual-game}
	% 
	P2's perceptual game is a tuple 
	\[
		\game^2_{X,Y} = \langle S, A, T, s_0, F \cup Y \rangle,
	\]
	where 
	\begin{itemize}
		\item $S$, $A$, $T$, $s_0$ have the same meanings as Definition~\ref{def:game};
		
		\item $F\cup Y$ is a set of states describing P2's reachability objective, perceived by P2. 
	\end{itemize}
\end{definition}


\paragraph*{} As a result of P2's misperception, P2 perceives the transition function $T$ in game $\game_{X, Y}$ to be the same as that in base game, $\game$. A special case occurs when P1 allocates no fake targets, \ie, $Y = \emptyset$, in which case $\game_{X, Y}^2 = \game$. 


\paragraph*{} The information structure of the interaction between P1 and P2 is captured by following assumption.


\begin{assumption}[Information Structure]
	\label{assume:information-structure}
	P1 knows the true game, $\game_{X, Y}$. P2 does not know the existence of traps and fake targets. Therefore, P2 misperceives the true game as $\game^2_{X, Y}$. P1 is knows that P2 is unaware of traps and fake targets.
\end{assumption}


%=============================================================================================================
% MOVE TO LATER SECTION.
%=============================================================================================================

%\paragraph*{Notation.} In this paper, we denote the base game as $\game$ and the winning regions of P1 and P2 in $\game$ as $\win_1$ and $\win_2$, respectively. P1's perceptual game, which is also the true game, is written as $\game^1_{X, Y} := \game_{X, Y}$, and the winning regions of P1 and P2 in $\game^1_{X, Y}$ by $\win_1^1$ and $\win_2^1$, respectively. Similarly, P2's perceptual game is  $\game^2_{X, Y}$ and the winning regions are $\win_1^2$ and $\win_2^2$. We reserve symbols $X, Y$ specially for traps and fake targets. The superscript is used to indicate that the game or winning region under consideration belongs to which player's perceptual game.

%=============================================================================================================

%It remains unaffected in P2's perceptual game because P2 cannot locate the traps or fake targets. Instead, P2 considers the states in $Y$ as target states because P2 misperceives the fake targets to be valuable resources.


%\paragraph*{} Since we consider one-shot interaction, we assume that P1 is aware that P2 does not know the location of traps and fake targets. \ak{Find supporting references and say why this assumption is reasonable.} 
%
%
%\begin{assumption}
%	P1 is aware that P2 does not know the location of traps and fake targets.
%\end{assumption}


\paragraph*{} The interaction between P1 and P2 under Assumption~\ref{assume:information-structure} is a game with incomplete information \deleted{due to P2's unawareness}. Thus, we model the interaction and the hierarchical information structure outlined in the assumption using hypergame \replaced{modeling}{theory} \cite{Bennett1977}. A hypergame models an interaction with incomplete information, in which different players have subjective views about the true game and about the perceptual games of other players. 

%To capture the hierarchical information structure outlined in the assumption, we adopt hypergame theory \cite{Bennett1977}. A hypergame models an interaction with incomplete information, in which different players have subjective views about the game and about the perceptual games of other players. Specifically, we define a hypergame to model P1's awareness of the true game $\game_{X, Y}$, P2's misperception of the game as $\game^2_{X, Y}$, and P1's knowledge of P2's perceptual game $\game^2_{X, Y}$.
%\ak{rewrite. Highlight necessity of hypergame.}


\begin{definition}[L1- and L2-hypergame] 
	\label{def:generalized-hypergame}
	%	Let $X$ be a set of states allocated with traps and $Y$ be a set of states allocated with fake targets. 
	Given the perceptual games $\game^1_{X,Y} \coloneqq \game_{X, Y}$ and $\game^2_{X,Y}$ of P1 and P2, respectively, the L1-hypergame is defined as a tuple of the perceptual games, 
	\[
		\hgame_1(X, Y) = \langle \game^1_{X,Y}, \game^2_{X,Y} \rangle. 
	\]
	In an L1-hypergame, neither of the players is aware of the other player's misperception. That is, P1 believes that P2 plays according to $\game^1_{X,Y}$ and P2 believes that P1 plays according to $\game^2_{X,Y}$.
	
	The L2-hypergame between P1 and P2 is the tuple, 
	\[
		\hgame_2(X, Y) = \langle \hgame_1(X, Y), \game^2_{X,Y} \rangle.
	\] 
	In L2-hypergame, P1 is aware of P2's perceptual game.
\end{definition}


\paragraph*{} In an L1-hypergame, P1 decides its strategy by solving the game $\game^1_{X, Y}$.  P1 assumes that P2 will play a strategy that is rational in $\game^1_{X, Y}$. Whereas, P2 decides its strategy by solving the game $\game^2_{X, Y}$ and assumes P1 to play a strategy that is rational in $\game^2_{X, Y}$. In an L2-hypergame, P2's strategy is computed in the same way as in the L1-hypergame since its perceptual game remains the same. However, P1, who is now aware of $\game^2_{X, Y}$ in addition to $\game^1_{X, Y}$, can anticipate P2's best response at a given state by solving the game $\game^2_{X, Y}$. If P2's best response at a state is not actually the best response at that state in the true game $\game^1_{X, Y}$, then P1 could leverage it to its advantage. 

\jf{write out L1 as LEVEL-1 and L2 as level-2}

\paragraph*{} In the next section, we \replaced{study}{develop an insight into} how P1 could leverage P2's misperception by analyzing the effects of placing traps and fake targets. Specifically, we characterize the states at which P2's best response in $\game^2_{X, Y}$ is not the best response in the true game, $\game^1_{X, Y}$. Based on it, in Section~\ref{sec:deception}, we synthesize a \emph{deceptive} strategy for P1, using which P1 can satisfy its safety objective from a state that would be winning for P2 had the game been complete information (\ie, if P2 was aware of the traps and fake targets). In Section~\ref{sec:allocation}, we will use these insights to identify the optimal decoy allocation.

\jf{``characterize the states at which P2's best response in $\game^2_{X, Y}$ is not the best response in the true game, $\game^1_{X, Y}$. ''  what does characterize mean? or do you mean "we identify   states"}

==> sections/hypergame2.tex <==
A deceptive strategy leverages the opponent's misinformation to manipulate them into making \ak{sub-optimal?} choices. In this section, we propose a hypergame-theoretic approach to synthesize a deceptive strategy for P1 when players use deterministic strategies and analyze their perceptual games under sure winning criterion. 

%In our problem, to synthesize a deceptive strategy for P1, we need a way to integrate P2's perceptual game into P1's decision-making. 

A hypergame, introduced in \cite{}, is capable of modeling strategic interactions when players have asymmetrical information. Intuitively, a hypergame is a game of games, and each game is associated with a player’s subjective view of its interaction with other players based on its own information and information about others’ subjective views. Hypergames are defined inductively based on the level of perception of individual players. In this work, we use a level-2 (L2-) hypergame to model the interaction between P1 and P2 under Assumption~\ref{assume:information-structure}. 


%A zeroth-level hypergame is a game with complete, symmetric information, where the perceptual games of both players' are identical to the \emph{true} game. In a first-level hypergame, at least one of the players misperceives the \emph{true} game but neither of them is aware of it. In this case, both players believe their perceptual game to be the \emph{true} game and play according to their perceptual games, which are zeroth-level hypergames. In a second-level hypergame, at least one of the players becomes aware of the misperception and is able to reason about her opponent's perceptual game. Recognizing that a second-level hypergame can represent the information structure given in Assumption~\ref{assume:information-structure}, we use a second-level hypergame\footnote{In general, it is possible define hypergames of an arbitrary level. The interested readers may refer to \cite{wang1989solution} for an elaborate discussion on the higher levels of hypergames.} to model Problem~\ref{prob:decoy-placement}.

%The interaction between P1 and P2 under Assumption~\ref{assume:information-structure} is a game with incomplete information. Thus, we model the interaction and the hierarchical information structure outlined in the assumption using hypergame theory \cite{Bennett1977}. A hypergame models an interaction with incomplete information, in which different players have subjective views about the true game and about the perceptual games of other players. 

%To capture the hierarchical information structure outlined in the assumption, we adopt hypergame theory \cite{Bennett1977}. A hypergame models an interaction with incomplete information, in which different players have subjective views about the game and about the perceptual games of other players. Specifically, we define a hypergame to model P1's awareness of the true game $\game_{X, Y}$, P2's misperception of the game as $\game^2_{X, Y}$, and P1's knowledge of P2's perceptual game $\game^2_{X, Y}$.
%\ak{rewrite. Highlight necessity of hypergame.}


\begin{definition}[L1- and L2-hypergame] 
	\label{def:generalized-hypergame}
	%	Let $X$ be a set of states allocated with traps and $Y$ be a set of states allocated with fake targets. 
	Given the perceptual games $\game^1_{X,Y} \coloneqq \game_{X, Y}$ and $\game^2_{X,Y}$ of P1 and P2, respectively, the level-1 (L1-) hypergame is defined as a tuple of the perceptual games, 
	\[
		\hgame_1(X, Y) = \langle \game^1_{X,Y}, \game^2_{X,Y} \rangle. 
	\]
	In an L1-hypergame, neither of the players is aware of the other player's misperception. That is, P1 believes that P2 plays according to $\game^1_{X,Y}$ and P2 believes that P1 plays according to $\game^2_{X,Y}$.
	
	The level-2 or L2-hypergame between P1 and P2 is the tuple, 
	\[
	\hgame_2(X, Y) = \langle \hgame_1(X, Y), \game^2_{X,Y} \rangle.
	\] 
	In L2-hypergame, P1 is aware of P2's perceptual game. 
\end{definition}


In an L1-hypergame, P1 decides its strategy by solving the game $\game^1_{X, Y}$.  P1 assumes that P2 will play a strategy that is rational in $\game^1_{X, Y}$. Whereas, P2 decides its strategy by solving the game $\game^2_{X, Y}$ and assumes P1 to play a strategy that is rational in $\game^2_{X, Y}$. In an L2-hypergame, P2's decides its strategy in the same way as in the L1-hypergame since its perceptual game remains the same. However, P1, who is now aware of $\game^2_{X, Y}$ in addition to $\game^1_{X, Y}$, can anticipate P2's best response at a given state by solving the game $\game^2_{X, Y}$. Therefore, P1 solves L1-hypergame $\hgame_1(X, Y)$ to compute its strategy in L2-hypergame. Because of this, if P2's best response at a state based on $\game^2_{X, Y}$ is not actually the best response at that state in the true game $\game^1_{X, Y}$, then P1 could leverage it to its advantage. 


Next, we introduce a graph-based model for $\hgame_1(X, Y)$ using which we can synthesize a deceptive strategy for P1. In this model, we start with base game $\game$ and eliminate any P2 action that P2 would not consider rational in its perceptual game $\game_{X, Y}^2$. Similarly, we eliminate any P1 action that P2 would not consider rational for P1 to use in $\game_{X, Y}^2$. The rationale behind eliminating P1 actions is to remain \emph{stealthy}: Assuming P2 expects P1 to be rational, if P1 uses an action that P2 does not expect P1 to use, P2 would become aware of its misperception. We formalize this notion of rationality using the concept of \emph{subjective rationalizability} from game theory. We refer the interested readers to \cite{kulkarni2021deceptive,sasaki2012subjective} for more details. 


\begin{definition}[Subjective Rationalizability under Sure Winning Criterion]
	\label{def:sracts}
	% 
	Let $\game^2_{X, Y}$ be P2's perceptual game. When the game is analyzed under sure winning criterion, an action $a \in A_2$ is said to be \emph{subjectively rationalizable} at a state $s \in S_2 \cap \win_2(\game_{X, Y}^2, F \cup Y)$ if and only if the next state $s' = T(s, a)$ has a strictly smaller rank than $s$ in $\win_2(\game_{X, Y}^2, F \cup Y)$. At any state in $S_1 \cup (S_2 \setminus \win_2(\game_{X, Y}^2, F \cup Y))$, every action is subjectively rationalizable for P2.
%	Given that P1 and P2 use greedy sure-winning strategies and P2's perceptual game $\game^2_{X, Y}$, an action $a \in A_2$ is said to be \emph{subjectively rationalizable} at a state $s \in S_2 \cap \win_2(\game_{X, Y}^2)$ if and only if the rank of state $s' = T(s, a)$ in $\game_{X, Y}^2$ is strictly smaller than that of $s$. At any state in $S_1 \cup (S_2 \setminus \win_2(\game_{X, Y}^2))$, every action is subjectively rationalizable for P2. The set of subjectively rationalizable actions at a state $s \in S$ is denoted by $\srAct(s)$.
\end{definition}



%\hrule 

%In the next section, we \replaced{study}{develop an insight into} how P1 could leverage P2's misperception by analyzing the effects of placing traps and fake targets. Specifically, we characterize the states at which P2's best response in $\game^2_{X, Y}$ is not the best response in the true game, $\game^1_{X, Y}$. Based on it, in Section~\ref{sec:deception}, we synthesize a \emph{deceptive} strategy for P1, using which P1 can satisfy its safety objective from a state that would be winning for P2 had the game been complete information (\ie, if P2 was aware of the traps and fake targets). In Section~\ref{sec:allocation}, we will use these insights to identify the optimal decoy allocation.

%\jf{``characterize the states at which P2's best response in $\game^2_{X, Y}$ is not the best response in the true game, $\game^1_{X, Y}$. ''  what does characterize mean? or do you mean "we identify   states"}


%In this subsection, we show how to synthesize a stealthy deceptive strategy for P1 given a fixed set of decoys based on results from Section~\ref{sec:characterization}. Using this strategy, P1 can enforce a visit to a decoy while preventing P2 to become aware of its misperception.
%In this subsection, we show how to synthesize a stealthy deceptive strategy for P1 given a fixed set of decoys based on results from Section~\ref{sec:characterization}. Using this strategy, P1 can enforce a visit to a decoy while preventing P2 to become aware of its misperception.


%\ak{Recall from previous section that allocation in $\win_2(\game, F) \setminus F$ is necessary for gaining benefit.}


%Suppose the set of decoys $X \cup Y$ containing traps $X$ and fake targets $Y$ is placed in $\win_2(\game, F) \setminus F$. By Lemma~\ref{lma:advantage-of-traps}, P1 can enforce a visit to $X \cup Y$ from a state $s \in \win_2(\game, F) \setminus (F)$ if and only if P1 has a strategy to surely visit $X \cup Y$ from $s$. However, we cannot compute such a strategy by simply solving the following reachability game: $$\langle S, A, T_{X \cup Y}, X \cup Y \rangle,$$ where $X \cup Y$ is P1's reachability objective and $T_{X \cup Y}(s, a) = T(s, a)$ if and only if $T(s, a) \in \win_2(\game, F)$. Otherwise, ${T}_{X \cup Y}(s, a)$ is undefined. The following example demonstrates why this intuition is incorrect. 
%
%
%\begin{example}
%	Consider the game shown in Fig.~\ref{fig:inverted-jobstmann-example}, in which P1 and P2 states are represented by circle and square states, respectively. P2's goal is to reach $F = \{3, 4\}$ shown as accepting states. Using Alg.~\ref{alg:zielonka}, we obtain $\win_1 = \{1, 2\} $ and $\win_2 = \{0, 3, 4, 5, 6, 7\}$. Particularly, the attractor level set obtained is $[\{3, 4\}, \{0\}, \{7\}, \{6\}, \{5\}]$, where the level-$0$ of attractor contains the final states, level-$1$ contains state $0$ and so on. The sure winning strategy at any P2 state in $\win_2$ is the action that reduces the level of attractor. Therefore, $\pi_2(0) = (0, 3)$ and $\pi_2(6) = (6, 7)$.
%	
%	\begin{figure}
%		\centering 
%		\include{figures/inverted-jobstmann}
%		\caption{TODO. }
%		\label{fig:inverted-jobstmann-example}
%	\end{figure}
%	
%	Suppose that P1 allocates a trap at state $0$ (colored red). Without the trap, from state $7$, P2 was guaranteed to visit $F$ because, if P1 chose $(7, 3)$ then a final state was visited immediately and if P1 chose $(7, 0)$ then P2 could choose $(0, 3)$ at state $0$ to visit $F$. However, when trap is allocated at $0$, P1 can choose $(7, 0)$ at state $7$ to enforce a visit to a trap, thereby achieving its safety objective. 
%	
%	Now, consider state $6$. Following Lemma~\ref{lma:advantage-of-traps}, if we were to use Alg.~\ref{alg:zielonka} to compute the sure winning region of P1 with $X = \{0\}$ as final states, then P1's winning region would be $\{0, 7\}$. This is because, at state $6$ in $\game_{X}^1$, there exists a self-loop action using which P2 can prevent the game from reaching $0$. But, since the self-looping action $(6, 6)$ is not a rank-reducing action for P2 in $\game$, P2 will never use $(6, 6)$ at state $6$. If $(6, 6)$ is eliminated from P2's available actions at state $6$, then $6$ becomes a sure winning state for P1 to visit the trap state $0$. 
%	\qed
%	\aknote{I will develop a running example to jointly illustrate allocation of fakes and traps. This example is just for traps.}
%\end{example}
%
%
%Formally, the action $(6, 7)$ at state $6$ in Fig.~\ref{fig:inverted-jobstmann-example} as a \emph{subjectively rationalizable} action for P2. This is because in P2's perceptual game, the action is rational. Whereas, the self-loop $(6, 6)$ is not subjectively rationalizable at $6$. Interested readers are referred to \cite{} for an elaborate discussion on subjective rationalizability for hypergames. 
%
%
%Given any state $s \in S$, let $\rank_{X, Y}^i(s)$ denote the rank of state $s$ in the game $\game_{X, Y}^i$, $i = 1, 2$. 
%
%
%\begin{definition}[Subjectively Rationalizable Actions]
%	\label{def:sracts}
%	% 
%	Given P2's perceptual game $\game^2_{X, Y}$, an action $a \in A_2$ is said to be \emph{subjectively rationalizable} at a state $s \in S_2 \cap \win_2(\game_{X, Y}^2)$ if and only if the state $s' = \Delta(s, a)$ satisfies $\rank_{X, Y}^2(s') < \rank_{X, Y}^2(s)$. Every action at a P1 state $s \in S_1 \cap \win_2(\game_{X, Y}^2)$ is subjectively rationalizable for P2. The set of subjectively rationalizable actions at any state $s \in \win_2(\game_{X, Y}^2)$ is denoted by $\srAct(s)$. 
%\end{definition}


A strategy is said to be \emph{subjectively rationalizable} if it maps any state to a subset of subjectively rationalizable actions at that state. The following lemma shows that every true sure winning strategy of P2 is subjectively rationalizable. Converse may not be true. \ak{This statement doesn't agree with lemma. Update lemma.}


\begin{lemma}
	In P2's perceptual game $\game_{X, Y}^2$, given any P2 state $s \in \win_2(\game, F)$, the set of subjectively rationalizable action includes an action $a \in \srAct(s)$ which is sure winning for P2 in the base game, $\game$. That is, there exists a sure winning strategy $\pi_2$ in $\game$ such that $\pi_2(s)$. 
\end{lemma}


\begin{example}
	TODO. 
\end{example}


From Lemma~\ref{}, we conclude that \emph{fake targets do not benefit P1 when placed in $\win_1(\game, F)$}. With this observation, we define a graph-based model representing $\hgame_1(X, Y)$ which P1 solves to compute its strategy in the L2-hypergame, $\hgame_2(X, Y)$.


\begin{definition}
	\label{def:hgame-labeling-misperception}
	% 
	Given the hypergame $\hgame_2(X, Y)$, \ak{revise: the hypergame on graph $\hgame_1$ is the following game on graph in which P1 has a reachability objective.}
	\[
	\widehat \hgame_1(X, Y)  = \langle \win_2(\game, F), A, \widehat T_{X, Y}, X \cup Y \rangle,
	\]
	where 
	\begin{itemize}
		\item $\win_2(\game, F)$ is P2's sure winning region in $\game$.
		
		\item $\widehat T_{X, Y}: S \times A  \rightarrow S$ is a \emph{deterministic} transition function such that, for any state $s \in \win_2(\game, F)$, $\widehat T_{X, Y}(s, a) = T(s, a)$ if and only if $a \in \srAct(s)$. Otherwise, $\widehat{T}_X(s, a)$ is undefined. 
		
		\item $X \cup Y \subseteq \win_2(\game, F) \setminus F$ is the set of states representing P1's reachability objective.  
	\end{itemize}	
\end{definition}
%\aknote{(Internal) We define the $\widehat{\hgame}_1(X, Y)$ over $S$ because P2 may be incentivized to visit $\win_1(\game, F)$ by allocating $Y \subseteq \win_1(\game, F)$.}


It is noted that the set $X \cup Y$ in $\widehat{\hgame}_1(X, Y)$ defines P1's reachability objective, not P2's objective.

%\replaced{REPLACE THIS!}{Intuitively, $\widehat{\hgame_1}$ only considers P2's winning states $\win_2(\game)$ because, following Proposition~\ref{prop:traps-p1-perceptual-win-regions}, we know that only a subset of $\win_2(\game)$ can be turned into P1's winning states by allocating traps. The transition function eliminates P2's actions that are not subjectively rationalizable.  }


\begin{theorem}
	\label{thm:hgame-swin-is-dswin}
	%		
	Given a state $s \in \win_2(\game, F) \setminus F$, let $\pi_2$ be any subjectively rationalizable, sure winning strategy of P2 to visit $F \cup Y$. Then, a strategy $\pi_1$ is sure winning for P1 in true game $\game_{X, Y}^1$ if and only if $\pi_1$ is a sure winning strategy for P1 in $\widehat{\hgame}_1$.
\end{theorem}


Theorem~\ref{thm:trap-effect} is true by construction. To see this, first, recall that a sure winning strategy of P1 ensures satisfaction of P1's reachability objective against every possible strategy choice of strategy by P2. And, notice that the set of all P2 strategies in the hypergame $\widehat{\hgame}_1(X, Y)$ is equal to the set of all subjectively rationalizable strategies of P2 in $\game_{X, Y}^1$. 

%To see this, recall that a sure winning strategy of P1 ensures satisfaction of P1's reachability objective against every possible strategy choice of strategy by P2. In the hypergame $\widehat{\hgame}_1(X, Y)$, the set of all P2 strategies is equal to the set of all subjectively rationalizable strategies of P2 in $\game_{X, Y}^1$. And, the set of all P1 strategies is equal to the set of all subjectively rationalizable strategies of P1 in $\game_{X, Y}^1$.


Since P1's sure winning strategy in $\widehat \hgame_1(X, Y)$ enforces a visit to $X \cup Y$ by leveraging P2's misinformation, it is called P1's \emph{sure winning strategy under deception}, for short, \emph{deceptive sure winning strategy}. The strategy is \emph{stealthy} because it always selects an action that is subjectively rationalizable in P2's view. Thus, P2 cannot become aware of deception. The sure winning region of P1 in $\widehat \hgame_1(X, Y)$ is called the \emph{deceptive sure-winning region}, denoted $\dswin_1(X, Y)$. % It is easy to see that every state from which P1 can surely win without deception is also a state in P1's deceptive winning region, \ie, $\win_1(\game_{X, Y}^1, F) \subseteq \dswin_1(X, Y)$.


We conclude this section by providing a condition for a state to be sure winning for P2 regardless of whether P1 uses deception. From these states, any subjectively rationalizable P2 strategy must avoid visit $X \cup Y$. We call such a P2 strategy as \emph{sure winning strategy of P2 under deception}, or abusing the notation slightly, P2's deceptively sure winning strategy.


%For this, we identify the states from which every subjectively rationalizable, sure winning strategy of P2 induces a visit to $F$ without visiting $X \cup Y$. Such a strategy is called a \emph{sure winning strategy of P2 under deception}, for short, P2's deceptively sure winning strategy. 


%Given P1's deceptive sure winning region, next, we want to characterize the set of states from which P2 can surely visit $F$ regardless of P1 using deception. Since $\widehat{\hgame}_1(X, Y)$ is an instance of Definition~\ref{def:game}, due to Fact~\ref{fact:determinacy}, P2 has a sure winning strategy from every state in $\win_2(\game) \setminus \dswin_1$. However, due to misperception, P2 might follow a strategy that is not sure winning. This is because P2 does not know $\widehat{\hgame}_1(X, Y)$. In this case, we say a state is deceptively sure winning for P2 if and only if every subjectively rationalizable strategy of P2 from that state is also a rational strategy in the true game.


\begin{proposition}
	\label{prop:traps-dswin2}
	%  
	Given any state $s \in \win_2(\game, F) \setminus F$, P2 has a deceptive sure winning strategy to visit $F$ from $s$ if and only if, for any pair of P1 and P2 strategies $\pi_1, \pi_2$, the path $\rho = \outcomes(s, \pi_1, \pi_2)$ in $\widehat{\hgame}_1(X, Y)$ does not visit $X \cup Y$. That is, $s$ is disconnected from $X \cup Y$ in the underlying graph of $\widehat{\hgame}_1(X, Y)$.
\end{proposition}
\begin{proof}[Proof (Sketch)]
	Let $\Pi^{SR}_2(\game_{X, Y}^2)$ be the set of P2's subjectively rationalizable strategies in $\game^2$. Given any pair of strategies $\pi_2, \pi_2' \in \Pi^{SR}_2(\game_{X, Y}^2)$, P2 has no incentive to choose $\pi_2$ over $\pi_2'$, or vice versa, because, in P2's perspective, starting from state $s$, both of them visit $F$ in at most $k$ steps, where $k$ is the rank of state $s$ in $\game_{X, Y}^2$. As a result, there exists a possibility that P2 chooses $\pi_2$ even if the resulting path $\rho = \outcomes(s, \pi_1, \pi_2)$, when P1 follows $\pi_1$ and P2 follows $\pi_2$, visits a state in $X \cup Y$ before visiting $F$. Noting that the set of all P2 strategies in $\widehat{\hgame}_1(X, Y)$ is equal to $\Pi^{SR}(\game^2)$, the states from which P2 is ensured to visit $F$ without visiting $X \cup Y$ are the states that are disconnected from $X \cup Y$ in the underlying graph of $\widehat{\hgame}_1(X, Y)$. 
	%		Given a set of subjectively rationalizable strategies at $s$, P2 has no incentive to choose any given strategy over the another because, in P2's perspective, all of them visit $F$. Therefore, if there exists a subjectively rationalizable strategy $\pi_2^*$ that induces a visit to $X \cup Y$, then there exists a possibility that P2 selects $\pi_2^*$. Thus, the states from which P2 is ensured to visit $F$ are those that are disconnected from $X \cup Y$ because every strategy at a state $s \in \win_2(\game, F) \setminus F$ in $\widehat{\hgame}_1(X, Y)$ is subjectively rationalizable, by construction. 
\end{proof}


It follows that $\widehat{\hgame}_1$ is \emph{not} determined. That is, from any state $s \in \win_2(\game, F) \setminus F$ which is connected to $X \cup Y$, the winner of the game can only be determined after players fix their strategies.


%Finally, we consider the case where the decoys $X \cup Y$ are placed in $\win_1(\game, F)$. 
%\begin{proposition}
%	\label{prop:decoy-in-win1-benefit}
%	If $X \cup Y \subseteq \win_1(\game, F)$, then $\dswin_1(X, Y) = \win_1(\game_{X, Y}^1, F) =  \win_1(\game, F)$. 
%\end{proposition}
%\begin{proof}
%	By Theorem~\ref{thm:traps-p1-perceptual-win-regions}, \ref{thm:fakes-p1-perceptual-win-regions}. 
%\end{proof}
%
%
%Proposition~\ref{prop:decoy-in-win1-benefit} states that P1 gains no benefit by placing decoys in $\win_1(\game, F)$. However, for similar reason as Proposition~\ref{prop:decoy-in-win1-benefit}, such a placement reduces the size of P2's deceptive winning region. 
%
%%Although P1 placing decoys in $\win_1(\game, F)$ does not affect sure winning region of P1, it shrinks the states from which P2's deceptive winning region. Again, this is a consequence of non-determinacy of $\widehat{\hgame}_1(X, Y)$.
%
%\begin{proposition}
%	If $X \cup Y \subseteq \win_1(\game, F)$, then $\dswin_2(X, Y) \subseteq \win_2(\game_{X, Y}^1, F)$. 
%\end{proposition}
%
%
%%Similar to Proposition~\ref{prop:traps-dswin2}, notice that any strategy that visits $Y$ is subjectively rationalizable for P2. Thus, there is a possibility that P2 may choose such a strategy.
%
%
%
%%In conclusion, the partition of state space of a L2-hypergame in Definition~\ref{def:generalized-hypergame} can be represented as shown in Fig.~\ref{fig:hgame-partition}. 




==> sections/main.tex <==
\paragraph*{} \ak{TODO.} 

%Our proposed solution to Problem~\ref{prob:decoy-placement} is based upon two key ideas from formal methods and hypergame theory, namely (a) deceptive synthesis, and (b) compositional synthesis. In Sec.~\ref{subsect:hgame}, we introduce  deceptive synthesis to construct a strategy for P1 to deceive P2 into reaching a pre-defined decoy set in finitely many steps by exploiting the  incomplete information of P2. The strategy is called \emph{deceptive sure-winning strategy} and depends on the chosen set of decoys. Then, in Sec.~\ref{subsect:compsynth}, we introduce a compositional synthesis approach to identify an approximately optimal allocation of decoys. 


==> sections/mixture.tex <==
\paragraph*{} Is allocating fakes or traps more beneficial? Yes, because given a set of states in $Z \subseteq \win_2 \setminus F$ if . 

\begin{proposition}
	Given a subset $Z \subseteq \win_2 \setminus F$, we have $\vod(\emptyset, Z) \geq \vod(Z, \emptyset)$. 
\end{proposition}
\begin{proof}[Proof (Idea)]
	Show that $\win_2(Z, \emptyset) \subseteq \win_2^2(\emptyset, Z) \setminus \win_2$. When traps are allocated, only the states from which P1 has sure winning strategy to visit $Z$ are removed from P2's winning region. Whereas, when $Z$ is are allocated as fake targets: note that sure winning states to visit $Z$ is a subset of $\win_2^2(\emptyset, Z) \setminus \win_2$. Show that it can also be larger: an example should suffice. 
\end{proof}


\aknote{To allocate, reduce the problem to GameSec paper. When computing $\{s: \dswin\}$ set, instead, construct $\{(s, \mathsf{fake}): \dswin\} + \{(s, \mathsf{trap}): \dswin\}$. Modify the algorithm to select at most $k$ traps and $m$ fake targets, and that no state is allocated as both fake target and trap. But allocation is done in mixed way. }

 

==> sections/randomized.tex <==
% 1. Prove. $\win_1(G_{Z, \emptyset}^1, F) = \win_1(G_{\emptyset, Z}^1, F \cup Z)$. 
% 2. Solving using Hypergame MDP, LCSS20 paper. 
% 2a. SR Strategy definition. 
% 3. Difference with . Game is determined. 
% 4. Allocation algorithm remains the same. 
% 5. The optimal allocation is different! Reason: SR strategy is different. 

In this section, we examine Problem~\ref{prob:decoy-placement} under the almost-sure winning criterion, when players employ randomized strategies. Unlike the result from Section~\ref{subsec:allocation}, we find that there is no clear advantage of either fakes or traps over the other. This difference stems from the fact that, when using randomized strategies, the players are not required to use rank-reducing strategies. Consequently, the set of actions subjectively rationalizable for P2 in this case is different.


\begin{definition}[Subjectively Rationalizability under Almost-sure Winning Criterion]
	Let $\game^2_{X, Y}$ be P2's perceptual game. When the game is analyzed under almost-sure winning criterion, an action $a \in A_2$ is said to be \emph{subjectively rationalizable} at a state $s \in S_2 \cap \win_2(\game_{X, Y}^2, F \cup Y)$ if and only if the next state $s' = T(s, a)$ is also almost-surely winning for P2, \ie, $s' \in \win_2(\game_{X, Y}^2, F \cup Y)$. At any state in $S_1 \cup (S_2 \setminus \win_2(\game_{X, Y}^2, F \cup Y))$, every action is subjectively rationalizable for P2.
\end{definition}
%\aknote{Add Fact that SW and ASW are equal in DTPTB Game.} 
%\aknote{Highlight that results of 4.1 apply here as well.}


%First, due to Fact~\ref{fact:SWin-ASWin-equivalence}, we note that the results from Section~\ref{subsec:effects-of-decoy} apply to the case when the players use randomized strategies and analyze their perceptual games under almost-sure winning criterion. 


Intuitively, every P2 action that restricts the game within P2's winning region $\win_2(\game_{X, Y}^2, F \cup Y)$ is subjectively rationalizable for P2. This is because (a) from every state within this region, there exists a path that visits $F \cup Y$, and (b) every P1 action at any $s \in \win_2(\game_{X, Y}^2, F \cup Y) \cap S_1$ is ensured to stay within P2's winning region. Therefore, P2 is guaranteed to visit its perceived final states $F \cup Y$ with probability one by following a randomized strategy that selects all actions which do not exit $\win_2(\game_{X, Y}^2, F \cup Y)$ \cite{kulkarni2021deceptive}. 


As a result, P1 can construct a graph-based model for L1-hypergame $\hgame_1$ by marginalizing the true game $\game_{X, Y}^1$ with P2's strategy. 


\begin{definition}[Adopted from {\cite{kulkarni2021deceptive}}]
	\label{def:hgame-mdp}
	% 
	Given the true game $\game_{X, Y}^1$, the L1-hypergame $\hgame_1(X, Y)$ is the following \ac{mdp} in which P1 has a reachability objective.
	\[
		\widetilde \hgame_1(X, Y)  = \langle \widetilde S, A, \widetilde T_{X, Y}, X \cup Y \rangle,
	\]
	where 
	\begin{itemize}
		\item $\widetilde S = \win_2(\game, F)$ is P2's sure winning region in $\game$. At P1 states in $\widetilde{S}_1 = \win_2(\game, F) \cap S_1$, P1 chooses the next action strategically. Whereas, the states in $\widetilde{S}_2 =\win_2(\game, F) \cap S_2$ are \emph{probabilistic} states. 
		
		\item $\widehat T_{X, Y}: \widetilde S \times A \rightarrow \dist{\widetilde S}$ is a transition function defined as follows: any state $s \in X \cup Y$ is a sink state. At a state $s \in \widetilde{S}_1$, we have $\widehat T_{X, Y}(s, a, s') = 1$ if and only if $s' = T(s, a)$. At a state $s \in \widetilde{S}_2$, we have $\widehat T_{X, Y}(s, a, s') > 0$ if and only if $a \in \srAct(s)$ and $s' = T(s, a)$. Otherwise, $\widehat T_{X, Y}(s, a, s') = 0$. 
				
		\item $X \cup Y \subseteq \win_2(\game, F) \setminus F$ is the set of states representing P1's reachability objective.  
	\end{itemize}	
\end{definition}


The following result is known from \cite[Theorem~2]{kulkarni2021deceptive}.


\begin{proposition}
	P1 can guarantee a visit to $X \cup Y$ from a state $s \in \win_2(\game, F)$ in the true game $\game_{X, Y}^1$ if and only if P1 has an almost-sure winning strategy to visit $X \cup Y$ from the state $s$ in $\widetilde{\hgame}_1(X, Y)$. 
\end{proposition}


A state from which P1 can guarantee a visit to $X \cup Y$ with probability one are called P1's \emph{deceptive almost-sure winning state}. The set of all such states is called P1's \emph{deceptive almost-sure winning region} and is denoted by $\daswin_1(X, Y)$. 


Now, we prove the key result of this section: \emph{When players use randomized strategies and the games are analyzed under almost-sure winning criterion, fake targets are equally valuable as traps}. 


\begin{theorem}
	For any $Z \subseteq \win_2(\game, F) \setminus F$, we have $\daswin_1(Z, \emptyset) = \daswin_1(\emptyset, Z)$. 	
\end{theorem}
\begin{proof}[Proof (Sketch)]
	Notice that the sets of subjectively rationalizable actions at any state in $\game_{Z, \emptyset}^2$ and $\game_{\emptyset, Z}^2$ are equal. Therefore, any almost-sure winning strategy to visit $Z$ in $\game_{Z, \emptyset}^2$ is also an almost-sure winning strategy to visit $Z$ in $\game_{\emptyset, Z}^2$. 
\end{proof}
	

Since the fake targets and traps are equally valuable, Algorithm~\ref{alg:greedymax} can be used to place the decoys in this setting by replacing $\dswin_1(X, Y)$ with $\daswin_1(X, Y)$. 



==> sections/traps.tex <==
\paragraph*{} We start by analyzing the effect of traps allocation. Because P2 cannot recognize traps, P2's perceptual game remains identical to the base game that contains no decoys. That is, $\game_{X}^2 = \game$. Therefore, the winning regions perceived by P2 in $\game_{X}^2$ are identical to that in the base game, $\game$.


\begin{proposition}
	\label{prop:traps-p2-perceptual-win-regions}
	%	
	In P2's perceptual game $\game^2_X$, we have
	$\win_1(\game^2_X) = \win_1(\game)$, and 
	$\win_2(\game^2_X) = \win_2(\game)$. 
\end{proposition}


\paragraph*{} Unlike in P2's perceptual game, the players' winning regions in P1's perceptual game depend on whether the traps are allocated within $\win_1(\game)$ or $\win_2(\game)$. 


\begin{proposition}
	\label{prop:traps-p1-perceptual-win-regions}
	%	
	In P1's perceptual game $\game^1_X$, the following statements hold.
	
	\begin{enumerate}
		\item If $X \subseteq \win_1(\game)$ then $\win_1(\game^1_X) = \win_1(\game)$ and $\win_2(\game^1_X) = \win_2(\game)$.
		
		\item If $X \subseteq \win_2(\game) \setminus F$ then $\win_1(\game^1_X) \supseteq \win_1(\game)$ and $\win_2(\game^1_X) \subseteq \win_2(\game)$.
	\end{enumerate}
\end{proposition}
\begin{proof}
	(1). We show that $\win_2(\game_X^1) = \win_2(\game)$. The validity of $\win_1(\game_X^1) = \win_1(\game)$ follows from Fact~\ref{fact:determinacy}. 
	
	($\win_2(\game) \subseteq \win_2(\game_X^1)$). From every state $s \in \win_2(\game)$, P2 has a sure winning strategy $\pi_2$ that, for any P1 strategy $\pi_1$, results in a path $\rho = \mathsf{Outcome}(s, \pi_1, \pi_2)$ which visits $F$. Moreover, every state in $\rho$ is an element of $\win_2(\game)$. Since the traps are allocated in $\win_1(\game)$, none of the states appearing in any $\rho \in \mathsf{Outcome}(s, \pi_1, \pi_2)$ are marked as sink states in $\game^1_X$ when compared to $\game$. Therefore, every path in $\mathsf{Outcome}(s, \pi_1, \pi_2)$ in $\game$ is also a valid path in $\game_X^1$. By definition, $s$ is a sure winning state for P2 in $\game_X^1$. 
		
	($\win_2(\game) \supseteq \win_2(\game_X^1)$). Due to Fact~\ref{fact:determinacy}, $\win_2(\game) \supseteq \win_2(\game_X^1)$ is true whenever $\win_1(\game) \subseteq \win_1(\game_X^1)$. We will show the latter statement. 
	
	From every state $s \in \win_1(\game)$, P1 has a sure winning strategy $\pi_1$ that, for any P2 strategy $\pi_2$, results in a path $\rho = \outcomes(s, \pi_1, \pi_2)$ that remains within $\win_1(\game)$ indefinitely. For the statement to be true, it is sufficient to show that even after allocating traps in $\win_1(\game)$, the path $\rho$ remains within $\win_1(\game)$ indefinitely. This is indeed the case because if a trap state $t \in X$ appears in $\rho$, then $\rho$ remains within $\win_1(\game)$ because every state until $t$ is visited is in $\win_1(\game)$ and thereafter the game remains at $t$, because $t$ is a sink state. If $\rho$ does not visit a trap, it remains in $\rho$, by definition. 
	
	From above two statements, it follows that $\win_2(\game) = \win_2(\game_X^1)$. 
	
	(2). Trivial. Every state $s \in X$ is P2's sure winning state in $\game$. Since allocating $s$ as trap makes it a sink state, it is disconnected from $F$ and, therefore, is included in $\win_1(\game_X^1)$.
\end{proof}


\paragraph*{} Intuitively, when traps are allocated within P1's winning region in $\game$, the winning regions of players remain unaffected because, from any state in $\win_1$, P1 has a strategy to remain within $\win_1$ indefinitely even when traps do not exist. Whereas, from any state in $\win_2$, a rational P2 is guaranteed to visit $F$ while never once visiting a state in $\win_1$. 

\paragraph*{} When traps are allocated in $\win_2$, the trap states become winning for P1 as they are converted to `sink'. Moreover, any state from which P1 has a strategy to surely visit $X$ also becomes winning for P1. In fact, the following proposition establishes this to be a necessary and sufficient condition for P1 to satisfy its safety objective from a P2's winning state in $\game$. 


\begin{lemma} \label{lma:advantage-of-traps}
	Let $X \subseteq \win_2(\game) \setminus F$. A strategy $\pi_1$ is sure winning for P1 in its safety objective in $\game^1_X$, \ie, to prevent the game from visiting $F$, if and only if $\pi_1$ is a sure winning strategy to visit $X$. 
\end{lemma}
\begin{proof}
	($\impliedby$). If $\pi_1$ is sure winning for P1 to visit $X$ from a state $s$, then for any strategy $\pi_2$, the path $\rho = \outcomes(s, \pi_1, \pi_2)$ visits $X$. But all states in $X$ are sink states in $\game_X^1$. Therefore, the path cannot visit $F$. Equivalently, $\pi_1$ is sure winning for P1 in its safety objective. 
	
	($\implies$). Since every state $s \in X$ is a sink state, there is no path from $s$ to $F$ in $\game_X^1$. Therefore, all states in $X$ are winning for P1 in $\game_X^1$. Thus, any sure winning strategy $\pi_1$ that visits $X$ from a state $s \in \win_2(\game)$ produces a path $\rho = \outcomes(s, \pi_1, \pi_2)$ that does not visit $F$, regardless of the sure winning strategy $\pi_2$ used by P2. In other words, $\pi_1$ is sure winning for P1 in its safety objective. 
\end{proof}


\paragraph*{} Intuitively, the effect of allocating traps in $\win_2(\game)$ is understood as follows: From any state $s \in \win_2(\game)$, P2 has a winning strategy $\pi_2$ which, for any P1 strategy $\pi_1$, produces a path $\rho \in \mathsf{Outcome}(s, \pi_1, \pi_2)$ that visits $F$. Since allocating a state $s \in \win_2$ as trap converts it to a sink state, any path $\rho$ that visits $s$ cannot visit $F$ in the true game, $\game_X^1$. Thus, allocation of a trap at $s$ cuts the winning paths that visit $F$ through $s$, thereby, converting them from being winning for P2 to being winning for P1.


\paragraph*{} Following Lemma~\ref{lma:advantage-of-traps}, it may seem that the set of states in $\win_2(\game)$ from which P1 can satisfy its safety objective is P1's sure winning region to visit $X$ in $\game_X^1$. The following examples illustrates why this intuition is wrong.


\begin{example}
	Consider the game shown in Fig.~\ref{fig:inverted-jobstmann-example}, in which P1 and P2 states are represented by circle and square states, respectively. P2's goal is to reach $F = \{3, 4\}$ shown as accepting states. Using Alg.~\ref{alg:zielonka}, we obtain $\win_1 = \{1, 2\} $ and $\win_2 = \{0, 3, 4, 5, 6, 7\}$. Particularly, the attractor level set obtained is $[\{3, 4\}, \{0\}, \{7\}, \{6\}, \{5\}]$, where the level-$0$ of attractor contains the final states, level-$1$ contains state $0$ and so on. The sure winning strategy at any P2 state in $\win_2$ is the action that reduces the level of attractor. Therefore, $\pi_2(0) = (0, 3)$ and $\pi_2(6) = (6, 7)$.
	
	\begin{figure}
		\centering 
		\include{figures/inverted-jobstmann}
		\caption{TODO. }
		\label{fig:inverted-jobstmann-example}
	\end{figure}
	
	Suppose that P1 allocates a trap at state $0$ (colored red). Without the trap, from state $7$, P2 was guaranteed to visit $F$ because, if P1 chose $(7, 3)$ then a final state was visited immediately and if P1 chose $(7, 0)$ then P2 could choose $(0, 3)$ at state $0$ to visit $F$. However, when trap is allocated at $0$, P1 can choose $(7, 0)$ at state $7$ to enforce a visit to a trap, thereby achieving its safety objective. 
	
	Now, consider state $6$. Following Lemma~\ref{lma:advantage-of-traps}, if we were to use Alg.~\ref{alg:zielonka} to compute the sure winning region of P1 with $X = \{0\}$ as final states, then P1's winning region would be $\{0, 7\}$. This is because, at state $6$ in $\game_{X}^1$, there exists a self-loop action using which P2 can prevent the game from reaching $0$. But, since the self-looping action $(6, 6)$ is not a rank-reducing action for P2 in $\game$, P2 will never use $(6, 6)$ at state $6$. If $(6, 6)$ is eliminated from P2's available actions at state $6$, then $6$ becomes a sure winning state for P1 to visit the trap state $0$. 
	\qed
\end{example}


\paragraph*{} The example motivates the need for a systematic way to incorporate P2's best response in $\game_X^2$ into P1's decision making. Formally, the action $(6, 7)$ at state $6$ in Fig.~\ref{fig:inverted-jobstmann-example} is referred to as a \emph{subjectively rationalizable} action. Whereas, the self-loop $(6, 6)$ is not subjectively rationalizable at $6$. This is based on the solution concept of subjective rationalizability for hypergames \cite{}. 


\begin{definition}[Subjectively Rationalizable Actions]
	\label{def:sracts}
	% 
	Given P2's perceptual game $\game^2_X$, an action $a \in A_2$ is said to be \emph{subjectively rationalizable} at a state $s \in S_2 \cap \win_2(\game_X^2)$ if and only if the state $s' = \Delta(s, a)$ is such that $\rank(s') < \rank(s)$. Every action at a P1 state $s \in S_1 \cap \win_2(\game_X^2)$ is subjectively rationalizable for P2. The set of subjectively rationalizable actions at any state $s \in \win_2(\game_X^2)$ is denoted by $\srAct(s)$. 
\end{definition}
\aknote{Why not define SRActs at states in $\win_1(\game_X^2)$?}


\paragraph*{} A strategy is said to be \emph{subjectively rationalizable} if it maps any state to a subset of subjectively rationalizable actions at that state.


\paragraph*{} We now define a zero-sum game on graph representing the $\hgame_1$ that P1 solves to compute its strategy in the L2-hypergame, $\hgame_2$.


\begin{definition}
	\label{def:hgame-labeling-misperception}
	% 
	Given the hypergame $\hgame_2$, the hypergame on graph $\hgame_1$  is the tuple,
	\[
	\widehat \hgame_1  = \langle \win_2(\game), A, \widehat T_X, X \rangle,
	\]
	where 
	\begin{itemize}
		\item $\win_2(\game)$ is a set of game states, partitioned into P1's states $S_1 \cap \win_2(\game)$ and P2's states $S_2 \cap \win_2(\game)$.
		
		\item $\widehat T_X: S \times A  \rightarrow S $ is a \emph{deterministic} transition function such that, for any state $s \in \win_2(\game)$, $\widehat T_X(s, a) = T_X(s, a)$ if and only if $a \in \srAct(s)$. Otherwise, $\widehat{T}_X(s, a)$ is undefined. 
		
		\item $X \subseteq \win_2(\game) \setminus F$ is the set of states representing P1's reachability objective.  
	\end{itemize}	
\end{definition}
\aknote{Notation update needed: Add $X$ to $\widehat{\hgame_1}$.}


\paragraph*{} Intuitively, $\widehat{\hgame_1}$ only considers P2's winning states $\win_2(\game)$ because, following Proposition~\ref{prop:traps-p1-perceptual-win-regions}, we know that only a subset of $\win_2(\game)$ can be turned into P1's winning states by allocating traps. The transition function eliminates P2's actions that are not subjectively rationalizable. It is noted that the set $X$ in $\widehat{\hgame_1}$ defines P1's reachability objective, not P2's objective. 


\begin{theorem}
	\label{thm:trap-effect}
	%		
	Let $s \in \win_2(\game)$ be a state in the game $\game$. Let $\pi_2$ be any subjectively rationalizable sure winning strategy from $s$ to visit $F$. Then, a P1 strategy $\pi_1$ guarantees a visit to the set of states $X$ in the game $\game_X^1$, given that Player 2 uses strategy $\pi_2$, if and only if $\pi_1$ is a sure winning strategy for P1 to visit $X$ in the game $\widehat{\hgame_1}$. 
\end{theorem}


\paragraph*{} The correctness of Theorem~\ref{thm:trap-effect} follows from the observation that (a) the set of subjectively rationalizable strategies of P1 in $\game_X^1$ is identical to the set of all P1 strategies in $\widehat{\hgame_1}$, and (b) the set of subjectively rationalizable strategies of P2 in $\game_X^1$ is identical to the set of all P2 strategies in $\widehat{\hgame_1}$. Both statements are true by construction (see Definition~\ref{def:hgame-labeling-misperception}).  


\paragraph*{} Since P1's sure winning strategy in $\widehat \hgame_1$ enforces a visit to $X$ by leveraging P2's misinformation, it is called a \emph{deceptive sure winning strategy}. The winning region of P1 in $\widehat \hgame_1$ is called the deceptive sure-winning region, denoted $\dswin_1$. Note that both the deceptive sure winning strategy and the deceptive sure winning region depend on the states that are allocated as traps.


\paragraph*{} Given P1's deceptive sure winning region, next, we want to characterize the set of states from which P2 can surely visit $F$. Since $\widehat{\hgame_1}$ is an instance of Definition~\ref{def:game}, due to Fact~\ref{fact:determinacy}, P2 has a sure winning strategy from every state in $\win_2(\game) \setminus \dswin_1$. However, due to misperception, P2 might follow a strategy that is not sure winning. This is because P2 does not know $\widehat{\hgame_1}$. In this case, we say a state is deceptively sure winning for P2 if and only if every subjectively rationalizable strategy of P2 from that state is also a rational strategy in the true game.


\begin{proposition}
	\label{prop:traps-dswin2}
	%  
	P2 has a deceptively sure winning strategy from a state $s \in \win_2(\game)$ if and only if it is disconnected from $X$ in $\widehat{\hgame_1}$.
\end{proposition}


\paragraph*{} Intuitively, the correctness of Proposition~\ref{prop:traps-dswin2} is understood as follows: Since $\widehat{\hgame_1}$ only contains subjectively rationalizable actions, if there exists a path from $s$ to $X$, then there must exist strategies $\pi_1, \pi_2$ for the players to realize that path. In addition, because every strategy $\pi_2$ in the hypergame is subjectively rationalizable, there exists a possibility that it would be chosen by P2. Thus, the only states from which P2 is ensured to visit $F$ regardless of which subjectively rationalizable strategy it chooses are the states that are disconnected from $X$. 


\paragraph*{} In essence, Proposition~\ref{prop:traps-dswin2} highlights that not all subjectively rationalizable strategies of P2 are truly rational. From the states in $\win_2(\game) \setminus \dswin_1$ that have a path to both $X$ and $F$, whether P2 wins or loses can be determined only after it chooses a strategy. 



% ===================================================
% DO NOT DELETE: DISCUSSION ON RANDOMIZED STRATEGIES
% ===================================================
%Now that we know $\dswin_1$ is the set of states from which P1 can satisfy its safety objective, we want to determine the set of states from where P2 can visit $F$ surely, regardless of P1's deceptive winning strategy. First, we observe that  from every state in $\win_2(\game) \setminus (F \cup \dswin_1)$, P2 has a sure winning strategy to visit $F$. This is because the state is sure winning for P2 in $\game$. However, since P2 is unaware of traps, P2 might follow a strategy that visits a state in $\dswin_1$. 
%
%
%\begin{proposition}
%	\label{prop:traps-dswin1}
%	Let $\pi_2$ be a randomized sure winning strategy of P2 such that $\pi_2(s)$ selects every subjectively rationalizable action in $\srAct(s)$ with a positive probability. $\pi_2$ ensures a visit to $F$ if no state in $\dswin_1$ is reachable from $s$ in $\widehat{\hgame_1}$.
%\end{proposition}
%\begin{proof}[Proof (Sketch)]
%	By Lemma~\ref{lma:advantage-of-traps}, the only way for P1 to satisfy its safety objective from a state in $\win_2(\game) \setminus F$ is by visiting a trap. From every state in $\dswin_1$, P1 has a strategy to enforce a visit to a trap. Since every subjectively rationalizable action is chosen by $\pi_2$ with a positive probability, if there exists a path from $s$ to a state in $\dswin_1$, the path could occur with a positive probability. Thus, for $\pi_2$ to enforce a visit to $F$ with probability one, there must not be a path from $s$ to $\dswin_1$.
%\end{proof}
%
%
%\paragraph*{} It is reasonable to assume that $\pi_2(s)$ selects every subjectively rationalizable action because P2 has no incentive to prefer any subjectively rationalizable action over another. Even when players use deterministic strategies, the only states from which P2 is ensured to satisfy its reachability objective are the ones that are disconnected from $\dswin_1$. To see this, fix a strategy $\pi_1$ for P1. If there exists a P2's sure winning strategy $\pi_2^*$ at a state $s \in \win_2 \setminus (F \cup \dswin_1)$ in $\game_X^2$ such that the resulting path $\rho = \outcomes(s, \pi_1, \pi_2)$ visits $\dswin_1$, then there is always a possibility that P2 follows $\pi_2^*$. This is because every action selected by $\pi_2^*$ is subjectively rationalizable and P2 has no incentive to not follow $\pi_2^*$.
%
% ===================================================

==> sections/traps_old.tex <==
\paragraph*{} In this subsection, we consider the case when P1 only allocates traps and no fake targets. That is, $X \neq \emptyset$, $Y = \emptyset$, and the true game is $G(X, \emptyset)$. For notation convenience, we simply denote the true game as $\game(X)$ with the understanding that fake targets are absent. We are interested to know: \emph{Given the perceptual games, $\game(X)$ and $\game^2(X)$, what is the advantage of placing traps?} 

 
%\paragraph*{Perceptual Games with Traps.} Given that P2 does not know about the traps, we distinguish her perception of the game from P1's view. For a subset $X\subseteq \Htraps$, P1's perceptual game is same as the true game: $\game(X) = \langle  S, A,T^X ,s_0, F \rangle$, where the transition function $T^X$ is defined from $T$ by making all states in $X$ sink states (a special case of $\game(X, \emptyset)$ in Def.~\ref{def:game-traps-faketargets}). On the other hand, P2's perceptual game is $\game^2 = \langle S, A, T, s_0, F \rangle$, which is the same as the original game before P1 placing any traps. 


%\paragraph*{} Given the perceptual games, $\game(X)$ and $\game^2$, we are interested to know \emph{what advantage does allocating traps provide to P1 with respect to P1's safety objective?} 


\paragraph*{} To answer the above question, we introduce a metric to measure of the \emph{value of deception}. Intuitively, we quantify the advantage of placing traps by measuring the reduction in the size of P2's sure-winning region from game $\game$ with no traps to $\game(X)$, in which the states $X$ are allocated as traps. 


\paragraph*{Notation.} The sure winning regions of P1 and P2 in the game $\game$ be denoted by $\win_1$ and $\win_2$, respectively. The sure winning regions of P1 and P2 in the game $\game(X)$ be denoted by $\win_1(X)$ and $\win_2(X)$, respectively. The sure winning regions of P1 and P2 in the game $\game^2(X)$ be denoted by $\win_1^2(X)$ and $\win_2^2(X)$, respectively. \ak{write better}


\paragraph*{} The value of deception is given by the following expression.

\begin{align}
	\vod = \frac{\abs{\win_2 \setminus F} - \abs{\win_2(X) \setminus F}}{\abs{\win_2 \setminus F}}
\end{align}


\paragraph*{} The value of deception takes a value between $0$ and $1$. $\vod = 0$ indicates that P1 gained no advantage by allocating the traps. Whereas, $\vod = 1$ indicates that P1 gained maximum advantage by allocating the traps.

\aknote{Move VoD definition after hypergame definition after definition of $\game(X, Y)$.}



\paragraph*{} We now investigate the relation between the sure winning regions in P1 and P2's perceptual games to gain an insight into the conditions under which trap allocation may provide advantage to P1. 





\begin{lemma} \label{lma:p2-swin-equal-in-G-and-G2X}
	P2's sure winning region in the perceptual game $\game^2(X)$ is the equal to that in the game $\game$ with no traps allocated, \ie, $\win_2 = \win_2^2(X)$. 
\end{lemma}
\begin{proof}
	Trivial. Because when $Y = \emptyset$, the games $\game$ and $\game^2(X)$ are identical.
\end{proof}


\begin{proposition} 
 	If $X \subseteq \win_1$, then $\vod = 0$.
\end{proposition}
\begin{proof}
	First, recall that there exists no strategy for P1 to enter $\win_1$ from any state $s \in \win_2$ by the definition of $\win_2$. This means there can be no strategy of P1 to reach a trap $X \subseteq \win_1$ from a state $s \in \win_2$. Since there is no strategy for P1 to reach a trap allocated under these constraints from any state  $s \in \win_2$ this means $\win_2 = \win_2(X)$ if $X \subseteq \win_1$. Based on the value of deception defined above if $\win_2 = \win_2(X)$ then $VoD = \frac{\abs{\win_2 \setminus F} - \abs{\win_2 \setminus F}}{\abs{\win_2 \setminus F}} = 0$
\end{proof}


\paragraph*{} Motivate a little why we look at P2's game to understand the following theorem. 
 

\begin{proposition} \label{prop:advantage-of-traps}
	Let $X \subseteq \win_2$. P1 can prevent the game from reaching $F$ from a state $s \in \win_2^2(X) \setminus F$ if and only if there exists a strategy $\pi_1$ such that for every sure winning strategy $\pi_2$ of P2 in its perceptual game $\game^2(X)$, the play induced by $(\pi_1,\pi_2)$ visits $X$. \ak{rewrote the statement on 28 Feb.}
	
%	Given $X \subseteq \win_2$, P1 can prevent the game from reaching $F$ from a state $s \in \win_2 \setminus F$ if and only if it has a strategy to visit $X$.
	
	\ak{For a state $s \in \win_2^2(X) \setminus F$, if P1 has a strategy to prevent the game from reaching $F$, then the strategy ensures the game will visit a trap in $X \subseteq \win_2$.}
\end{proposition}
\aknote{We are assuming deterministic sure winning strategies. Randomized strategies may require us to study positive winning regions---hence, not considering. Ensure the same is in preliminaries.}
\begin{proof}
    First, we recall that $\win_2^2(X) = \win_2$ (Lemma~\ref{lma:p2-swin-equal-in-G-and-G2X}). Therefore, there does not exist a strategy for P1 to enter $\win_1(X)$ from any state $s \in \win_2^2(X)$. Hence, starting at a state $s \in \win_2^2(X)$ the game indefinitely remains within $\win_2^2(X)$.\\
	
   Next, we show that starting from a state $s \in \win_2^2(X)$, if P2 follows its sure winning strategy in its perceptual game, $\game^2(X)$, then the game must either visit either $F$ or $X$.
    
    By way of contradiction, suppose there exists a strategy $\pi_1$ of P1 that prevents the game from reaching $F \cup X$ from an initial state $s \in \win_2^2(X) \setminus F$. Then, $\pi_1$ guarantees that the game stays in $\win_2^2(X) \setminus (F \cup X)$. Since $F \subseteq (F \cup X)$, $\pi_1$ ensures that the game stays in $\win_2^2(X) \setminus F$. This is a contradiction because, by definition, a sure winning strategy $\pi_2$ of P2 ensures a visit to $F$ in finitely many steps, regardless of P1's strategy $\pi_1$. Since there does not exist a strategy for P1 to prevent the game from visiting $F$ from a state $s \in \win_2^2(X)$, it must be the case that $\pi_1$ enforces a visit to $X$. Since every state in $X$ is a sink state, P1 prevents the game from reaching $F$.\\

\end{proof}


\begin{corollary}
	If $X \subseteq \win_2 \setminus F$, then $\vod > 0$. 
\end{corollary}
\begin{proof}
	Note that $X \subseteq \win_2 \setminus \win_2(X)$. Therefore, $\vod \geq \frac{\abs{X}}{\abs{\win_2 \setminus F}}$. 
\end{proof}

\paragraph*{} Propositions~\ref{}-\ref{} establish the necessary and sufficient condition for the traps to provide an advantage for P1. Specifically, P1 must allocate traps within P2's sure winning region in the game $\game$. 

%Provides a mechanism to convert P2's winning states to P1's. It is a N\&S condition for the conversion. It follows that P1 may get advantage by allocating traps within P2's perceived winning region. Can P1 get advantage by allocating traps in P1's SWin in P2's perceived game? 
%
%\begin{corollary}
%	\label{prop:X_in_Win_2^2_advantage}
%	
%	Under the assumption that $X \cap F = \emptyset$, the following statements are true.
%	\begin{enumerate}
%		\item If $X \cap \win_2^2(X) \neq \emptyset$, then $\win_2(X) \subsetneq \win_2^2(X)$.
%		\item If $X \cap \win_2^2(X) = \emptyset$, then $\win_2(X) = \win_2^2(X)$. 
%	\end{enumerate}
%\end{corollary}
%\begin{proof}
%	TODO. 
%\end{proof}
%
%
%\paragraph*{Points to Note.} P1 gets advantage by allocation in P2's winning region and no advantage by allocating traps in P1's winning region. 


\paragraph*{} Suppose that P1 allocates the traps $X$ within P2's sure winning region $\win_2$. Then, we are interested to construct \emph{a stealthy deceptive sure winning strategy using which P1 can prevent the game from visiting $F$.} \ak{what is stealthy deceptive sure winning strategy: define? Why stealthiness is important.}

\begin{definition}[Stealthy Deceptive Sure Winning Strategy]
	\ak{Adopt from LCSS'20}.
\end{definition}

\paragraph*{} To construct a stealthy deceptive sure winning strategy, we first characterize \emph{the states in $\win_2$ from which P1 has a strategy to prevent P2 from visiting $F$}.  To this end, we define a hypergame on graph representing $\hgame^1(X)$ from Definition~\ref{def:generalized-hypergame} that P1 uses to determine its strategy in the L2-hypergame, $\hgame^2(X)$. 


\paragraph*{} The hypergame on graph representing $\hgame^1(X)$ is constructed based on the true game, $\game(X)$. First, we restrict the states to $\win_2$ since we assume that $X \subseteq \win_2$. Second, we disable any actions that P1 knows are not rational for P2 to choose in the game $\game^2(X)$. The rationality of actions is defined with respect to the concept of \emph{subjective rationalizability} from game theory. Specifically, an action is considered subjectively rationalizable at a state if it is rational (in our context, sure winning) in P2's perceptual game $\game^2(X)$. For a rigorous treatment of this concept, we refer the interested reader to \cite{kulkarni2020deceptive}.



\begin{definition}[Subjectively Rationalizable Actions in $\game^2$]
	\label{def:sracts}
	% 
	Given P2's perceptual game $\game^2(X)$, an action $a \in A_2$ is said to be \emph{subjectively rationalizable} at a state $s \in S_2 \cap \win_2^2(X)$ if and only if $\Delta(s, a) \in \win_2^2(X)$. Every P1 action at a state $s \in S_1 \cap \win_2^2(X)$ is subjectively rationalizable. The set of subjectively rationalizable actions at a state $s \in \win_2$ is denoted by $\srAct(s)$.
\end{definition}


\paragraph*{} The removal of actions that are \emph{not} subjectively rationalizable guarantees that P1 remains stealthy \cite{kulkarni2020labeling} \ak{(check if reference is good!)}. That is, P2 cannot detect that P1 is using deception by observing P1's behavior. We now define a zero-sum game on graph representing $\hgame^1(X)$ in which P1 has a reachability objective to visit a trap.


\begin{definition}
	\label{def:hgame-labeling-misperception}
	% 
	Given the hypergame $\hgame^2(X)$, the hypergame on graph $\hgame^1(X)$ to synthesize P1's stealthy deceptive sure winning strategy is the tuple,
	\[
		\widehat \game(X)  = \langle \win_2, A, \widehat T^X, X \rangle,
	\]
	where 
	\begin{itemize}
		\item $\win_2$ is a set of game states, partitioned into P1's states $S_1 \cap \win_2$ and P2's states $S_2 \cap \win_2$.
		
		\item $\widehat T^X: S \times A  \rightarrow S $ is a \emph{deterministic} transition function such that $\widehat T^X(s, a) = T^X(s, a)$ if and only if $a \in \srAct(s)$. Otherwise, $\widehat{T}^X(s, a)$ is undefined. 
		
		\item $X$ is the set of states representing P1's reachability objective.  
	\end{itemize}	
\end{definition}


%\paragraph*{} It is reminded from Definition~\ref{def:game-traps-faketargets} that $F \subseteq \win_2^2(X)$ and that all states in $F \cup X$ are sink states.


\paragraph*{} The hypergame on graph $\widehat \game(X)$ incorporates P2's misperception into P1's decision-making. The next result shows a reduction from the problem of synthesizing stealthy deceptive sure winning strategy in $\game(X)$ to that of synthesizing (non-deceptive) sure winning strategy in $\widehat \game(X)$.


\begin{theorem}
	\label{thm:trap-effect}
	%		
	In the game $\game(X)$, P1 is ensured to reach a trap state in $X$ from a state $s \in \win_2$ if and only if $s$ is a sure winning state for P1 in the game $\widehat \game(X)$.
	
	%	P1 can ensure a visit to a trap in $X$ starting from a state $s \in \win_2$ in game $\game(X)$ if and only if the state $s$ is sure winning for P1 in $\widehat \game(X)$.  
	
	%	Given a state $s$, if P1 has a sure-winning strategy in $\widehat  \game(X)$ starting from $s$, then P1 can ensure a run to reach $X$ but not $F$ by following this sure-winning strategy in $\widehat \game(X)$ in finite many steps.
\end{theorem}
\begin{proof}
	First we show that if $s \in \win_2$ in the game $\game(X)$ is a sure winning state for P1 in the game $\widehat \game(X)$ then P1 has a strategy to visit a trap state X in the game $\game(X)$.\\
 
     This is true by the definition of sure winning in a reachability game. Since the final states in the game $\widehat \game(X)$ are the trap states $X$, if P1 has a sure winning strategy in $\widehat \game(X)$ then P1 is ensured to reach a trap state. \\

    Next, we show that if $s$ is not a sure winning state for P1 in the game $\widehat \game(X)$ then P1 cannot reach a trap state in $X$ from $s$. \\

    By way of contradiction, suppose there is a state $s \in \win_2$ in the game $\game(X)$ that is not sure winning for P1 in the game $\widehat \game(X)$ and P1 can ensure a visit to a trap state $X$ from an initial state $s$. Since $s$ is not sure winning for P1 in the game $\widehat \game(X)$ then it must be sure winning for P2. By the definition of sure winning P2 must have a strategy to ensure the game does not reach a final state $X$ in the game $\widehat \game(X)$. This contradicts the initial statement that P1 can ensure a visit to a trap $X$ from an initial state $s$. Therefore P1 cannot ensure a visit to a trap state $X$ from $s$ if $s$ is not sure winning for P1 in the game $\widehat \game(X)$. \\

    It follows that P1 has a strategy to ensure a visit to a trap state $X$ from $s \in \win_2$ in the game $\game(X)$ if and only if $s$ is a sure winning state for P1 in the game $\widehat \game(X)$. 
\end{proof}

\paragraph*{} Since P1's sure winning strategy in $\widehat \game(X)$ enforces a visit to $X$ by leveraging P2's misinformation, it is called a \emph{deceptive sure winning strategy}. The winning region of P1 in $\widehat \game(X)$ is called the deceptive sure-winning region, denoted $\dswin_1$. Note that both winning regions and winning strategies depends on the trap allocation $X$.


\begin{example}
	Consider the game shown in Fig.~\ref{fig:game-ex1}, in which P1 and P2 states are represented by circle and square states, respectively. P2's goal is to reach state 8 (colored red). Using Zielonka's recursive algorithm from \cite[Ch.2]{gradel_automata_2002} to solve the game, we obtain $\win_1 = \emptyset$ and $\win_2 = S$, indicating that P2 can always reach the target ${8}$ in finitely many steps from any state in the game, regardless of P1's strategy.
		
		
	Now, suppose that a trap is placed at state $7$ (colored gray). In P2's perceptual game $\game^2$, the winning region $\win_2^2(\{7\}) = \win_2 = S$. The action $b_2$ at state $2$ (marked in dashed line) is not subjectively rationalizable for P2 because by taking that action, P1 can then restrict the game to stay within $\{0, 2\}$. 
	
	\begin{figure}
	\centering 
		\include{figures/game-traps-ex}
		\caption{An example to illustrate the effects of traps and P1's deceptive winning strategy. }
		\label{fig:game-ex1}
	\end{figure}

	Given the trap location, we can then compute P1's reachability game for deception, in which $\{7\}$ becomes P1's reachability objective. The solution of this game yields $\dswin_1(\{7\})=\{0, 2 , 4, 7\}$. In words, if the game starts from any state in $\dswin_1$, then P1 can guarantee a visit to $\{7\}$, regardless of which strategy P2 uses as long as it only selects subjective rationalizable actions. P1's deceptive winning strategy is such that at both states $1$ and $4$, P1 selects action $a_2$. 
	
	Different allocations of traps result in different deceptive winning regions for P1. Suppose P1 allocates the trap at $6$ instead of $7$, then $\dswin_1(\{6\})= \{1, 2, 3, 4, 6, 0\}$. Since $\card{\win_2(\{7\})} = \card{\win_2^2(\{7\})} - \card{\dswin_1(\{7\})}$ is greater than $\card{\win_2(\{6\})} = \card{\win_2^2(\{6\})} - \card{\dswin_1(\{6\})}$, allocating a trap at $6$ provides more advantage to P1 than allocating it at $7$. 
	%	One of P1's deceptive sure-winning strategy is $\hat \pi_1 (0)=a_1$, $\hat \pi_1(3) = a_2$, and $\hat \pi_1(4)=a_1$. Clearly, $\card{\dswin_1(\{7\})}<\card{\dswin_1(\{6\})}$. When the size of deceptive sure-winning region is used to assess the benefit of trap allocation, then we can see that placing the trap at $6$ is a better choice than placing it at $7$.
\end{example}
	

==> sections/vod.tex <==
Define two metrics.
